Non-Rigid Designators in Modal and Temporal Free Description Logics (Extended Version)

Definite descriptions, such as 'the General Chair of KR 2024', are a semantically transparent device for object identification in knowledge representation. In first-order modal logic, definite descriptions have been widely investigated for their non-rigidity, which allows them to designate different objects (or none at all) at different states. We propose expressive modal description logics with non-rigid definite descriptions and names, and investigate decidability and complexity of the satisfaction problem. We first systematically link satisfiability for the one-variable fragment of first-order modal logic with counting to our modal description logics. Then, we prove a promising NEXPTIME-completeness result for concept satisfiability for the fundamental epistemic multi-agent logic $\mathbf{S5}^{n}$ and its neighbours, and show that some expressive logics that are undecidable with constant domain become decidable (but Ackermann-hard) with expanding domains. Finally, we conduct a fine-grained analysis of decidability of temporal logics.

==> 3-motivations.tex <==
\section{Motivations and examples}
\label{sec:motivation}
In the following, we provide some motivating examples to illustrate
the novel features of the modal and temporal free DL
languages introduced in the previous section.
\nb{M: rewrite/expand with ToM motivations + fix examples + move to later Sections}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Epistemic scenario.}
We discuss here the main features of the language $\MLALCOud$
interpreted on partial modal interpretations without the RDA and based
on frames
%for $\Sfive$
%where the accessibility relation is an
equipped with an
equivalence relation,
to provide motivating examples in an epistemic
setting. Thus, in the following, we will refer to such interpretations
as \emph{epistemic contexts}, and the worlds of the epistemic context
will be called \emph{states}.

%\paragraph{Terms}
Let us consider the following individual names: $\mathsf{clark}$ standing
for the `Clark Kent', $\mathsf{superman}$ standing for `Superman', and
$\mathsf{lois}$ standing for `Lois Lane'. In a given state of an epistemic
context, $\mathsf{clark}$ and $\mathsf{superman}$ can denote the same element
of the domain. However, since the epistemic context does not satisfy
the RDA, these individual names can also refer to different
individuals at different states. Moreover, the term
$\defdes ( \mathsf{Journalist} \sqcap \exists
\mathsf{worksWith}.\{\mathsf{lois}\})$ can be used to refer to the
journalist that works with Lois Lane, which can be understood as an
alternative way to describe Clark Kent.

%\paragraph{Concepts}
The concept $\Box\{\mathsf{superman}\}$ captures those individuals that are
\emph{known to be} Superman, whereas $\Diamond\{\mathsf{superman}\}$ would
be the set of individuals \emph{suspectable of being} (i.e., for which
it is not known that they are not) Superman.
%
% \paragraph{Concept inclusions}
The following CI can be used to express that Clark Kent is known to be
Clark Kent: $\{ \mathsf{clark} \} \sqsubseteq \Box \{ \mathsf{clark} \}$,
whereas we can use
$\{ \mathsf{clark} \} \sqsubseteq \lnot \Box \{ \mathsf{superman} \}$ to
express that Clark Kent is not known to be Superman. Moreover, the
following CIs assert that Lois Lane is known to be Lois Lane, i.e.,
$\{ \mathsf{lois} \} \sqsubseteq \Box \{ \mathsf{lois} \} $, and she is
also known to love Superman, i.e.,
$\{ \mathsf{lois} \} \sqsubseteq \Box \exists
\mathsf{loves}.\{\mathsf{superman}\}$,
but
%(unfortunately for Clark Kent)
not the journalist that works with
her, i.e., $\{\mathsf{lois}\} \sqsubseteq \lnot \Box \exists \mathsf{loves}.\{
\defdes ( \mathsf{Journalist} \sqcap \exists
\mathsf{worksWith}.\{\mathsf{lois}\}\}$.
%and the journalist that works with
%her, i.e., $\{\mathsf{lois}\} \sqsubseteq \Box\exists \mathsf{loves}.\{
%\defdes ( \mathsf{Journalist} \sqcap \exists
%\mathsf{worksWith}.\{\mathsf{lois}\}\}$.

\begin{example}
%\nb{M: todo fix}

\begin{itemize}
\item In the actual scenario, Clark \emph{is} Superman, but for Lois there is an epistemically conceivable alternative in which he \emph{is not}
\begin{align*}
\Mmf, w & \models \forall u. (\{ \mathsf{clark} \} \Leftrightarrow \{ \mathsf{superman} \}) \\
\Mmf, v & \not \models \forall u. (\{ \mathsf{clark} \} \Leftrightarrow \{ \mathsf{superman} \})
\end{align*}
\item
Lois knows that Superman is the hero that saves her
\[
\Mmf, w \models \Box \forall u. (\{ \mathsf{superman} \} \Leftrightarrow \{ \defdes ( \mathsf{Hero} \sqcap \exists
\mathsf{saves}.\{\mathsf{lois}\}) \} )
\]
\item
Lois loves who she knows to be the hero that saves her
\[
\Mmf, w \models \forall u. ( \{ \mathsf{lois} \} \Rightarrow \exists \mathsf{loves}. \Box \{ \defdes ( \mathsf{Hero} \sqcap \exists \mathsf{saves}.\{\mathsf{lois}\}) \} )
\]
\item
Lois actually loves Clark without even realising it
\begin{align*}
\Mmf, w \models & \forall u. ( (\{ \mathsf{lois} \} \Rightarrow \exists \mathsf{loves}.\{ \mathsf{clark} \} ) \\
						  & \sqcap \lnot \Box (\{ \mathsf{lois} \} \Rightarrow \exists \mathsf{loves}.\{ \mathsf{clark} \}) )
\end{align*}
\end{itemize}
\end{example}


% \paragraph{Formulas}

% The formula
% $\Box (\{ \mathsf{lois} \} \sqsubseteq \exists \mathsf{loves}.\{
% \mathsf{superman} \})$ states that it is known that Lois Lane loves
% Superman, whereas the formula
% $\lnot \Box (\{ \mathsf{lois} \} \sqsubseteq \exists \mathsf{loves}.\{
% \defdes ( \mathsf{Journalist} \sqcap \exists
% \mathsf{worksWith}.\{\mathsf{lois}\} ) \})$ says that it is not known
% that Lois Lane loves the journalist that works with her.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Temporal scenario.}
In the following, we exemplify and discuss the main features of the
language $\TLALCOud$ interpreted on partial traces without the RDA.
%providing motivations for its constructors and semantic choices.

%\paragraph{Terms}
Let us consider the individual name $\mathsf{dl}$ which can serve as a
``variable''-name, that might change its value (and even remain
uninterpreted) at different instants, so to denote, e.g., the
Description Logic (DL) workshops that take place over the years.
Instead, the individual name $\mathsf{dl22}$ can be used as an
individual name with a fixed referent across time, denoting the DL
workshop that takes place in 2022 only. Finally, the definite
description $\defdes\exists \mathsf{isGCof}.\{\mathsf{dl}\}$ is
able to refer non-rigidly to the General Chair of the DL workshop.

%\paragraph{Concepts}
The concept $\Diamond^{+} \{\mathsf{dl}\}$ can be used to refer to
those objects that will eventually be the DL workshop. When
interpreted on total traces with the RDA, the extension of this
concept would contain exactly one object, i.e., the (rigid) referent
of the individual name $\mathsf{dl}$. On the other hand, on partial
traces without the RDA, its extension might contain also zero, or more
than one, objects, namely, those individuals that are the values of
$\mathsf{dl}$ at different time points. In addition, the concept
$\Diamond^{+}\{\defdes\exists\mathsf{isGCof}.\{\mathsf{dl}\}\}$ can be
used to represent those individuals that will eventually be the
General Chair of the various DL workshops.
%
The concept
$\Diamond^{+} \exists \mathsf{hasPCM}.\Diamond^{+} \{\defdes \exists
\mathsf{isGCof}.\{\mathsf{dl}\}\}$ captures those objects that will
eventually have as PC Members some individuals that, at some point in
the future, will be the General Chair of the DL workshop.

% \paragraph{Concept inclusions}
Let $\mathsf{proc\mbox{-}dl22}$ stands for the proceedings of the DL22
workshop. To enforce the proceedings of the DL22 to behave as a rigid
designator, we can enforce the following CI,\nb{A: expanding?}
$\Diamond^{+} \{\mathsf{proc\mbox{-}dl22}\} \sqsubseteq
\Box^+\{\mathsf{proc\mbox{-}dl22}\}$.
%
% To let the individual name $\mathsf{dl22}$ for the DL22 workshop
% behave as a rigid designator, we can enforce both the CIs
% $\{ \mathsf{dl22} \} \sqsubseteq \Box^{+} \{ \mathsf{dl22} \}$ and
% $\Diamond^{+} \{ \mathsf{dl22} \} \sqsubseteq \{ \mathsf{dl22} \}$,
% or, alternatively, the CI
% $\Diamond^{+} \{ \mathsf{dl22} \} \sqsubseteq \Box^+\{ \mathsf{dl22}
% \}$.
On the other hand, we can require $\mathsf{dl}$ to be a
\emph{flexible} designator by enforcing the following CI,
$\top \sqsubseteq \exists u.(\Diamond^{+}\{\mathsf{dl}\} \sqcap
\Diamond^{+} \lnot \{ \mathsf{dl}\})$.
%
% $\Diamond^{+}\{ \mathsf{dl} \} \sqsubseteq \Diamond^{+} \lnot \{
% \mathsf{dl}\}$. An individual name which is left uninterpreted at each
% instant of a partial trace would satisfy all the previous CIs, thus
% behaving both as a rigid and as a flexible designator. To state
% instead that $\mathsf{dl}$ is \emph{not} a rigid designator, we can
% use the CI
% $\top \sqsubseteq \exists u.( \Diamond^{+} \{ \mathsf{dl} \} \sqcap
% \Diamond^{+} \lnot \{ \mathsf{dl} \} )$, involving the universal role.
Finally, we can enforce $\mathsf{dl22}$ to be an \emph{instantaneous}
designator by using the following CIs,
$\top \sqsubseteq \Diamond^{+}\exists u.\{\mathsf{dl22}\}$,\nb{A: No
  if CI are global}
$\Diamond^{+} (\{\mathsf{dl22}\} \sqcap
\Diamond\{\mathsf{dl22}\})\sqsubseteq \bot$, meaning that
$\mathsf{dl22}$ is not a ghost and that no objects can be the denotation
of the individual name $\mathsf{dl22}$ at two distinct instants.
%
Notice that ghost individuals are assumed to be (vacuously) rigid,
while flexible and instantaneous individuals should denote.

%\paragraph{Formulas}
To state that the (current) General Chair of DL will be one of next
year's PC Members of DL we can use the assertion,
$(\Next \exists {\sf isPCMof}.\{{\sf dl}\})(\{\defdes\exists {\sf
  isGCof}.\{ {\sf dl }\}\})$.
% Recall that this assertion is just
% shorthand for (the conjunction of) the CIs
% $\top \sqsubseteq \exists u.\{ \defdes \exists {\sf isGCof}. \{ {\sf
%   dl }\} \}$ and
% $\{ \defdes \exists {\sf isPCof}. \{ {\sf dl }\} \} \sqsubseteq \Next
% \exists {\sf isPCMof}. \{ {\sf dl} \}$.
%
On the other hand, to say that, next year, the (future) General Chair
of DL will be one of the PC Members of DL, the following formula
should be used instead,
$\Next (\top \sqsubseteq \exists u.\{\defdes \exists {\sf isGCof}.
\{{\sf dl}\}\} \land \{\defdes \exists {\sf isGCof}.\{ {\sf dl}\}\}
\sqsubseteq \exists{\sf isPCMof}.\{{\sf dl}\})$.
%
Moreover, one can express that, at some point, DL22 will be the DL
workshop, by writing the following assertion,
$\Diamond^{+} (\{\mathsf{dl}\}(\{\mathsf{dl22}\}))$. Finally, the
formula
$\Box^{+}(\{\defdes\exists{\sf isGCof}.\{{\sf dl}\}\}
\sqsubseteq \exists{\sf isPCMof}.\Next\{{\sf dl}\})$ asserts
that it will always be the case that the General Chair of DL is going
to be a DL's PC Member on the subsequent year.
        
\begin{example}
\begin{itemize}
%
	\item
	KR24 is a rigid designator
	\[
	\Mmf, t \models \Diamond^{+} \{ \mathsf{kr24} \} \sqsubseteq
\Box^+  \{ \mathsf{kr24} \}
\]
	\item
	KR24 is the upcoming KR Conference, but there will be more (hopefully)
	\begin{align*}
	\Mmf, t & \models \exists u. \{\mathsf{kr24}\} \land \{\mathsf{kr24}\} \sqsubseteq \Next \{ \mathsf{kr} \}  \\
	\Mmf, t & \not \models \Diamond^{+} \{\mathsf{kr}\} \sqsubseteq \Next \{ \mathsf{kr} \}
	\end{align*}
	\item
	However, KR24 will never come back (as the current KR conference)
	\[
	\Mmf, t \models \Box^{+} (\{ {\sf kr24 } \} \sqsubseteq \Next \Box \lnot \{\mathsf{kr}\} )
\]
\item
Whoever is a Program Chair of KR always becomes either the General Chair or a PC Member of KR next year
	\begin{align*}
\Mmf, t \models \ & \Box^{+} ( \exists {\sf isPrgChr}.\{ {\sf kr} \} \sqsubseteq \\
							& \{ \defdes \exists {\sf isGenChr}. \Next \{ {\sf kr} \} \} \sqcup \exists {\sf isPCMbr}. \Next \{ {\sf kr } \} )
	\end{align*}
\end{itemize}
\end{example}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "rda"
%%% End:


==> camera-ready/0-abstract.tex <==
\begin{abstract}
Definite descriptions, such as
`the General Chair of KR 2024,\!'
are a semantically transparent device for object identification in knowledge representation. In first-order modal logic, definite descriptions have been widely investigated for their non-rigidity, which allows them to designate different objects (or  none at all) at different states. %In this contribution, 
We propose expressive modal description logics with non-rigid definite descriptions and names, and investigate decidability and complexity of the satisfiability problem. We first systematically link satisfiability for the one-variable fragment of first-order modal logic with counting to our modal description logics. Then, we prove a promising \NExpTime{}-completeness result
%upper bound
for concept satisfiability for the fundamental epistemic multi-agent logic $\Sfive^{n}$ 
and its neighbours,
and show that some expressive logics that are undecidable with constant domain become decidable (but Ackermann-hard) with expanding domains. Finally, we conduct a fine-grained analysis of decidability of temporal logics.


%%in, e.g., epistemic or  temporal settings.
%In this direction, we introduce \emph{epistemic} and \emph{temporal} extensions of standard description logics, with nominals and the universal role, additionally equipped with definite descriptions constructors.
%Regarding names and descriptions, in these languages we allow for: possible \emph{lack of denotation}, ensured by \emph{partial} models, coming from free logic semantics as a generalisation of the classical ones; and \emph{non-rigid designation} features, obtained by assigning to terms distinct values across states, as opposed to the standard rigidity condition on individual expressions.
%%from first-order modal logic.
%In the absence of the rigid designator assumption, we show that the satisfiability problem for epistemic free description logics is $\NExpTime$-complete, while satisfiability for temporal free description logics
%%with non-rigid individual names or definite descriptions
%over linear time structures
%is undecidable.
\end{abstract}


==> camera-ready/1-introduction.tex <==
% !TEX root =  rda.tex

%{\color{red}{
%M: To fix
%
%\begin{itemize}
%\item Common knowledge operator: $\mathcal{ML}^{nC}_{\mathcal{ALCO}_{u}^\iota}$ and ${\bf S5}^{nC}_{\mathcal{ALCO}_{u}^\iota}$ (to be mentioned only).
%\item ${\bf K}^{\ast}$?
%\item \sout{Multi-modal languages: $\mathcal{ML}^{n}_{\mathcal{ALCO}_{u}^\iota}$ and ${\bf S5}^{n}_{\mathcal{ALCO}_{u}^\iota}$}.
%\item \sout{undecidability of $({\bf S5}^{m}_{u})_{\mathcal{ALCO}_{u}^\iota}$ formula satisfiability $\leadsto$ undecidability of ${\bf S5}^{m}_{\mathcal{ALCO}_{u}^\iota}$ entailment under global ontology? (ontology := finite set of CIs)}
%\item \sout{partial $\LTLELO$ entailment under global ontology without the RDA?}
%%consequence of $\LTLBDNELO$ global CI under a finite set of $\LTLBDNELO$ global CIs without RDA? (what about partial semantics?)
%\item \sout{$\mathcal{T}\mathcal{L}^{\Until}_{\DL}$, $\mathcal{T}\mathcal{L}^{\Box\Diamond\nxt}_{\DL}$ $\leadsto$ $\mathcal{T}\mathcal{L}_{\DL}$ + $\LTLALCOud$, $\LTLELO$}
%%$\LTLBDNELO$
%\item \sout{$\ALCOud$-$\TL$ without temporalised concepts + $\ALCOud$-$\LTLf$ formula satisfiability problem without the RDA}
%\end{itemize}
%
%}}



\section{Introduction}
\label{sec:intro}

%\nb{M: todo discuss content}
\emph{Definite descriptions},
like
`the General Chair of KR 2024,\!'
%`the KR Conference held in Southeast Asia'/
%`the nearest major galaxy to the Milky Way'/
%`the smallest planet in the Solar System'/
%`the brightest celestial object'
%%`the first celestial object visible at night' (or `the evening star'),
are expressions of the form `the unique $x$ such that $\p$.\!' Together with \emph{individual names}
such as
`Pierre,\!'
%`KR 2024'/
%`Andromeda'/
%`Mercury'/
%`Venus',
they are used as \emph{referring expressions} to identify objects in a given domain~\cite{ReiDal00,BorEtAl16,BorEtAl17}.
%TomWed18

Definite descriptions and individual names can also \emph{fail to designate} any object at all, as in the case of the definite description
`the KR Conference held after KR 2018 and before KR 2020,\!'
%`the KR Conference between KR 2018 and KR 2020'/
%`the planet between Mercury and the Sun'/
or the individual name
`KR 2019.\!'
%`Vulcan'.
In order to admit these
%constructs
%definite descriptions and individual names
as genuine terms of the language, while allowing for their possible lack of referents, formalisms based on \emph{free logic} semantics have been developed~\cite{Ben02,Leh02,Ind21,IndZaw21}.
In contrast, classical logic approaches assume that individual names always designate, and that definite descriptions can be paraphrased in terms of
%sentences expressing
existence and uniqueness conditions, an approach dating back to Russell~(\citeyear{Rus05}).
%
Recently,
%in a non-modal setting,
definite descriptions have been introduced to enrich standard description logics (DLs) with nominals, $\ALCO$ and $\ELO$~\cite{NeuEtAl20,ArtEtAl20b,ArtEtAl21a}.

In particular, DLs $\ALCOud$ and $\ELOud$~\cite{ArtEtAl20b,ArtEtAl21a} include the universal role, $u$, as well as nominals and definite descriptions of the form $\{ \defdes C \}$ (`the unique object in $C$')
as basic concept constructs,
while also employing a free logic semantics that allows non-designating terms.
Hence, for instance, using nominal $\{ \mathsf{kr24} \}$ to designate KR 2024, we can refer to the General Chair of KR 2024 by means of the definite description $\{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \}$.
Then, in $\ALCOud$, we can say that Pierre is the General Chair of KR 2024 with the following concept:
%
\begin{equation*}
\exists u. ( \{ \mathsf{pierre} \} \sqcap \{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \} ).
\end{equation*}
%
Indeed, if this concept is satisfiable (in other words, has a non-empty extension), then there are objects $p$ and $k$ designated by $\mathsf{pierre}$ and $\mathsf{kr24}$, respectively,  and the pair $(p, k)$ belongs to the interpretation of role $\mathsf{isGenChair}$, which contains no other $(o,k)$, thus making $p$ the only object connected to $k$ by  $\mathsf{isGenChair}$.
The free DLs $\ALCOud$ and $\ELOud$ have, respectively, $\ExpTime$-complete ontology satisfiability and $\PTime$-complete entailment problems, thus matching the complexity of the classical
DL counterparts.

Names and descriptions display interesting behaviours also in \emph{modal} (epistemic, temporal) settings. % such as \emph{epistemic} or \emph{temporal} logics. 
These are indeed \emph{referentially opaque} contexts, where the \emph{intension} (i.e., the meaning) of a term might not coincide with its \emph{extension} (that is, its referent)~\cite{Fit04}.
Here, referring expressions can behave as \emph{non-rigid designators}, meaning that they can designate different individuals across different states (epistemic alternatives, instants of time, etc.).
%In addition, expressions referring to the same object cannot always be mutually substituted  in a sentence while preserving the truth value.
%%For instance,
%%even if everyone knows that Venus is a celestial body illuminated by the Sun, not everyone is thereby aware the evening star is illuminated by the Sun, where `the evening star' denotes the planet Venus,~\cite{FregeSenseAndReference}.
%%despite the fact that everyone is aware of the truism that Venus is Venus, not everyone thereby knows that the evening star is Venus, even though `the evening star' denotes the planet Venus.
%%Similarly, the first workshop \ldots
%Indeed, \emph{modal} settings, like the temporal or the epistemic ones, are
%%instances of
%\emph{referentially opaque} contexts, where the \emph{intension} (i.e., the meaning) of a term might not coincide with its \emph{extension} (that is, its referent)~\cite{Fit04}.
%In these cases, referring expressions can behave as \emph{non-rigid designators}, meaning that they can denote different individuals across different states (epistemic alternatives, instants of time, etc.).

For example, in an epistemic scenario, even if everybody is aware that Pierre is the General Chair of KR 2024, not everyone thereby knows that he is also the General Chair of the (only, so far, and excluding virtual location) KR Conference held in Southeast Asia, despite the fact that `the KR Conference held in Southeast Asia' and `KR 2024' refer (to this day) to the same object. Indeed, `the KR Conference held in Southeast Asia' can be conceived to designate another event by someone unaware of its actual reference to KR 2024.
%
%In our formalism, by using the nominals $\{ \mathsf{pierre} \}$ and $\{ \mathsf{kr24} \}$ to denote, respectively, \ldots
%
%\begin{example}
%\nb{M: todo fix -- adjust to conference scenario}
%\begin{itemize}
%\item In our scenario, KR 2024, denoted by $\mathsf{kr24}$, \emph{is} the 21st International Conference on the Principles of Knowledge Representation and Reasoning, denoted by $\mathsf{21icpkrr}$, but there is an epistemically conceivable alternative in which it \emph{is not}
%\begin{align*}
% & \forall u. (\{ \mathsf{kr24} \} \Leftrightarrow \{ \mathsf{21icpkrr} \}), \\
% & \lnot \Box \forall u. (\{ \mathsf{kr24} \} \Leftrightarrow \{ \mathsf{21icpkrr} \})
%\end{align*}
%\item
%It is known that KR 2024 is the (first, and so far only) KR Conference held in Southeast Asia
%\[
%\Box \forall u. (\{ \mathsf{kr24} \} \Leftrightarrow \{ \defdes ( \mathsf{KRConf} \sqcap \exists
%\mathsf{hasLoc}.\mathsf{SEAsiaLoc}) \} )
%\]
%\item
%Pierre is the General Chair of what is known to be the KR Conference held in Southeast Asia
%\begin{align*}
%\forall u. ( & \{ \mathsf{pierre} \} \Rightarrow \\
%				& \{ \defdes \exists \mathsf{isGenChr}. \Box \{ \defdes ( \mathsf{KRConf} \sqcap \exists
%\mathsf{hasLoc}.\mathsf{SEAsiaLoc}) \} \} )
%\end{align*}
%\item
%Pierre actually is the General Chair of the 21 International Conference on the Principles of Knowledge Representation and Reasoning, but it is not known :
%\begin{align*}
%& \forall u. (\{ \mathsf{pierre} \} \Rightarrow \{ \defdes \exists \mathsf{isGenChr}.\{ \mathsf{21icpkrr} \} \} ), \\
%& \lnot \Box (\{ \mathsf{pierre} \} \Rightarrow \{ \defdes \exists \mathsf{isGenChr}.\{ \mathsf{21icpkrr} \} \} )
%\end{align*}
%\end{itemize}
%\end{example}
%
Similarly, in a temporal setting,
`the General Chair of KR'
%`the smallest planet'
refers to
Pierre
%Mercury
in 2024,
%nowadays,
but
will designate someone else over the years.
So, for instance, if we assume that Pierre works and will continue working in Europe, 
%and always will, 
we can conclude that the General Chair of KR currently works in Europe, but we should not infer that it will always remain the case.
%~\cite{FitMen12}.





%For instance, in an epistemic scenario, `the first celestial object visible at night' can be conceived as referring to different astronomical bodies, by someone unaware of its actual coreference with Venus. Similarly, on a temporal scale, `the first celestial object visible at night' might refer to a certain heavenly object in a given season, and to different ones later on in the year.
%
Due to this fundamental and challenging interplay between designation and modalities,
non-rigid descriptions and names
%definite descriptions---and, more generally, non-rigid designators---
have been widely investigated in first-order modal and temporal logics
%\nb{missing ref}
%\nb{M: new edition Fitting \& Mendelshon + Synthese article Indrzejczak \& Zawidzki}
%For instance, while `the smallest planet in the Solar System' currently denotes the Mercury, it instead referred to Pluto less than twenty years ago.
%%For instance, while `the number of planets' currently denotes the number eight, it instead referred to the number nine less than twenty years ago.
%Non-rigid descriptions and names have been proposed
as individual concepts or flexible terms
%as \emph{intensional objects} or \emph{individual concepts},
capable of taking different values across states~\cite{Coc84,Gar01,BraGhi07,KroMer08,FitMen12,CorOrl13,Ind20,Orl21,IndZaw23}.
%The approach by~\cite{FittingMendhelsonFirstOrderModalLogic,FittingFOIntensionalLogic},
%in turn rooted in the modal~\cite{StalnakerThomason?} and intensional~\cite{Montague?} logic literature,
%uses \emph{predicate abstraction} ($\lambda x P$, for a predicate $P$) as a syntactic device to distinguish between:
%%\emph{de re} sentences, like `the number of planets (at the current instant) has always been even' (formalisable as $[\lambda x \Box P (x)](c)$), and \emph{de dicto} ones, such as `It has always been true that the number of planets (at that instant) was even' (with $\Box([\lambda x  P (x)](c))$ used to represent this instead).
%\emph{de re} sentences, like `The smallest planet in the Solar System (at the current instant) has always been close to the Sun' (formalisable as $[\lambda x \Box P (x)](c)$, where: $c$ stands for `the  smallest planet in the Solar System'; $P$ is the predicate `is close to the Sun'; and $\Box$ is read here as `always in the past');
%and \emph{de dicto} ones, such as `It has always been true that the smallest planet in the Solar System (at any of those instants) was close to the Sun' (with $\Box([\lambda x  P (x)](c))$ used to represent this sentence instead).
%%While the former sentence should be evaluated to true (since the number of currently recognised planets is eight, and eight has always been even), the latter one is clearly false (as the number of recognised planets was odd at some point in the past).
%
%When considering modal settings,

%{\color{red} Frank from here}

The aim of this contribution is to introduce modal DLs that have sufficient expressive power to represent the phenomena discussed above, explore their relationship to standard modal DLs without definite descriptions and non-designating names, and investigate decidability and complexity of reasoning in these formalisms.
%\nb{replaced `languages.'}

In detail, we propose the language $\MLALCOud$, which is a modalised extension of the free DL $\ALCOud$.
%
%% ORIGINAL VERSION - PIERRE ONLY
For instance, under an epistemic reading of the modal operator $\Box$, we can express with an $\MLALCOud$ concept that \emph{of} Pierre it is \emph{known} that he is the General Chair of KR 2024:
\[
\exists u. ( \{ \mathsf{pierre} \} \sqcap \Box \{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \} ),
\]
while \emph{of} Pierre it is \emph{not} known that he is the General Chair of the KR Conference held in Southeast Asia:
%
\begin{multline*}
	\exists u. ( \{ \mathsf{pierre} \} \sqcap \lnot \Box  \{ \defdes \exists \mathsf{isGenChair}. \\
								 \{ \defdes ( \mathsf{KRConf} \sqcap \exists
\mathsf{hasLoc}.\mathsf{SEAsiaLoc}) \} \} ).
\end{multline*}

%%% EXAMPLE - NOT KNOWN THAT THE GC OF KR24 IS THE GC OF S-E ASIA KR
%{\color{blue}{%
%because, for instance, it is not known \emph{that} the General Chair of KR 2024 is the General Chair of the KR Conference held in Southeast Asia:
%\begin{multline*}
%	\lnot \Box \exists u. (  \{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \}  \sqcap \{ \defdes \exists \mathsf{isGenChair}. \\
%								 \{ \defdes ( \mathsf{KRConf} \sqcap \exists
%\mathsf{hasLoc}.\mathsf{SEAsiaLoc}) \} \} ).
%\end{multline*}
%}}





%%% NOT VALID ARGUMENT
%{\color{red}{
%\nb{M: working here}
%For instance, under an epistemic reading of the modal operator $\Box$, we can express with an $\MLALCOud$ concept that it is \emph{known} \emph{of} Pierre that he is busy:
%\[
%\exists u. ( \{ \mathsf{pierre} \} \sqcap \Box \mathsf{Busy}),
%\]
%while it is \emph{not known} \emph{that} the General Chair of KR 2024 is busy:
%%
%\[
%\lnot \Box \exists u. ( \{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \}  \sqcap \mathsf{Busy} ),
%\]
%because, for instance, it is \emph{not known} \emph{of} Pierre that he is the General Chair of KR 2024 :
%\[
%\exists u. ( \{ \mathsf{pierre} \} \sqcap \lnot \Box \{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \} ).
%\]
%}}



%%% ALTERNATIVE VERSION - BUSY GENERAL CHAIR KR24
%{\color{blue}{
%For instance, under an epistemic reading of the modal operator $\Box$, we can express with an $\MLALCOud$ concept that it is known \emph{that} the General Chair of KR 2024 is busy:
%\[
%\Box \exists u. ( \{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \} \sqcap \mathsf{Busy} ),
%\]
%while it is \emph{not} known \emph{of} the General Chair of KR 2024 that they are the General Chair of the KR Conference held in Southeast Asia:
%%
%\begin{multline*}
%	\exists u. ( \{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \} \sqcap \lnot \Box  \{ \defdes \exists \mathsf{isGenChair}. \\
%								 \{ \defdes ( \mathsf{KRConf} \sqcap \exists
%\mathsf{hasLoc}.\mathsf{SEAsiaLoc}) \} \} ).
%\end{multline*}
%}}

In a temporal setting, where $\Box$
%\nb{+ is not necessary}
is read as `always' and its dual $\Diamond$ as `at some point in the future,\!' KR 2024 can be made a rigid designator, which refers to the same object at all time instants. This can be achieved, for example, by means of an ontology that holds globally, at all time instants, and consists of the following concept inclusion (CI):
\[
	\{ \mathsf{kr24} \} \sqsubseteq \Box  \{ \mathsf{kr24} \}.
%	\quad \Diamond \{ \mathsf{kr24} \} \sqsubseteq \{ \mathsf{kr24} \}.
\]
%{\color{blue}{%
In contrast, we can use the nominal $\{ \mathsf{kr} \}$
%\nb{how is this related to KRConf above?}
to refer to the current edition of the KR Conference,
for instance 
stating that KR 2024 is the current KR Conference with the concept $\exists u. (\{\mathsf{kr24}\} \sqcap \{ \mathsf{kr} \})$.
Moreover, by reading $\Next$ as `next year',
we can exploit its lack of rigidity to express, e.g., that there will be \emph{other}
%different
KR Conferences in the future, with the CIs:
	\[
	\top \sqsubseteq \Diamond  \exists u. \{\mathsf{kr}\}, \qquad \{\mathsf{kr}\} \sqsubseteq \lnot \Next \{ \mathsf{kr} \}.
	\]
%	}}

%%% ALTERNATIVE VERSION -- NEXT YEAR'S KR
%In contrast, we can use the nominal $\{ \mathsf{kr} \}$ to refer to the current edition of the KR Conference, and
%(by reading $\Next$ as `next year')
%exploit its lack of rigidity to express, e.g., that the Program Chair of KR always becomes either the General Chair or a PC member of next year's KR,\nb{is next in the right place? \\ M: maybe not} with the CI:
%	\begin{multline*}
%\exists {\sf isProgChair}.\{ {\sf kr} \} \sqsubseteq \\
%							 \{ \defdes \exists {\sf isGenChair}. \Next \{ {\sf kr} \} \} \sqcup \exists {\sf isPCMember}. \Next \{ {\sf kr } \} ).
%	\end{multline*}

Compared
%\nb{re-read the paragraph}
to first-order modal logics
with non-rigid designators~\cite{StaTho68,FitMen12},
both the definition of the language and the scope distinctions
for
modal operators are simplified in modalised DLs,
as first-order variables are replaced by a class-based DL syntax  leaving quantification
and predicate abstraction
implicit.
We, however, show that 
our modal DLs can be translated to a natural fragment of first-order modal logic with definite descriptions and predicate abstraction.

In this work, we consider
interpretations with both constant domains (in which the first-order domain is fixed across all worlds) and expanding domains (in which it
%\nb{replaced `domain'}
can grow when moving 
to accessible worlds).
%from a world to an accessible world).
%
We
first
establish, for any class of Kripke frames and both constant and expanding domains, polytime  satisfiability-preserving reductions (with and without ontology)  to the language $\MLALCOu$ without definite descriptions. We will show that, in addition, we can assume that each nominal designates in every world, but importantly is still non-rigid.
%}

We
then
study
the satisfiability problem for various fundamental modal logics with epistemic and temporal interpretations. While for first-order modal logics with
%\nb{cut  `only'}
rigid designators and no counting the restriction to \emph{monodic} formulas (in which modal operators are  applied only to formulas with at most one
%\nb{replaced `only'}
free variable) very often ensures decidability, this is no longer the case if non-rigid designators
and/or
some counting are admitted~\cite{GabEtAl03}. For our modal DLs, this implies that the standard recipe for designing decidable languages --- apply modal operators only to concepts --- does not always work anymore.
Here,
we explore in detail when this recipe still works, and when it does not. 

First, we
%We first
closely link the two main sources of bad computational behaviour, non-rigid designators and counting, enabling us to use the results and machinery introduced
for first-order modal logics with counting~\cite{DBLP:conf/aiml/HampsonK12,HamKur15,DBLP:conf/aiml/Hampson16}.

Next, we prove that, rather surprisingly, for some fundamental modal epistemic logic, non-rigid designators come for free: concept satisfiability for the modal logics of all Kripke frames with $n$ accessibility relation, $\K^{n}$, and of all Kripke frames with $n$ equivalence relations, $\Sfive^{n}$, is in \NExpTime{} and thus no harder than without names at all. This holds under both  constant and expanding domains, and the proof is by showing the exponential finite model property. This answers an open problem discussed in~\cite{DBLP:conf/aiml/Hampson16}. With ontologies, however, concept satisfiability becomes undecidable under constant domains. While for $\Sfive^{n}$ (because of symmetric accessibility relations) constant domains coincide with expanding domains, for $\K^{n}$ decidability under expanding domains remains open with ontologies. As a fundamental example of an expressive modal logic, we investigate the extension $\K^{\ast n}$ of $\K^{n}$ with a modal operator interpreted by the transitive closure of the union of the $n$ accessibility relations, which can be interpreted as common knowledge~\cite{DBLP:books/mit/FHMV1995} but also as a fragment of propositional dynamic logic, PDL~\cite{DBLP:journals/sigact/HarelKT01}. In this case concept satisfiability is undecidable under expanding and constant domains, but becomes decidable, though Ackermann-hard, for the corresponding logic, $\Kfn$, on finite acyclic models with expanding domains. This answers an open problem posed in~\cite{WolZak01}.
 Note that Ackermann-hardness means that  the time required to establish (un)satisfiability is not bounded by any primitive recursive (or computable) function.
We refer the reader to Table~\ref{table:complexity} for an overview of our results. Recall that with rigid designators all these problems are known to be in 
%\nb{M: ?}
2\NExpTime~\cite{WolZak01,GabEtAl03}.

%\textcolor{red}{
Finally, in the temporal setting, we show that undecidability is a widespread phenomenon: concept satisfiability under global ontology with constant domain is undecidable for all our $\ALCO$-based fragments; the same applies to concept satisfiability in the languages with the universal modality and the temporal $\Diamond$ operator. 
Reasoning becomes decidable only when considering concept satisfiability (under global ontology) with expanding domains over finite flows of time (though the problem is Ackermann-hard),  or in fragments with  the  $\Next$ operator only, 
for which we prove \ExpTime{}-membership of  concept satisfiability (without ontologies).
%}

%\begin{table*}[t] % put at top of page if possible 
%	\centering
%	\begin{tabular}{l|c|c|c|c}
%		& \multicolumn{2}{c|}{concept satisfiability} &  \multicolumn{2}{c}{concept sat. under global ontology}\\
%		\mbox{}\hfil modal logic $L$ & const.\ domain & exp.\ domains & const.\ domain & exp.\ domains  \\
%		\hline
%		$\K^n$, $n \geq 1$ & NExp-c & NExp-c & undec. & ? \\[4pt]
%		$\Sfive$ & NExp-c & NExp-c & NExp-c & NExp-c \\
%		$\Sfive^{n}$, $n\geq 2$ & NExp-c & NExp-c & undec. & undec. \\[4pt]
%		%		$\KDfourfive$ & NExp-c & NExp-c & NExp-c & NExp-c \\
%	%	$\Kfour$ & ? & ? & ? & ?\\
%	%	$\Kfour^{n}, n\geq 2$ & ? & ? & undec. & ?\\[4pt]
%	%	$\GL$, $\Grz$ & ? & decidable & ? & decidable\\
%		%		$\K^{n}, n\geq 1$ & NExp-c & NExp-c & undec & undec. \\
%		%		$\KDfourfive_{n}, n\geq 2$ & NExp-c & NExp-c & undec & undec\\
%	%	$\GL^{n}$, $\Grz^{n}$, $n\geq 2$ & ? & dec & undec. & ? \\
%		$\K^{\ast n}$, $n\geq 1$ & undec. & undec. & undec. & undec. \\
%		$\Kfn$, $n\geq 1$ & undec. & dec., Ackermann-hard & undec. &  dec., Ackermann-hard
%		%        $\K^{n,\text{ftree},\ast}$, 
%	\end{tabular}
%	\caption{Concept satisfiability (under global ontology) for $L_{\ALCOud}$}\label{table:complexity}
%\end{table*}

\begin{table}[t] % put at top of page if possible 
\centering\tabcolsep=4pt%
\newcommand{\refr}[1]{~{\tiny[#1]}}%
	\begin{tabular}{lccc}\toprule
		\mbox{}\hfil modal  & \multirow{2}{*}{domain} & \multirow{2}{*}{concept sat.} &  concept sat.\\  
		\mbox{}\hfil logic $L$ & & & under global ont.\\
		\midrule
		\multirow{2}{*}{$\K^n$, $n \geq 1$} & const. & \textsc{NExp}-c.\refr{T~\ref{thm:modconcdec}} & undecidable\refr{T~\ref{thm:k:global:sat}}\\ & exp. &  \textsc{NExp}-c.\refr{T~\ref{thm:modconcdec}}   & ? \\[2pt]
		$\Sfive$ & ---& \multicolumn{2}{c}{\textsc{NExp}-complete\refr{T~\ref{thm:modconcdec}}} \\
		$\Sfive^{n}$, $n\geq 2$ & --- & \textsc{NExp}-c.\refr{T~\ref{thm:modconcdec}} & undecidable\refr{T~\ref{thm:k:global:sat}} \\[2pt]
		\multirow{2}{*}{$\K^{\ast n}$, $n\geq 1$} & const. & \multicolumn{2}{c}{$\Sigma^{1}_{1}$-complete\refr{L~\ref{lemma:ltl-to-kfn} + T~\ref{th:temp1:const}}} \\ 
		& exp. & \multicolumn{2}{c}{undecidable\refr{L~\ref{lemma:ltl-to-kfn} + T~\ref{th:temp1:exp}.1}}  \\[2pt]
		\multirow{2}{*}{$\Kfn$, $n\geq 1$} & const. & \multicolumn{2}{c}{undecidable\refr{L~\ref{lemma:ltl-to-kfn} + T~\ref{th:temp1:const}}} \\
		  &  exp. & \multicolumn{2}{c}{\begin{tabular}{c}decidable\refr{T~\ref{thm:moddickson}},\\[-2pt]Ackermann-hard\refr{L~\ref{lemma:ltl-to-kfn} + T~\ref{th:temp1:exp}.2}\end{tabular}}\\\bottomrule
	\end{tabular}
	\caption{Concept satisfiability (under global ontology) for $L_{\ALCOud}$}\label{table:complexity}
\end{table}

%{\color{red}
It is to be emphasised that the non-rigidity of symbol interpretation by itself is \emph{not} the cause for the satisfiability problem to become harder. For instance, 
rigid roles are known to often cause %harder satisfaction problems than non-rigid roles
an increase in the hardness of
the satisfiability problem compared with the case of non-rigid roles only~\cite{GabEtAl03}. What makes non-rigid designators computationally much harder than rigid designators is their ability to count in an unbounded way across worlds.
%}

The full version of the paper with proofs and additional material is available on ArXiv~\cite{ArtEtAl24}.


\paragraph{Related Work}

Other than in non-modal DLs~\cite{NeuEtAl20,ArtEtAl20b,ArtEtAl21a}, and  in the already mentioned \emph{first-order} modal and temporal settings,
%~\cite{RepeatFOMLStuff?},
definite descriptions have been recently investigated in the context of \emph{propositional} hybrid logics with nominals and the $@$ operator~\cite{WalZaw23}. Here, the additional $\defdes$ operator allows one to refer to the (one and only) state of a model that satisfies a certain condition.
%\nb{M: todo fix refs}

Non-rigid designators have received, to the best of our knowledge, little attention in modal DLs,
despite the extensive body of research both on temporal~\cite{WolZak98,ArtFra05,LutEtAl08,ArtEtAl14} and epistemic~\cite{DonEtAl98,ArtEtAl07a,CalEtAl08,ConLen20} extensions.
As a notable exception, \citeauthor{MehRud11}~(\citeyear{MehRud11}) investigate non-rigid individual names  in an epistemic DL context,  
where
abstract individual names are interpreted on an infinite common domain, but without definite descriptions.
%A notable  exception is~\cite{MehRud11}, involving non-rigid ``abstract'' individual names interpreted on an infinite common domain, and without definite descriptions).
%DonEtAl92,CalEtAl06
%%definite descriptions and
%In an epistemic DL context, non-rigid individual names appear in~\cite{MehRud11}, under an approach that involves abstract individual names interpreted on an infinite common domain, but without definite descriptions.

%In this paper, we extend the free DLs proposed for the non-modal case
%in~\cite{ArtEtAl20b,ArtEtAl21a}, by: (i) adding \emph{epistemic
%  modalities}, such as $\Box$ (\emph{box}, read as `it is known
%that'), or \emph{temporal} ones, like $\Until$ (\emph{until}),
%applicable both to formulas\nb{A:use DL terminology, TBox or KB axioms?} and concepts of the language; (ii)
%introducing nominals built from \emph{definite descriptions} of the
%form $\iota C$ (read as `the object that is $C$'), where $C$ is a
%concept, alongside the standard ones based on \emph{individual names};
%%like $a$;
%(iii) dropping the \emph{rigid designator assumption}, hence allowing
%terms to behave as flexible individual concepts across states.  We
%study the complexity of formula satisfiability, showing that, without
%the rigid designator assumption, this problem for epistemic free DLs
%is $\NExpTime$-complete (same as the logic \Sfivee~\cite[Theorem
%5.26]{GabEtAl03}), whereas it becomes undecidable for temporal free
%DLs interpreted on linear time structures (while
%%\nb{A: added}
%it is
%decidable without definite descriptions and with the RDA~\cite[Theorem
%14.12]{GabEtAl03}).

%Section~\ref{subsec:ml-nonrig} provides the necessary background on
%modal free DLs.
%%In Section~\ref{sec:motivation}, we motivate with examples the syntactical and semantical choices for these languages.
%In Section~\ref{sec:reduction}, we define the reasoning problems studied in this paper and provide basic observations and reductions, and Section~\ref{sec:counting} draws the connection with the one-variable fragment of first-order modal logic with counting.
%Then, Section~\ref{sec:reasoning} studies the complexity of
%reasoning in epistemic free DLs, while
%Section~\ref{sec:reasontfdl} focuses on temporal
%free DLs over time flows consisting of finite or infinite traces.
%Finally, in Section~\ref{sec:conc}, we discuss open
%problems and future research directions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "rda"
%%% End:


==> camera-ready/2-preliminaries.tex <==
% !TEX root =  rda.tex

%\section{Epistemic and Temporal Free Description Logics}
%\label{sec:tdlnonrig}

%We introduce $\MLALCOud$ and $\TLALCOud$, epistemic and, respectively,
%temporal extensions of the free description logic
%$\ALCOud$~\cite{ArtEtAl20b,ArtEtAl21a}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}
%\section{Modal Free Description Logics}
\label{subsec:ml-nonrig}

The
$\MLALCOud$
language
is a modalised extension of the free description logic (DL)
$\ALCOud$~\cite{ArtEtAl20b,ArtEtAl21a}.
%
% \begin{definition}[$\TLALCOud$ syntax]
Let \NC, \NR and \NI be countably infinite and pairwise disjoint sets
of \emph{concept names}, \emph{role names} and \emph{individual names}, respectively, and let $I = \{ 1, \ldots, n \}$ be a finite set of \emph{modalities}.
$\MLALCOud$ \emph{terms} and
\emph{concepts} are defined by the following grammar:
%
\begin{gather*}
  \tau ::= a \mid \defdes C,
  \\
  C ::= A \mid \{ \tau \} \mid \lnot
  C \mid (C \sqcap C)
%\mid \exists_{\mathop{\geq n}} r.C
\mid \exists r.C
\mid \exists u.C
\mid \Diamond_{i} C,
%\mid (C \Until C),
\end{gather*}
%
where $a \in \NI$, $A \in \NC$, $r \in \NR$,
%\nb{rigid roles? \\ M: perche' rigid? non direi}
 $u\notin \NR$ is the
\emph{universal role}, and $\Diamond_{i}$, with $i \in I$, is a \emph{diamond} operator.
%
A term of the form $\defdes C$ is called a \emph{definite
  description} and
%  \nb{shortened}
  $C$ its \emph{body}; a concept $\{ \tau \}$ is called a \emph{\textup{(}term\textup{)}
  nominal}. All the usual syntactic abbreviations are assumed:
%In particular,
$\bot = A \sqcap \lnot A$, $\top = \lnot \bot$,
$C \sqcup D = \lnot (\lnot C \sqcap \lnot D)$,
$C \Rightarrow D = \lnot C \sqcup D$,
$C \Leftrightarrow D = (C \Rightarrow D) \sqcap (D \Rightarrow C)$,
$\forall s. C = \lnot \exists s. \lnot C$, for
$s \in \NR \cup \{ u \}$, and \emph{box} operator $\Box_{i} C = \lnot \Diamond_{i} \lnot C$.
%We
%also consider the \emph{reflexive diamond} operator,
%$\Diamond_{i}^{+} C = C \sqcup \Diamond_{i} C$, and the \emph{reflexive box}
%operator, $\Box_{i}^{+} C = \neg\Diamond_i^+\neg C$. %C \sqcap \Box_{i} C$.
%
A \emph{concept inclusion} (\emph{CI}) is of the form $C \sqsubseteq D$,
%or an \emph{$\MLALCOud$ assertion} of the form $C(\tau)$ or
%$r(\tau_1,\tau_2)$, 
for  concepts $C, D$.  We  use $C \equiv D$ to abbreviate $C \sqsubseteq D$ and $D \sqsubseteq C$.
An \emph{ontology} $\Omc$ is a finite set of CIs.

Fragments
$\ML^n_{\ALCOu}$, $\ML^n_{\ALCOd}$, and $\ML^n_{\ALCO}$ of  the full language are defined by restricting the
available DL constructors: they do not contain, respectively, definite descriptions, the universal role, and both 
definite descriptions and the universal role.


Given a concept $C$, the
set of \emph{subconcepts} of $C$, denoted by $\sub{C}$, is defined as usual
(see Appendix~A in the full version):
%\footnote{
%The full version of the paper with proofs and additional material is available on ArXiv~\cite{ArtEtAl24}.}
we only note that 
$\sub{\{\defdes C\}}$ contains $C$ along with its own subconcepts.
% 
%inductively as follows.
%For $C = A$ and $C = \{ a \}$, we set $\sub{C} = \{ C \}$.
%For $C = \lnot D$, $C = \{ \defdes D \}$, and $C = \exists s. D$, with $s \in \NR \cup \{ u \}$, and $C = \Diamond_{i} D$, we set $\sub{C} = \{ C \} \cup \sub{D}$.
%For $C = D \sqcap E$, we set $\sub{C} = \sub{D} \cup \sub{E}$.
%}}
The \emph{signature} of $C$, denoted by~$\Sigma_{C}$, is the set of concept, role and individual names in~$C$. The signature of a CI or an ontology is defined similarly.
The set of \emph{connectives} of an ontology $\Omc$ is the constructors from the following list that occur in $\Omc$: $\defdes$, $\{ \cdot \}$, $\lnot$, $\sqcap$, $\exists$ with roles in $\NR$, $\exists u$, and $\Diamond_{i}$ with $i\in I$.
%
The \emph{modal depth} of terms and concepts is the maximum number of nested modal operators: $\md(A) = 0$, $\md(\defdes C) = \md(C)$ and $md(\Diamond_{i} C)  = \md(C) + 1$, for example.
%defined by mutual induction:
%%
%\begin{align*}
%\md(a) & = 0, & \md(\defdes C) & = \md(C), \\
%\md(A) & = 0,  &  \md(\{ \tau \}) & = \md(\tau), \\
%\md(\lnot C) & = \md(C), \hspace*{-20em}\\
%\md(C \sqcap D) & = \max\{ \md(C), \md(D) \}, \hspace*{-20em}\\
%\md(\exists s.C) & = \md(C), \ \text{with $s \in \NR \cup \{ u \}$}, \hspace*{-20em}\\
%\md(\Diamond_{i} C) & = \md(C) + 1. \hspace*{-20em}
%%\md(C \sqsubseteq D) & = \max\{ \md(C), \md(D) \}, \hspace*{-20em}\\
%%\md(\Omc) & = \max\{ \md(C \sqsubseteq D) \ | \ C \sqsubseteq D \in \Omc \}. \hspace*{-20em}
%\end{align*}
%
The \emph{modal depth} of a CI or an ontology is the maximum modal depth of their concepts.




%
%An \emph{$\MLALCOud$ formula} is an expression of the following form:
%
%\[
%\p ::=
%(\alpha)
%\mid \neg \p \mid (\p \land \p)
%\mid \Diamond_{i} \p.
%\]
%%
%\ifshort
%Let \NC, \NR and \NI be countably infinite and pairwise
%disjoint sets of \emph{concept names}, \emph{role names}, and
%\emph{individual names}, respectively. The
%$\SfiveALCOud$  \emph{concepts} and \emph{formulas} are defined as:
%%
%\begin{align*}
% C ::= A \mid \{ \tau \} \mid \lnot
%  C \mid C \sqcap C
%%\mid \exists_{\mathop{\geq n}} r.C
%\mid \exists r.C
%\mid \exists u.C
%  \mid \Diamond C,
%  \qquad
%\p ::=
%(\alpha)
%\mid \neg \p \mid \p \land \p
%\mid \Diamond \p,
%%\mid (C \Until C),
%\end{align*}
%%
%where
% $\tau ::= a \mid \defdes C$ is an 
% \emph{$\SfiveALCOud$ term}, 
% $a \in \NI$, $A \in \NC$, $r \in \NR$,
%% \nb{rigid roles? \\ M: perche' rigid? non direi},
%$u$ is the \emph{universal role} and $\alpha$ is an
%\emph{$\MLALCOud$ axiom},
%denoting either a \emph{concept inclusion} (\emph{CI}) of
%the form $C \sqsubseteq D$, or an
%\emph{$\MLALCOud$ assertion}
%of the
%form $C(\tau)$ or $r(\tau_1,\tau_2)$, where $C, D$ are concepts,
%$r \in \NR$, and $\tau, \tau_1, \tau_2$ are terms.
%%
%A term of the form $\defdes C$ is called a \emph{definite
%  description},
%  with the concept $C$ being the \emph{body of
%  $\defdes C$},
%  and a concept $\{ \tau \}$ is a \emph{(term)
%  nominal}.
%  All the usual syntactic abbreviations are assumed.  In
%particular, we will consider also the \emph{reflexive diamond}
%operator, $\Diamond^{+} C = C \sqcup \Diamond C$, the \emph{box} operator, $\Box C = \lnot \Diamond \lnot C$, and the
%\emph{reflexive box} operator, $\Box^{+} C = C \sqcap \Box C$.
%%%
%% An \emph{$\MLALCOud$ formula} is an expression of the following form:
%% %
%% \[
%% \p ::=
%% (\alpha)
%% \mid \neg \p \mid \p \land \p
%% \mid \Diamond \p
%% \]
%\fi




%The
%set of concepts occurring in~$\Omc$ is denoted by $\con{\Omc}$, and the
%set of individual names occurring in $\Omc$ is denoted by $\ind{\Omc}$.


A \emph{frame} is a pair $\Fmf = (W, \{ R_{i} \}_{i \in I})$, where $W$ is a non-empty set of \emph{worlds} (or \emph{states}) and each
\mbox{$R_{i} \subseteq W \times W$}, for $i\in I$, is a binary \emph{accessibility relation} on $W$.
%
%%% VERSION EXPANDING DOMAINS
A \emph{partial interpretation with expanding domains} based on
a frame $\Fmf = (W, \{ R_{i} \}_{i \in I} )$ is a triple $\Mmf = ( \Fmf, \Delta, \Int)$, where
%$\Fmf$ is the frame of $\Mmf$;
$\Delta$ is a function associating with every $w \in W$ a non-empty set, $\Delta^{w}$, called the \emph{domain of $w$ in~$\Mmf$}, such that $\Delta^{w} \subseteq \Delta^{v}$, whenever $w R_{i} v$,
%\nb{slight renaming to avoid confusion with $u$}
for some $i \in I$;
and $\Int$ is a function associating with every $w \in W$ a
  \emph{partial} DL interpretation
  $\Imc_{w} = (\Delta^{w}, \cdot^{\Imc_{w}})$ that maps every
  $A \in \NC$ to a subset $A^{\Imc_{w}}$ of~$\Delta^{w}$, every
  $r\in\NR$ to a subset $r^{\Imc_{w}}$ of
  $\Delta^{w} \times \Delta^{w}$, the universal role $u$ to the set
  $\Delta^{w} \times \Delta^{w}$, and every $a$ in \emph{some
  subset} of $\NI$ to an element $a^{{\Imc_{w}}}$ in
  $\Delta^{w}$.
Hence, every
$\cdot^{\Imc_{w}}$ is a total function on $\NC \cup \NR$ but a
\emph{partial} function on~$\NI$. If $\Imc_{w}$ is defined on $a\in\NI$, then we say
that $a$ \emph{designates at~$w$}.
If every $a\in\NI$ designates at $w\in W$, then $\Imc_{w}$ is called \emph{total}.
%
We say that $\Mmf = ( \Fmf, \Delta, \Int)$ is a \emph{total} 
  interpretation if every $\Imc_{w}$, 
$w \in W$, is a \emph{total} interpretation.
In the sequel, we refer to partial interpretations as interpretations, and add the adjective `total' explicitly whenever this is the case.


%%% VERSION CONSTANT DOMAIN
%A \emph{partial modal interpretation} based on
%$\Fmf$ is a triple $\Mmf = ( \Fmf, \Delta, \Int)$, where: $\Fmf$ is
%the frame of $\Mmf$; $\Delta$ is a non-empty set, called the
%\emph{domain} of $\Mmf$ (we adopt the so-called \emph{constant domain
%  assumption}~\cite{GabEtAl03}); and $\Int$ is a function associating
%with every $w \in W$ a \emph{partial interpretation}
%$\Imc_{w} = (\Delta, \cdot^{\Imc_{w}})$ that maps every $A \in \NC$ to
%a subset of $\Delta$, every $r\in\NR$ to a subset of
%$\Delta \times \Delta$, the universal role $u$ to the set
%$\Delta \times \Delta$ itself, and every $a$ in a \emph{subset} of
%$\NI$ to an element in $\Delta$. In other words, every
%$\cdot^{\Imc_{w}}$ is a total function on $\NC \cup \NR$ and a
%\emph{partia}l function on $\NI$.
%%
%We say that
%$\Mmf = ( \Fmf, \Delta, \Int)$ is a \emph{total modal
%  interpretation} if every $\Imc_{w}$, with $w \in W$, is a \emph{total}
%interpretation,
%meaning that $\cdot^{\Imc_{w}}$ is defined as above, except that it maps \emph{every} $a \in \NI$ to an element of $\Delta$.



An \emph{interpretation with constant domains} is defined as a special case% of interpretation with expanding domains
, where the function $\Delta$ is such that $\Delta^{w} = \Delta^{v}$, for every $w, v \in W$. With an abuse of notation, we denote the common domain by $\Delta$ and call it the \emph{domain of $\Mmf$}.
%We observe that partial modal interpretations with constant domain can be seen a special case of partial modal interpretations with expanding domains, with the function $\Delta$ assigning to every $w \in W$ the \emph{same} domain $\Delta^{w}$.
%\end{definition}


Given $\Mmf = (\Fmf, \Delta, \Int)$, with
$\Fmf = (W, \{ R_{i} \}_{i \in I})$, we define the \emph{value}
$\tau^{\Int_{w}}$ of a term $\tau$ in world $w\in W$ as $a^{\Int_{w}}$, for
$\tau = a$, and as follows, for $\tau = \defdes C$:
%
\begin{gather*}
		(\defdes C)^{\Int_{w}}  =
			\begin{cases}
				d, & \text{if} \ C^{\Int_{w}} = \{ d \}, \ \text{for some} \ d \in \Delta^{w}; \\
				\text{undefined}, & \text{otherwise}.
			\end{cases}
\end{gather*}
%
A term $\tau$ is said to
\emph{designate at $w$}
%be \emph{denoting at $w$}
if $\tau^{\Int_{w}}$ is defined.
%$\tau^{\Int_{w}} = d$, for some $d\in\Delta$, 
%and to
%%$\tau^{\Int_{w}} = \{d\}$, for some $d\in\Delta$,
%\emph{designate in $\Mmf$}
%be \emph{denoting in $\Mmf$}
%if $\tau$
%designates\nb{do we use it at all?}
%is denoting
%at some $w\in W$.  
%Moreover, an individual name $a$ is called a \emph{ghost
%  in} $\Mmf$ if, for every $w\in W$, $a$ does not denote at
%$w$.\nb{F: don't like ghost}
%
The
\emph{extension} $C^{\Int_{w}}$ of a concept $C$ in $w\in W$ is defined
as
follows, where $s \in \NR \cup \{ u \}$:
%
\begin{align*}
	(\neg C)^{\Int_{w}} & = \Delta^{w} \setminus C^{\Int_{w}}, \\ 
	(C \sqcap D)^{\Int_{w}} & = C^{\Int_{w}} \cap D^{\Int_{w}}, \\
	(\exists s.C)^{\Int_{w}} & = \{d \in \Delta^{w} \mid \exists  e \in C^{\Int_{w}}: (d,e) \in s^{\Int_{w}}\}, \\
  	(\Diamond_{i} C)^{\Imc_{w}} &= \bigl\{ d \in \Delta^{w}  \mid \exists 
  v \in W :
  w R_{i} v \text{ and } d \in C^{\Imc_{v}}
  \bigr\},
  \\
  %
  \{ \tau \}^{\Imc_{w}} &=
			\begin{cases}
				\{ \tau^{\Imc_{w}} \}, & \text{if $\tau$ designates at $w$}, \\
%				\text{if $\tau$ is denoting at $w$}, \\
				\, \emptyset, & \text{otherwise.}
			\end{cases}
\end{align*}
%
%where a term $\tau$ is said to \emph{denote} in $\Imc_{w}$ if
%$\tau^{\Imc_{w}}$ is defined.
%
A concept $C$ is \emph{satisfied at $w\in W$ in $\Mmf$} if
$C^{\Imc_{w}} \neq \eset$; $C$ is \emph{satisfied in $\Mmf$} if it is satisfied at some $w\in W$ in $\Mmf$.  % and it is \emph{satisfiable} if there is a
% partial modal interpretation $\Mmf$ and a world $w$ of $\Mmf$ such
% that $C$ is satisfied at $w$ of $\Mmf$.
%
%An
%\ifshort
%\emph{$\SfiveALCOud$ formula $\p$ is satisfied at $w$ of $\Mmf$},
%\fi
%\ifappendix
%\emph{$\MLALCOud$ formula $\p$ is satisfied at $w$ of $\Mmf$},
%\fi
%  written $\Mmf, w \models \p$, when:
%% in $\ALCOud$, but relative to the world $w$ of $\Mmf$ and with the following additional clause:
%%
%\begin{align*}
%	\Mmf, w \models C\sqsubseteq D  &\text{ \, iff \, } C^{\Imc_{w}} \subseteq D^{\Imc_{w}}, \\
%	\Mmf, w  \models C(\tau) &\text{ \, iff \, } \tau ~\text{denotes in}~{\Imc_{w}} ~\text{and}~\tau^{\Imc_{w}}\in C^{\Imc_{w}},\\
%	\Mmf, w \models r(\tau_1,\tau_2) &\text{ \, iff \, }
%        \tau_1,\tau_2 ~ \text{denote in} ~ {\Imc_{w}} ~ \text{and} \\
%        &  \ \qquad (\tau_1^{\Imc_{w}},\tau_2^{\Imc_{w}}) \in r^{\Imc_{w}}, \\
%%	\Mmf, w  \models \neg \p \text{ \, iff \, } \Mmf, w  \not \models \p, \qquad
%%	\Mmf, w  \models \p \land \psi \text{ \, iff \, } \Mmf, w  \models \p \text{ and } \Mmf, w  \models \psi, \\
%%	\Mmf, t  \models \p \Until \psi \text{ \, iff \, } \exists u \in T, t < u \colon \Mmf, u \models \psi \text{ and } \forall v \in (t,u) \colon \Mmf, v \models \p
%	\Mmf, w  \models \Diamond \psi  &\text{ \, iff \, } \exists v \in W,
%	w R_{i} v \colon \Mmf, v \models \psi,
% \end{align*}
% %
% together with the usual interpretation of Boolean operators.
% An
% $\MLALCOud$ formula $\p$  (resp., concept $C$) is \emph{satisfied} in a (partial or total) {modal interpretation $\Mmf$} if there
% exists a world $w$ in $\Mmf$ such that
% $\p$ is satisfied at $w$ of $\Mmf$ (resp., $C$ is satisfied at $w$ of $\Mmf$).
%% $\Mmf, w \models \p$  (resp., $C^{\Imc_{w}} \neq \emptyset$).
%% and it  is \emph{partial} (resp., \emph{total}) \emph{satisfiable} if there is a partial (resp., total) modal interpretation $\Mmf$ such that $\p$ is satisfied in $\Mmf$.
A CI $C \sqsubseteq D$ is \emph{satisfied in~$\Mmf$}, written $\Mmf\models C\sqsubseteq D$, if 
%
$C^{\Imc_{w}} \subseteq D^{\Imc_{w}}$, for every $w\in W$. An ontology $\Omc$ is \emph{satisfied in $\Mmf$}, written $\Mmf\models \Omc$, if every CI in $\Omc$ is satisfied in $\Mmf$; we also say a concept $C$ is \emph{satisfied in $\Mmf$ under an ontology~$\Omc$}
if $\Mmf\models \Omc$ and $C^{\Imc_w} \neq \emptyset$, for some $w\in W$. 
% 




An ontology $\Omc'$ is called a
\emph{model conservative extension} of an ontology $\Omc$ if every  interpretation that satisfies $\Omc'$ also satisfies $\Omc$, and every interpretation that satisfies $\Omc$ can be turned to satisfy $\Omc'$ by modifying the interpretation of symbols in $\sig{\Omc'} \setminus \sig{\Omc}$, while keeping fixed the interpretation of symbols in $\sig{\Omc}$.
Similarly, a concept $C'$ is said to be a \emph{model conservative extension} of a concept $C$ if every interpretation that satisfies $C'$ also satisfies $C$, and every interpretation satisfying $C$ can be turned into an interpretation that satisfies $C'$, by modifying the interpretation of symbols in $\sig{C'} \setminus \sig{C}$, while keeping fixed the interpretation of symbols in $\sig{C}$.








%{\color{red} formula satisfiability = concept satisfiability: use the universal role and nominals - $\varphi$ is satisfied in $\Mmf$ at $w$ iff $\forall u.\varphi^\dagger$ is satisfied in $\Mmf$ at $w$, where $\cdot^\dagger$ replaces $\land$ with $\sqcap$, etc. and $C \sqsubseteq D$ with $\forall u.(C \Rightarrow D)$, $A(a)$ with $\{a\} \Rightarrow A$ and $r(a,b)$ with $\{a\} \Rightarrow \exists r.\{b\}$}
%\nb{M: here we have to be a bit careful with assertions, see Remark~\ref{rem:assertion} below}
%
%{\color{red} concept satisfiability under global ontology = global CIs + local CIs + ABox satisfiability (in temporal case; does it have any meaning in the modal setting?): internalise the conjunction  of local CIs $ \mathcal{T}_L$ and ABox $\mathcal{A}$  using $\cdot^\dagger$ defined above as $C$, then $(\mathcal{T}_G \cup \mathcal{T}_L, \mathcal{A})$ is satisfied in $\Mmf$ at $0$ iff $C$ is satisfied in $\Mmf$ at 0 and $\mathcal{T}_G$ is satisfied in $\Mmf$ (globally)}



%{\color{red} F: I believe the syntax and reasoning problems have to be reduced: let's only introduce concepts and CIs. CIs are always interpreted globally.
%Two decision problems: 
%\begin{itemize}
%	\item concept satisfiability (complement of CI validity)
%	\item concept satisfiability under global ontology (complement of CI validity under global ontology)
%\end{itemize}
%Drop formulas and drop assertions and only global CIs. Then add discussion about expressivity.} 

%An $\MLALCOud$ ontology $\Omc$ is \emph{satisfied} in a (partial or total) {modal interpretation $\Mmf$} if there exists a world $w$ in $\Mmf$ such that every CI in $\Omc$ is satisfied at $w$ of $\Mmf$,
%and it is \emph{globally satisfied} in $\Mmf$ if every CI in $\Omc$ is satisfied at every $v$ of $\Mmf$.
%% 
%Moreover, an $\MLALCOud$ formula $\p$ is \emph{entailed under an $\MLALCOud$ ontology $\Omc$} (with respect to partial or total modal interpretations, respectively), written $\Omc \models \p$, if,
%for every partial (resp., total) modal interpretation $\Mmf$ and every $w$ of $\Mmf$, we have that $\p$ is satisfied at $w$ of $\Mmf$ whenever $\Omc$ is satisfied at $w$ of $\Mmf$.
%%every partial (resp., total) modal interpretation $\Mmf = (\Fmf, \Delta, \Imc)$ that satisfies $\p$ at $w$ satisfies also $\psi$ at $w$, for every $w$ in $\Fmf$.
%Finally, we say that $\p$ is \emph{entailed under a global $\MLALCOud$ ontology $\Omc$} (with respect to partial or total modal interpretations, respectively), written $\Omc \models^{\ast} \p$, if, for every partial (resp., total) modal interpretation
%$\Mmf$ 
%and every $w$ of $\Mmf$, we have that $\p$ is satisfied at $w$ of $\Mmf$, whenever $\Omc$ is satisfied at every $v$ of $\Mmf$.
%%Finally, an $\MLALCOud$ formula $\p$ \emph{partially} (resp., \emph{totally}) \emph{entails} an $\MLALCOud$ formula $\psi$, written $\p \models \psi$, if,
%%for every partial (resp., total) modal interpretation $\Mmf$ and every $w$ of $\Mmf$, we have that $\psi$ is satisfied at $w$ whenever $\p$ is satisfied at $w$.
%%%every partial (resp., total) modal interpretation $\Mmf = (\Fmf, \Delta, \Imc)$ that satisfies $\p$ at $w$ satisfies also $\psi$ at $w$, for every $w$ in $\Fmf$.
%%Instead, we say that $\psi$ is \emph{partially} (resp., \emph{totally}) \emph{entailed under a global formula $\p$}, written $\p \models^{\ast} \psi$, if, for every partial (resp., total) modal interpretation
%%$\Mmf = (\Fmf, \Delta, \Imc)$ 
%%and every $w$ in $\Fmf$, we have that $\psi$ is satisfied at $w$ of $\Mmf$, whenever $\p$ is satisfied at $v$ of $\Mmf$, for every $v$ in $\Mmf$.
%%\nb{M: todo change}
%%Finally, given a KB $\Kmc$, we say that $\Kmc$ is \emph{satisfied} in $\Mmf$ if, for each CI $\alpha \in \Kmc$, it holds that $\Mmf, w \models \alpha$, for every $w \in W$ (that is, $\alpha$ is \emph{globally} \emph{satisfied} in $\Mmf$).
%%If if there is a partial (total) modal interpretation $\Mmf$ such that $\Kmc$ is satisfied in $\Mmf$,  we say that $\Kmc$ is \emph{partial} (\emph{total}) \emph{satisfiable}.
 
%\subsubsection{Expanding Domains}
% 
% 
% A \emph{partial modal interpretation with expanding domains} based on
%$n$-frame $\Fmf = (W, \{ R_{i} \}_{i \in I} )$ is (with an abuse of notation) a triple $\Mmf = ( \Fmf, \Delta, \Int)$, where:
%$\Fmf$ is the frame of $\Mmf$;
%$\Delta$ is function associating with every $w \in W$ a non-empty set, $\Delta^{w}$, called the \emph{domain of $w$} in $\Mmf$, such that $\Delta^{v} \subseteq \Delta^{u}$, whenever $v R_{i} u$, for some $i \in I$;
%and $\Int$ is a function associating with every $w \in W$ a \emph{partial interpretation}
%$\Imc_{w} = (\Delta^{w}, \cdot^{\Imc_{w}})$ that maps
%every $A \in \NC$ to
%a subset of $\Delta^{w}$,
%every $r\in\NR$ to a subset of
%$\Delta^{w} \times \Delta^{w}$,
%the universal role $u$ to the set
%$\Delta^{w} \times \Delta^{w}$ itself,
%and every $a$ in a \emph{subset} of
%$\NI$ to an element in $\Delta^{w}$.
%In other words, every
%$\cdot^{\Imc_{w}}$ is a total function on $\NC \cup \NR$ and a
%\emph{partia}l function on $\NI$.
%%
%We say that
%$\Mmf = ( \Fmf, \Delta, \Int)$ is a \emph{total modal interpretation with expanding domains} if every $\Imc_{w}$, with $w \in W$, is a \emph{total}
%interpretation, meaning that $\cdot^{\Imc_{w}}$ is defined as above, except that it maps \emph{every} $a \in \NI$ to an element of $\Delta^{w}$.
%
%All the other semantic definitions are given similarly to the constant domain case. We observe that partial modal interpretations with constant domain can be seen a special case of partial modal interpretations with expanding domains, with the function $\Delta$ assigning to every $w \in W$ the \emph{same} domain $\Delta^{w}$.
 
 
 
 
 
 
 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Temporal Free Description Logics}

%{\color{red} F: Emphasize and use that this is an instance of $\MLALCOud$: without next we have one modal operator, the frames are $(\mathbb{N}, <)$, where $<$ is the natural strict
%	linear order on $\mathbb{N}$ and $(\{0, \ldots, n \}, <)$. With next we have two modal operators, next interpreted by the successor relation.
%	Then we can just introduce a few abbreviations we use for this special case.}



%%% VERSION CONSTANT DOMAIN
%We call \emph{flow of time} a frame $\Fmf = (T, <)$, where $T$ is a
%non-empty set of \emph{instants} and $< \ \subseteq T \times T$ is a
%strict linear order on $T$.  A \emph{partial temporal interpretation},
%or \emph{partial trace}, based on a flow of time $\Fmf$, is a triple
%$\Mmf = ( \Fmf, \Delta, \Int)$, defined as in the modal case.  We
%similarly define the notion of \emph{total trace}.  If $\Mmf$ is based
%on the flow of time $(\mathbb{N}, <)$, where $<$ is the natural strict
%linear order on $\mathbb{N}$, we call it an \emph{infinite trace}, and
%we often denote it (with an abuse of notation) by
%$\Mmf = (\Delta, (\Imc_{t})_{t \in \mathbb{N}})$; whereas, if it is
%based on $(\{0, \ldots, n \}, <)$, with $n \in \mathbb{N}$, it is
%called a \emph{finite trace}, and it is simply denoted by
%$\Mmf = (\Delta, (\Imc_{t})_{t \in T})$, with $T = [0, n]$.
%%We call \emph{flow of time} a frame $\Fmf = (T, <)$, with
%%$T \in \{ \mathbb{N} \} \cup \bigcup_{n \in \mathbb{N}} \{ \{ 0,
%%\ldots, n \} \}$, where $\mathbb{N}$ is the set of non-negative
%%integers, the elements of $T$ are called \emph{instants} and
%%$< \ \subseteq T \times T$ is the natural strict linear order on $T$.
%%A \emph{partial temporal interpretation}, or \emph{trace}, based on a
%%flow of time $\Fmf$ is a triple $\Mmf = ( \Fmf, \Delta, \Int)$, as
%%defined for the modal case.
%%%
%%If $\Mmf$ is based on the flow of time $(\mathbb{N}, <)$, we call it
%%an \emph{infinite trace}; whereas, if it is based on
%%$(\{0, \ldots, n \}, <)$, with $n \in \mathbb{N}$, it is called a
%%\emph{finite trace}.
%%Moreover, given a $k \in \mathbb{N}$, we call a \emph{$k$-bounded
%%trace} any finite trace based on $(\{0, \ldots, m \}, <)$, with $m
%%\leq k$.
%%



%\subsection{Constant Domain Assumption}

%\begin{definition}










\begin{remark}[Encoding of assertions]\em
\label{rem:assertion}
Assertions can be introduced as syntactic sugar using the universal role, with $C(\tau)$ and  $r(\tau_1,\tau_2)$ abbreviations for, respectively, concepts
%\nb{more Pierre-like}
%
\begin{equation*}
   \exists u. (\{ \tau \} \sqcap  C) \text{ and }
   \exists u. (\{ \tau_{1} \} \sqcap \exists r.\{ \tau_{2} \}).
%  & \exists u. \{ \tau \} \sqcap \forall u. ( \{ \tau \} \Rightarrow C),\\
%  & \exists u. \{ \tau_{1} \} \sqcap \forall u. (\{ \tau_{1} \} \Rightarrow \exists r.\{ \tau_{2} \}).
\end{equation*}
%
The first example in Sec.~\ref{sec:intro} is thus $\mathsf{isGenChair}(\mathsf{pierre}, \mathsf{kr24})$.
%Thus,~our~first~example~in~Section~\ref{sec:intro}~is~$\mathsf{isGenChair}(\mathsf{pierre}, \mathsf{kr24})$.
%the
%%first
%example
%in Section~\ref{sec:intro}
%%above
%
%In addition, \emph{local} \nb{M: move to Appendix} CIs, that is, CIs that
%%\nb{ok? \\ M: ok}
%are true at a particular world rather than at all worlds (as the CIs in our ontologies), 
%%(i.e., CIs evaluated at a single world)
%%and ontologies
%can be \emph{internalised}~\cite[Chapter~5]{BaaEtAl03a} into concepts, by replacing CI $C \sqsubseteq D$ with concept $\forall u.(C \Rightarrow D)$.
%Finally, arbitrary formulas can be introduced as abbreviations for the application of Boolean or modal operators to the concepts encoding assertions and local CIs.




%\paragraph{Internalisation of formulas}
%
%\nb{M: working here}
%
%Given a formula $\p$ in $\MLALCOu$ or $\TLALCOu$, checking
%for its satisfiability reduces to check concept satisfiability in
%$\MLALCOu$ or $\TLALCOu$, respectively.
%%
%\begin{lemma}
%\label{lemma:redformtoconcuniv}
%Partial $\MLALCOu$ and $\TLALCOu$ formula satisfiability are
%linear-time reducible to, respectively, partial $\MLALCOu$ and
%$\TLALCOu$ concept satisfiability.
%\end{lemma}
%%
%\begin{proof}
%  This is an adaptation to the modal and temporal case of the
%  so-called \emph{internalisation}
%  property~\cite[Chapter~5]{BaaEtAl03a} of those DLs equipped with the
%  universal role, allowing us to internalise a CI of the form
%  $C\sqsubseteq D$ as a concept of the form
%  $\forall u.(\lnot C \sqcup D)$.
%\end{proof}
%
%
%    {\color{red} formula satisfiability = concept satisfiability: use the universal role and nominals - $\varphi$ is satisfied in $\Mmf$ at $w$ iff $\forall u.\varphi^\dagger$ is satisfied in $\Mmf$ at $w$, where $\cdot^\dagger$ replaces $\land$ with $\sqcap$, etc. and $C \sqsubseteq D$ with $\forall u.(C \Rightarrow D)$, $A(a)$ with $\{a\} \Rightarrow A$ and $r(a,b)$ with $\{a\} \Rightarrow \exists r.\{b\}$}
    
    
    
    
    
To avoid ambiguities, we need to use
%\nb{M: slight notation change}
square brackets
%angled
%parentheses
when applying negation and modal operators to assertions, as in
$\lnot [ C(\tau) ]$
%$\lnot \lp C(\tau) \rp$
%$\lnot (C(\tau))$
and
$\Diamond_i [ C(\tau) ]$.
%$\Diamond \lp C(\tau) \rp$.
%$\Diamond (C(\tau))$.
%
Observe that, in an assertion of the form $\Diamond_{i} C(\tau)$, the diamond acts as a \emph{de re} operator, since the concept $\Diamond_{i} C$ applies to the object, if any, designated by the term $\tau$ at the current world $w$, and the assertion is false at a world whenever $\tau$ fails to designate at $w$. On the other hand, in an expression of the form
$\Diamond_{i} [ C(\tau) ]$,
%$\Diamond_{i} (C(\tau))$,
the diamond plays the role of a \emph{de dicto} modality, as it refers to the world of evaluation for the whole assertion $C(\tau)$. Using the lambda abstraction notation for first-order modal logic~\cite{FitMen12}, assertion $\Diamond_{i} A(a)$
%\nb{add ref to Appendix}
corresponds to
$\exists x. (\lp \lambda y. x = y \rp (a) \land \Diamond_i A(x))$,
%$\langle \lambda x. \Diamond A(x) \rangle (a)$,
whereas
$\Diamond_i [A(a)]$
%$\Diamond (A(a))$
stands for
$\Diamond_{i} \exists x. (\lp \lambda y. x = y \rp (a) \land A(x))$; see Appendix~A of the full version for details on the standard translation.
%$\Diamond \langle \lambda x.A(x) \rangle (a)$.
%\nb{M: rewrite more clearly}

 \end{remark}
%  In addition, we can introduce arbitrary formulas by applying Boolean or modal/temporal operators to assertions and CIs.
%  To avoid ambiguities, we write $\lnot (C(\tau))$ as an abbreviation of
%  $\lnot (\exists u. \{ \tau \} \sqcap \forall u. (\{ \tau \} \Rightarrow C))$
%  and
%  $\Diamond (C(\tau))$ to abbreviate:
%  $\Diamond(\exists u. \{ \tau \} \sqcap \forall u. (\{ \tau \} \Rightarrow C) )$ (in this case, the $\Diamond$ is called a \emph{de dicto} modality).
%  On the other hand, $\lnot C(\tau)$ stands for
%  $\exists u. \{ \tau \} \sqcap \forall u. (\{ \tau \} \Rightarrow
%  \lnot C)$ and
%  $\Diamond C(\tau)$ abbreviates
%  $\exists u. \{ \tau \} \sqcap \forall u.(\{ \tau \} \Rightarrow \Diamond C)$ (here, $\Diamond$ is  a \emph{de re} operator).
%  


%\begin{remark}
%\label{rem:assertion}
%  Assertions can be introduced as syntactic sugar, with $C(\tau)$ and
%  $r(\tau_1,\tau_2)$ being captured by the following CIs, respectively:
%  $\top \sqsubseteq \exists u. \{ \tau \}, \{ \tau \} \sqsubseteq C$;
%  and
%  $\top \sqsubseteq \exists u. \{ \tau_{1} \}, \{ \tau_{1} \}
%  \sqsubseteq \exists r.\{ \tau_{2} \}$.  To avoid ambiguities, we use
%  parentheses when applying Boolean or modal/temporal operators to
%  assertions. Thus, for instance, the formulas $\lnot (C(\tau))$ and
%  $\Diamond (C(\tau))$ abbreviate, respectively,
%  $\lnot ( \top \sqsubseteq \exists u. \{ \tau \} \land \{ \tau \}
%  \sqsubseteq C)$ and
%  $\Diamond( \top \sqsubseteq \exists u. \{ \tau \} \land \{ \tau \}
%  \sqsubseteq C)$, whereas the assertions $\lnot C(\tau)$ and
%  $\Diamond C(\tau)$ stand, respectively, for
%  $\top \sqsubseteq \exists u. \{ \tau \} \land \{ \tau \} \sqsubseteq
%  \lnot C$ and
%  $\top \sqsubseteq \exists u. \{ \tau \} \land \{ \tau \} \sqsubseteq
%  \Diamond C$.
%%
%%   Finally, as already observed for $\ALCOud$~\cite{ArtEtAl21a},
%%   we point out that formulas are just syntactic sugar in $\MLALCOud$ and $\TLALCOud$,
%%   since a CI $C\sqsubseteq D$ can be internalised~\cite{BaaEtAl03a,Rud11} as a concept of
%%   the form $\forall u. ( C \Rightarrow D)$.
%%%   \nb{M: explain also why all formulas (other than CIs) can be internalised?}
% \end{remark}
 
















%%%%%%%%%%%%%%%%%%%%%
%\paragraph{Fragments}

%\nb{M: added -- discuss $L_{\ELOud}$ def (formulas) -- fix modal operators}

%We now define other epistemic and temporal DLs with nominals, obtained
%from the languages introduced above.  In the following, let
%$L \in \{ \ML^{n}, \TL \}$.

%
%On the one hand, 

%First, we define $\ALCO$ as $\ALCOud$ without neither definite descriptions nor the universal role, while $\ALCOd$ and $\ALCOu$ are defined as $\ALCO$ with the addition of either definite descriptions or the universal role, respectively.
%We define $\ALCOd$ as $\ALCOud$ without the universal role, while $\ALCOu$ is defined as $\ALCOud$ without definite descriptions, and the classical $\ALCO$ is the sublanguage of $\ALCOu$
%without the universal role.
%






%\input{3-motivations.tex}





==> camera-ready/3-motivations.tex <==
\section{Motivations and examples}
\label{sec:motivation}
In the following, we provide some motivating examples to illustrate
the novel features of the modal and temporal free DL
languages introduced in the previous section.
\nb{M: rewrite/expand with ToM motivations + fix examples + move to later Sections}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Epistemic scenario.}
We discuss here the main features of the language $\MLALCOud$
interpreted on partial modal interpretations without the RDA and based
on frames
%for $\Sfive$
%where the accessibility relation is an
equipped with an
equivalence relation,
to provide motivating examples in an epistemic
setting. Thus, in the following, we will refer to such interpretations
as \emph{epistemic contexts}, and the worlds of the epistemic context
will be called \emph{states}.

%\paragraph{Terms}
Let us consider the following individual names: $\mathsf{clark}$ standing
for the `Clark Kent', $\mathsf{superman}$ standing for `Superman', and
$\mathsf{lois}$ standing for `Lois Lane'. In a given state of an epistemic
context, $\mathsf{clark}$ and $\mathsf{superman}$ can denote the same element
of the domain. However, since the epistemic context does not satisfy
the RDA, these individual names can also refer to different
individuals at different states. Moreover, the term
$\defdes ( \mathsf{Journalist} \sqcap \exists
\mathsf{worksWith}.\{\mathsf{lois}\})$ can be used to refer to the
journalist that works with Lois Lane, which can be understood as an
alternative way to describe Clark Kent.

%\paragraph{Concepts}
The concept $\Box\{\mathsf{superman}\}$ captures those individuals that are
\emph{known to be} Superman, whereas $\Diamond\{\mathsf{superman}\}$ would
be the set of individuals \emph{suspectable of being} (i.e., for which
it is not known that they are not) Superman.
%
% \paragraph{Concept inclusions}
The following CI can be used to express that Clark Kent is known to be
Clark Kent: $\{ \mathsf{clark} \} \sqsubseteq \Box \{ \mathsf{clark} \}$,
whereas we can use
$\{ \mathsf{clark} \} \sqsubseteq \lnot \Box \{ \mathsf{superman} \}$ to
express that Clark Kent is not known to be Superman. Moreover, the
following CIs assert that Lois Lane is known to be Lois Lane, i.e.,
$\{ \mathsf{lois} \} \sqsubseteq \Box \{ \mathsf{lois} \} $, and she is
also known to love Superman, i.e.,
$\{ \mathsf{lois} \} \sqsubseteq \Box \exists
\mathsf{loves}.\{\mathsf{superman}\}$,
but
%(unfortunately for Clark Kent)
not the journalist that works with
her, i.e., $\{\mathsf{lois}\} \sqsubseteq \lnot \Box \exists \mathsf{loves}.\{
\defdes ( \mathsf{Journalist} \sqcap \exists
\mathsf{worksWith}.\{\mathsf{lois}\}\}$.
%and the journalist that works with
%her, i.e., $\{\mathsf{lois}\} \sqsubseteq \Box\exists \mathsf{loves}.\{
%\defdes ( \mathsf{Journalist} \sqcap \exists
%\mathsf{worksWith}.\{\mathsf{lois}\}\}$.

\begin{example}
%\nb{M: todo fix}

\begin{itemize}
\item In the actual scenario, Clark \emph{is} Superman, but for Lois there is an epistemically conceivable alternative in which he \emph{is not}
\begin{align*}
\Mmf, w & \models \forall u. (\{ \mathsf{clark} \} \Leftrightarrow \{ \mathsf{superman} \}) \\
\Mmf, v & \not \models \forall u. (\{ \mathsf{clark} \} \Leftrightarrow \{ \mathsf{superman} \})
\end{align*}
\item
Lois knows that Superman is the hero that saves her
\[
\Mmf, w \models \Box \forall u. (\{ \mathsf{superman} \} \Leftrightarrow \{ \defdes ( \mathsf{Hero} \sqcap \exists
\mathsf{saves}.\{\mathsf{lois}\}) \} )
\]
\item
Lois loves who she knows to be the hero that saves her
\[
\Mmf, w \models \forall u. ( \{ \mathsf{lois} \} \Rightarrow \exists \mathsf{loves}. \Box \{ \defdes ( \mathsf{Hero} \sqcap \exists \mathsf{saves}.\{\mathsf{lois}\}) \} )
\]
\item
Lois actually loves Clark without even realising it
\begin{align*}
\Mmf, w \models & \forall u. ( (\{ \mathsf{lois} \} \Rightarrow \exists \mathsf{loves}.\{ \mathsf{clark} \} ) \\
						  & \sqcap \lnot \Box (\{ \mathsf{lois} \} \Rightarrow \exists \mathsf{loves}.\{ \mathsf{clark} \}) )
\end{align*}
\end{itemize}
\end{example}


% \paragraph{Formulas}

% The formula
% $\Box (\{ \mathsf{lois} \} \sqsubseteq \exists \mathsf{loves}.\{
% \mathsf{superman} \})$ states that it is known that Lois Lane loves
% Superman, whereas the formula
% $\lnot \Box (\{ \mathsf{lois} \} \sqsubseteq \exists \mathsf{loves}.\{
% \defdes ( \mathsf{Journalist} \sqcap \exists
% \mathsf{worksWith}.\{\mathsf{lois}\} ) \})$ says that it is not known
% that Lois Lane loves the journalist that works with her.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Temporal scenario.}
In the following, we exemplify and discuss the main features of the
language $\TLALCOud$ interpreted on partial traces without the RDA.
%providing motivations for its constructors and semantic choices.

%\paragraph{Terms}
Let us consider the individual name $\mathsf{dl}$ which can serve as a
``variable''-name, that might change its value (and even remain
uninterpreted) at different instants, so to denote, e.g., the
Description Logic (DL) workshops that take place over the years.
Instead, the individual name $\mathsf{dl22}$ can be used as an
individual name with a fixed referent across time, denoting the DL
workshop that takes place in 2022 only. Finally, the definite
description $\defdes\exists \mathsf{isGCof}.\{\mathsf{dl}\}$ is
able to refer non-rigidly to the General Chair of the DL workshop.

%\paragraph{Concepts}
The concept $\Diamond^{+} \{\mathsf{dl}\}$ can be used to refer to
those objects that will eventually be the DL workshop. When
interpreted on total traces with the RDA, the extension of this
concept would contain exactly one object, i.e., the (rigid) referent
of the individual name $\mathsf{dl}$. On the other hand, on partial
traces without the RDA, its extension might contain also zero, or more
than one, objects, namely, those individuals that are the values of
$\mathsf{dl}$ at different time points. In addition, the concept
$\Diamond^{+}\{\defdes\exists\mathsf{isGCof}.\{\mathsf{dl}\}\}$ can be
used to represent those individuals that will eventually be the
General Chair of the various DL workshops.
%
The concept
$\Diamond^{+} \exists \mathsf{hasPCM}.\Diamond^{+} \{\defdes \exists
\mathsf{isGCof}.\{\mathsf{dl}\}\}$ captures those objects that will
eventually have as PC Members some individuals that, at some point in
the future, will be the General Chair of the DL workshop.

% \paragraph{Concept inclusions}
Let $\mathsf{proc\mbox{-}dl22}$ stands for the proceedings of the DL22
workshop. To enforce the proceedings of the DL22 to behave as a rigid
designator, we can enforce the following CI,\nb{A: expanding?}
$\Diamond^{+} \{\mathsf{proc\mbox{-}dl22}\} \sqsubseteq
\Box^+\{\mathsf{proc\mbox{-}dl22}\}$.
%
% To let the individual name $\mathsf{dl22}$ for the DL22 workshop
% behave as a rigid designator, we can enforce both the CIs
% $\{ \mathsf{dl22} \} \sqsubseteq \Box^{+} \{ \mathsf{dl22} \}$ and
% $\Diamond^{+} \{ \mathsf{dl22} \} \sqsubseteq \{ \mathsf{dl22} \}$,
% or, alternatively, the CI
% $\Diamond^{+} \{ \mathsf{dl22} \} \sqsubseteq \Box^+\{ \mathsf{dl22}
% \}$.
On the other hand, we can require $\mathsf{dl}$ to be a
\emph{flexible} designator by enforcing the following CI,
$\top \sqsubseteq \exists u.(\Diamond^{+}\{\mathsf{dl}\} \sqcap
\Diamond^{+} \lnot \{ \mathsf{dl}\})$.
%
% $\Diamond^{+}\{ \mathsf{dl} \} \sqsubseteq \Diamond^{+} \lnot \{
% \mathsf{dl}\}$. An individual name which is left uninterpreted at each
% instant of a partial trace would satisfy all the previous CIs, thus
% behaving both as a rigid and as a flexible designator. To state
% instead that $\mathsf{dl}$ is \emph{not} a rigid designator, we can
% use the CI
% $\top \sqsubseteq \exists u.( \Diamond^{+} \{ \mathsf{dl} \} \sqcap
% \Diamond^{+} \lnot \{ \mathsf{dl} \} )$, involving the universal role.
Finally, we can enforce $\mathsf{dl22}$ to be an \emph{instantaneous}
designator by using the following CIs,
$\top \sqsubseteq \Diamond^{+}\exists u.\{\mathsf{dl22}\}$,\nb{A: No
  if CI are global}
$\Diamond^{+} (\{\mathsf{dl22}\} \sqcap
\Diamond\{\mathsf{dl22}\})\sqsubseteq \bot$, meaning that
$\mathsf{dl22}$ is not a ghost and that no objects can be the denotation
of the individual name $\mathsf{dl22}$ at two distinct instants.
%
Notice that ghost individuals are assumed to be (vacuously) rigid,
while flexible and instantaneous individuals should denote.

%\paragraph{Formulas}
To state that the (current) General Chair of DL will be one of next
year's PC Members of DL we can use the assertion,
$(\Next \exists {\sf isPCMof}.\{{\sf dl}\})(\{\defdes\exists {\sf
  isGCof}.\{ {\sf dl }\}\})$.
% Recall that this assertion is just
% shorthand for (the conjunction of) the CIs
% $\top \sqsubseteq \exists u.\{ \defdes \exists {\sf isGCof}. \{ {\sf
%   dl }\} \}$ and
% $\{ \defdes \exists {\sf isPCof}. \{ {\sf dl }\} \} \sqsubseteq \Next
% \exists {\sf isPCMof}. \{ {\sf dl} \}$.
%
On the other hand, to say that, next year, the (future) General Chair
of DL will be one of the PC Members of DL, the following formula
should be used instead,
$\Next (\top \sqsubseteq \exists u.\{\defdes \exists {\sf isGCof}.
\{{\sf dl}\}\} \land \{\defdes \exists {\sf isGCof}.\{ {\sf dl}\}\}
\sqsubseteq \exists{\sf isPCMof}.\{{\sf dl}\})$.
%
Moreover, one can express that, at some point, DL22 will be the DL
workshop, by writing the following assertion,
$\Diamond^{+} (\{\mathsf{dl}\}(\{\mathsf{dl22}\}))$. Finally, the
formula
$\Box^{+}(\{\defdes\exists{\sf isGCof}.\{{\sf dl}\}\}
\sqsubseteq \exists{\sf isPCMof}.\Next\{{\sf dl}\})$ asserts
that it will always be the case that the General Chair of DL is going
to be a DL's PC Member on the subsequent year.
        
\begin{example}
\begin{itemize}
%
	\item
	KR24 is a rigid designator
	\[
	\Mmf, t \models \Diamond^{+} \{ \mathsf{kr24} \} \sqsubseteq
\Box^+  \{ \mathsf{kr24} \}
\]
	\item
	KR24 is the upcoming KR Conference, but there will be more (hopefully)
	\begin{align*}
	\Mmf, t & \models \exists u. \{\mathsf{kr24}\} \land \{\mathsf{kr24}\} \sqsubseteq \Next \{ \mathsf{kr} \}  \\
	\Mmf, t & \not \models \Diamond^{+} \{\mathsf{kr}\} \sqsubseteq \Next \{ \mathsf{kr} \}
	\end{align*}
	\item
	However, KR24 will never come back (as the current KR conference)
	\[
	\Mmf, t \models \Box^{+} (\{ {\sf kr24 } \} \sqsubseteq \Next \Box \lnot \{\mathsf{kr}\} )
\]
\item
Whoever is a Program Chair of KR always becomes either the General Chair or a PC Member of KR next year
	\begin{align*}
\Mmf, t \models \ & \Box^{+} ( \exists {\sf isPrgChr}.\{ {\sf kr} \} \sqsubseteq \\
							& \{ \defdes \exists {\sf isGenChr}. \Next \{ {\sf kr} \} \} \sqcup \exists {\sf isPCMbr}. \Next \{ {\sf kr } \} )
	\end{align*}
\end{itemize}
\end{example}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "rda"
%%% End:


==> camera-ready/3-reductions.tex <==
% !TEX root =  rda.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reasoning Problems and Reductions}
\label{sec:reduction}


%\subsubsection{Reasoning problems}
%.{\color{red}{F: I believe this has to be reduced to two main problems: see above.}}

Let $\Cmc$ be a class of frames (e.g., frames with $n$ equivalence relations) and $\ML^n_{\DL}$ a language.
We consider the following two main reasoning problems. 
%
\begin{description}
\item[Concept $\Cmc$-Satisfiability:] Given an  $\ML^n_{\DL}$-concept $C$, is there an interpretation $\Mmf$ based on a frame in $\Cmc$ such that
$C$ is satisfied in $\Mmf$?
\item[Concept $\Cmc$-Satisfiability under Global Ontology:] \hfill Given an  $\ML^n_{\DL}$-concept $C$ and an  $\ML^n_{\DL}$-ontology $\Omc$, is there an interpretation $\Mmf$ based on a frame in $\Cmc$
such that $C$ is satisfied  in $\Mmf$ under $\Omc$?
\end{description}
%
In the sequel, for the case of concept $\Cmc$-satisfiability under global ontology, we will assume without loss of generality that $C$ is a concept name.
Indeed, we can extend $\Omc$ with CI $A \equiv C$, for a fresh concept name $A$, and consider satisfiability of $A$ under the extended ontology, which is a model conservative extension of $\Omc$.




%Given a DL $\DL$
%%(among those considered in this paper)
%and a class of $n$-frames $\Cmc$, the \emph{partial} (respectively, \emph{total})
%\emph{$\ML^{n}_{\DL}$}
%%$\MLALCOud$
%\emph{concept} \emph{satisfiability problem over $\Cmc$}
%\emph{without} (respectively, \emph{with}) \emph{the RDA} is the problem
%of deciding, given an
%$\ML^{n}_{\DL}$
%%$\MLALCOud$
%concept $C$, whether there exists a
%partial (respectively, total) modal interpretation without (respectively, with) the RDA based on an $n$-frame in $\Cmc$, and a world $w$ in $\Mmf$, such that $C^{\Imc_{w}} \neq \emptyset$.
%
%\paragraph{Modal concept satisfiability under global ontology}
%
%The \emph{partial} (respectively, \emph{total})
%\emph{$\ML^{n}_{\DL}$
%concept satisfiability problem under
%%$\MLALCOud$
%global ontology} \emph{over $\Cmc$}
%\emph{without} (respectively, \emph{with}) \emph{the RDA} is the problem
%of deciding, given an $\ML^{n}_{\DL}$ ontology $\Omc$ and a concept $C$, whether $C$ is \emph{satisfiable under (global) $\Omc$ on partial} (resp., \emph{total}) \emph{modal interpretations in $\Cmc$} \emph{without} (resp., \emph{with}) \emph{the RDA}, that is: whether there exists a partial (respectively, total) modal interpretation $\Mmf$ without (respectively, with) the RDA based on an $n$-frame in $\Cmc$, and a world $w$ in $\Mmf$, such that $\Mmf \models \Omc$ and $C^{\Imc_{w}} \neq \emptyset$.
%
%%% OLD VERSION -- ALL REASONING PROBLEMS (MODAL)
%Given a DL $\DL$
%%(among those considered in this paper)
%and a class of $n$-frames $\Cmc$, the \emph{partial} (respectively, \emph{total})
%\emph{$\ML^{n}_{\DL}$
%%$\MLALCOud$
%formula} (respectively: \emph{concept}; \emph{ontology}) \emph{satisfiability problem over $\Cmc$}
%\emph{without} (respectively, \emph{with}) \emph{the RDA} is the problem
%of deciding, given an
%$\ML^{n}_{\DL}$
%%$\MLALCOud$
%formula $\p$ (respectively: concept $C$; ontology $\Omc$), whether there exists a
%partial (respectively, total) modal interpretation without (respectively, with) the RDA and based on an $n$-frame in $\Cmc$ that satisfies $\p$ (respectively: $C$; $\Omc$).
%The \emph{partial} (respectively, \emph{total})
%\emph{$\ML^{n}_{\DL}$
%%$\MLALCOud$
%global ontology} \emph{satisfiability problem over $\Cmc$}
%\emph{without} (respectively, \emph{with}) \emph{the RDA} is the problem
%of deciding, given an $\ML^{n}_{\DL}$ ontology $\Omc$, whether there exists a partial (respectively, total) modal interpretation without (respectively, with) the RDA and based on an $n$-frame in $\Cmc$ that globally satisfies $\Omc$.

%%Given a class of frames $\Cmc$, we say that $\p$ is \emph{satisfiable (in partial modal interpretations with, respectively without, the RDA) in $\Cmc$} if there exists a (partial) modal interpretation (with, respectively without, the RDA) based on a frame in $\Cmc$ that satisfies $\p$.
%%The \emph{formula satisfiability problem for $L_{\ALCOud}$} (\emph{with}, respectively \emph{without}, \emph{the RDA}) is the following decision problem: given an $\MLALCOud$ formula $\p$, decide whether $\p$ is
%%$L_{\ALCOud}$ satisfiable (with, respectively without, the RDA).
%
%%%A frame $\Fmf = (W, \sim)$, where $\sim$ is an
%%%\emph{equivalence relation} on $W$, is called \emph{epistemic frame}.
%%The \emph{partial} (\emph{total}) \emph{$\SfivenALCOud$ formula
%%  satisfiability problem} (\emph{with} or \emph{without the RDA},
%%respectively) is the {partial} ({total}) $\MLALCOud$ formula
%%satisfiability problem (with or without the RDA, respectively) over
%%the class of
%%$n$-frames
%%%\emph{epistemic $n$-frames}
%%$(W, \{ R_{i} \}_{i \in I})$, with $I = \{ 1, \ldots, n \}$,
%%%that is, frames such that each $R_{i}$ is
%%%an \emph{equivalence relation} on $W$.
%%such that each $R_{i}$ is an \emph{equivalence relation} on $W$.
%%%\nb{M: todo fix}
%%The \emph{partial} (\emph{total}) \emph{$\K^{n}_{\ALCOud}$} and \emph{$\KDfourfive^{n}_{\ALCOud}$} \emph{formula satisfiability problems} are defined analogously, over the classes of \emph{all} frames, and of \emph{serial}, \emph{transitive} and \emph{Euclidean} frames, respectively.



%%% ML_{\ALCOud} FORMULA SATISFIABILITY
%
%Given $L \in \{ \K^{n}, \KDfourfive^{n}, \Sfive^{n} \}$, the \emph{partial} (\emph{total}) \emph{$L_{\ALCOud}$ formula satisfiability problem} (\emph{with} or \emph{without the RDA}) is the {partial} ({total}) $\MLALCOud$ formula
%satisfiability problem (with or without the RDA) over
%the class of $n$-frames
%%\emph{epistemic $n$-frames}
%$(W, \{ R_{i} \}_{i \in I})$, with $I = \{ 1, \ldots, n \}$,
%%that is, frames such that each $R_{i}$ is
%%an \emph{equivalence relation} on $W$.
%such that each $R_{i}$ is:
%\begin{itemize}
%\item any relation on $W$, if $L = \K^{n}$;
%\item a \emph{serial}, \emph{transitive}, and \emph{Euclidean} relation on $W$, if $L = \KDfourfive^{n}$;
%\item a \emph{reflexive}, \emph{transitive}, and \emph{symmetric}
%%(i.e., an \emph{equivalence})
%{relation} on $W$, if $L = \Sfive^{n}$.
%\end{itemize}


%\paragraph{Temporal concept satisfiability}
%
%Similarly, for a class of flows of time $\Cmc$, the \emph{partial}
%(respectively, \emph{total}) \emph{$\TL_{\DL}$}
%%$\TLALCOud$
%\emph{concept} \emph{satisfiability problem over $\Cmc$} \emph{without} (respectively, \emph{with}) \emph{the RDA} is the
%problem of deciding, given a
%$\TL_{\DL}$
%%$\TLALCOud$
%concept $C$ whether there
%exists a partial (respectively, total) trace $\Mmf$ without (respectively, with) the RDA based on a flow of time in $\Cmc$ such that $C^{\Imc_{0}} \neq \emptyset$.
%%at instant $0$.
%
%\paragraph{Temporal concept satisfiability under global ontology}
%
%
%The \emph{partial} (respectively, \emph{total})
%\emph{$\TL_{\DL}$
%%$\MLALCOud$
%concept satisfiability problem under 
%global ontology} \emph{over $\Cmc$}
%\emph{without} (respectively, \emph{with}) \emph{the RDA} is the problem
%of deciding, given a $\TL_{\DL}$ ontology $\Omc$ and concept $C$, whether $C$ is is \emph{satisfiable under (global) $\Omc$  on partial} (resp., \emph{total}) \emph{temporal interpretations in $\Cmc$} \emph{without} (resp., \emph{with}) \emph{the RDA}, that is:  whether there exists a partial (respectively, total) trace $\Mmf$ without (respectively, with) the RDA and based on a flow of time in $\Cmc$ such that $\Mmf \models \Omc$ and $C^{\Imc_{0}} \neq \emptyset$.
%
%%% OLD VERSION -- ALL REASONING PROBLEM (TEMPORAL)
%Similarly, for a class of flows of time $\Cmc$, the \emph{partial}
%(respectively, \emph{total}) \emph{$\TL_{\DL}$
%%$\TLALCOud$
%formula} (respectively: \emph{concept}; \emph{ontology}) \emph{satisfiability problem over
%  $\Cmc$} \emph{without} (respectively, \emph{with}) \emph{the RDA} is the
%problem of deciding, given a
%$\TL_{\DL}$
%%$\TLALCOud$
%formula $\p$ (respectively: concept $C$; ontology $\Omc$), whether there
%exists a partial (respectively, total) trace without (respectively, with) the RDA and based on a flow of time in $\Cmc$ that satisfies $\p$ (respectively: $C$; $\Omc$).
%%at instant $0$.
%The \emph{partial} (respectively, \emph{total})
%\emph{$\TL_{\DL}$
%%$\MLALCOud$
%global ontology} \emph{satisfiability problem over $\Cmc$}
%\emph{without} (respectively, \emph{with}) \emph{the RDA} is the problem
%of deciding, given a $\TL_{\DL}$ ontology $\Omc$, whether there exists a partial (respectively, total) trace without (respectively, with) the RDA and based on a flow of time in $\Cmc$ that globally satisfies $\Omc$.
%
%%The \emph{partial} (\emph{total}) \emph{$\LTLALCOud$ formula
%%  satisfiability problem} (\emph{with} or \emph{without the RDA},
%%respectively) is the {partial} ({total}) $\TLALCOud$ formula
%%satisfiability problem (with or without the RDA, respectively) over
%%$\{ (\mathbb{N}, <) \}$.  The \emph{partial} (\emph{total})
%%\emph{$\LTLfALCOud$ formula satisfiability problem} (\emph{with} or
%%\emph{without the RDA}, respectively) is the {partial} ({total})
%%$\TLALCOud$ formula satisfiability problem (with or without the RDA,
%%respectively) over the class of finite strict linear orders.
%%%of the form $(\{ 0, \ldots, n \}, <)$, where $n \in \mathbb{N}$.


%%% TL_{\ALCOud} FORMULA SATISFIABILITY
%Given $L \in \{ \LTL, \LTLf \}$, the \emph{partial} (\emph{total}) \emph{$L_{\ALCOud}$ formula satisfiability problem} (\emph{with} or \emph{without the RDA},
%respectively) is the {partial} ({total}) $\TLALCOud$ formula
%satisfiability problem (with or without the RDA, respectively) over the class:
%\begin{itemize}
%\item $\{ (\mathbb{N}, <) \}$, if $L = \LTL$;
%\item of \emph{finite strict linear orders}, if $L = \LTLf$.
%\end{itemize}



%%% OLD VERSION -- ENTAILMENT PROBLEMS
%Given a class of $n$-frames $\Cmc$, the \emph{partial} (resp., \emph{total}) \emph{$\ML^{n}_{\DL}$ entailment problem over $\Cmc$}
%\emph{without} (resp., \emph{with}) \emph{the RDA} is the problem
%of deciding, given an $\ML^{n}_{\DL}$ formula $\p$ and ontology $\Omc$, whether $\p$ is entailed under $\Omc$ with respect to partial (resp., total) modal interpretations without (resp., with) the RDA and based on $n$-frames in $\Cmc$.
%
%The \emph{partial} (resp., \emph{total}) \emph{$\ML^{n}_{\DL}$ entailment problem under global ontology over $\Cmc$} \emph{without} (resp., \emph{with}) \emph{the RDA} is the problem of deciding, given an $\ML^{n}_{\DL}$ formula $\p$ and ontology $\Omc$, whether $\p$ is entailed under global $\Omc$ with respect to partial (resp., total) modal interpretations without (resp., with) the RDA and based on $n$-frames in $\Cmc$.
%
%Similarly, for a class of flows of time $\Cmc$, the \emph{partial} (resp., \emph{total}) \emph{$\TL_{\DL}$
%%$\TLALCOud$
%entailment problem over $\Cmc$} \emph{without} (resp., \emph{with}) \emph{the RDA} is the problem of deciding, given a
%$\TL_{\DL}$
%%$\TLALCOud$
%formula $\p$ and ontology $\Omc$, whether $\p$ is entailed under $\Omc$ with respect to partial (resp., total) traces without (resp., with) the RDA and based on time flows in $\Cmc$.
%
%The \emph{partial} (resp., \emph{total}) \emph{$\TL_{\DL}$
%%$\TLALCOud$
%entailment problem under global ontology over $\Cmc$} \emph{without} (resp., \emph{with}) \emph{the RDA} is the problem of deciding, given a $\TL_{\DL}$
%%$\TLALCOud$
%formula $\p$ and ontology $\Omc$, whether $\p$ is entailed under global $\Omc$ with respect partial (resp., total) traces without (resp., with) the RDA and based on time flows in $\Cmc$.



%\medskip

%Let $P$ be a reasoning problem among
%concept satisfiability and concept satisfiability under global ontology, 
%%formula satisfiability, concept satisfiability, entailment, and entailment under global ontology, 
%and let $\DL$ be a DL among those considered in this paper.



%\nb{M: working here}


%Analogous definitions are given for the fragments that disallow
%modalised and temporalised concepts.
%For instance, the partial
%$\ALCOud$-$\LTLf$ concept satisfiability problem without the RDA is
%the problem of deciding, given an $\ALCOud$-$\TL$
%%$\TLALCOud$
%concept $C$, whether there exists a partial finite trace without the RDA that satisfies $\p$.
%For instance, the partial
%$\ALCOud$-$\LTLf$ formula satisfiability problem without the RDA is
%the problem of deciding, given an $\ALCOud$-$\TL$
%%$\TLALCOud$
%formula $\p$, whether there exists a partial finite trace without the RDA that satisfies $\p$.

%For instance, the partial
%$\ALCOud$-$\LTLf$ formula satisfiability problem without the RDA is
%the problem of deciding, given an $\ALCOud$-$\TL$
%%$\TLALCOud$
%formula $\p$, whether there exists a partial finite trace without the RDA that satisfies $\p$.
 
%the partial $\ALCOud$-$\TL$ formula satisfiability problem without the RDA over finite strict linear orders.
%Finally, given a reasoning problem $P$, the \emph{problem $P$ on expanding domains} is defined similarly, with respect to modal or temporal interpretations with expanding domains.


%Analogous 
%%\nb{M: todo fix}
%definitions are given
%%for the entailment problems, as well as
%for the fragments that restrict the DL dimension,
%%(e.g., $\Sfive_{\ELOud}$ formula satisfiability)
%or the modal/temporal dimension.
%%as well as for the KB satisfiability problems.
%%(such as $\ALCOud$-$\LTL$ formula satisfiability).
%For instance, the partial $\Sfive^{n}_{\ELOud}$ formula satisfiability problem without the RDA,
%respectively) is the partial $\ML^{n}_{\ELOud}$ formula
%satisfiability problem without the RDA over
%the class of frames based on equivalence relations.
%Moreover, the partial $\ALCOud$-$\LTLf$ formula satisfiability problem without the RDA is the partial $\ALCOud$-$\TL$ formula satisfiability problem without the RDA over finite traces.
%As another example, the partial $\LTLELO$ entailment problem without the RDA is the partial $\mathcal{T}\mathcal{L}_{\ELO_{\bot}}$ entailment problem without the RDA over $\{ (\mathbb{N}, <) \}$.






%\allowdisplaybreaks


%\subsection{RDA-Independent Observations}

%{\color{red}
We begin
with a few observations on polytime
	reductions between the concept satisfiability problems (under global ontology) for two main languages, $\ML^n_{\ALCOu}$ and $\MLALCOud$, and various semantic conditions, including (non-)rigid designators, total and partial interpretations, and expanding and constant domains. We also show how to eliminate the universal role using the global ontology and how to replace definite descriptions with nominals, and the other way round, which in particular means that satisfiability in the full $\MLALCOud$ and its fragment without $\defdes$ has the same computational properties. These observations will be useful in our constructions below, where we also apply them to smaller fragments, if the results carry over. Proofs are available in Appendix~B of the full version.
%}

\paragraph{No-RDA Subsumes
%{\color{red}{Global}}
RDA}

%%% (LOCALLY) RIGID
An interpretation $\Mmf$ satisfies the \emph{rigid designator assumption} \textup{(}\emph{RDA}\textup{)} if every individual name $a \in \NI$ is a \emph{rigid designator} in $\Mmf$, in the sense that,
for every $w, v \in W$ such that $w R_{i} v$, if $a$ designates at $w$, then it designates at~$v$ and $a^{\Int_{w}} = a^{\Int_{v}}$.
%\nb{M: check}
%\textcolor{red}{does it not imply that we only need $\{a\} \sqsubseteq \Box \{ a\}$? the diamond CI would translate into an additional condition: if $a$ designates at $v$ and the object exists at $w$, then $a$ designates at $w$ and = }
%%% STRONGLY RIGID
%{\color{red}{
%Moreover, we say that an interpretation satisfies the \emph{strong rigid designator assumption} \textup{(}\emph{strong RDA}\textup{)} if every individual name $a \in \NI$ is a \emph{strongly rigid designator}, meaning that, for every $w, v \in W$ such that $w R_{i} v$, $a$ designates at $w$ iff $a$ designates at $v$, and $a^{\Int_{w}} = a^{\Int_{v}}$.
%}}
%%%GLOBALLY RIGID
%{\color{red}{
%  Moreover, we say that $\Mmf$ satisfies
%  the \emph{global rigid designator assumption} \textup{(}\emph{global RDA}\textup{)} if every individual name $a \in \NI$ is a \emph{globally rigid designator} in $\Mmf$, meaning that, for every $w, v \in W$, if $a$ is denoting at $w$, then it is denoting at~$v$ and $a^{\Int_{w}} = a^{\Int_{v}}$.
%  }}
%    \nb{M: changed, check + move to Appendix?}
%
%
%
%\begin{remark}[Satisfiability with the RDA]\em
%\label{rem:nonRDA}
%\nb{M: moved this remark here (it doesn't fit the example section)}
%We point out an interesting behaviour of formula satisfiability without the RDA.
%under the non-RDA
%Let us consider the following:
For instance, concept %the concept %\nb{if we replace the first $\Rightarrow$ with $\sqcap$, can we get rid of total? also do we not miss a forall here?}
\begin{equation*}
\exists u.(\{a\} \sqcap \Box C) \sqcap \Diamond \exists u.(\{a\} \sqcap \lnot C),
\end{equation*}
%$(\{a\} \sqsubseteq \Box C) \land \Diamond (\{a\} \sqsubseteq \lnot C)$.
%This concept,
%formula,
is unsatisfiable in
interpretations 
\emph{with the RDA},
%if the RDA is assumed,
but is satisfiable otherwise, 
as $a$ can designate differently at
different worlds.
Note that
 an individual that fails to designate at all worlds is vacuously
 rigid.
%The same applies to the formula\nb{remove?} abbreviating the above concept:
%\begin{align*}
%& (\exists u. \{ a \} \sqcap \forall u.(\{a\} \Rightarrow \Box C)) \ \sqcap \\
%\Diamond & (\exists u. \{ a \} \sqcap \forall u.(\{a\} \Rightarrow \lnot C))
%\end{align*}
%   \[
%   \Box C(a) \land \Diamond(\lnot C(a)).
%  \]
%$(\{a\} \sqsubseteq \Box C) \land \Diamond (\{a\} \sqsubseteq \lnot C)$.
%This concept,
%formula,
%is unsatisfiable
%in partial interpretations
%with the RDA,
%%if the RDA is assumed,
%but
%satisfiable
%on partial interpretations
%without the RDA.
%\end{remark}
%
%
% Note that
%  {\color{red}{global rigidity implies rigidity, and that }}
%% {\color{red}{strong rigidity implies rigidity, and that }}
% an individual name that fails to designate at all worlds is vacuously
%{\color{red}{globally}} 
%% {\color{red}{strongly}}
% rigid.
%  {\color{red}{
% However, an individual name that designate at a world $v$ and not at a world $w$, where $wR_{i}v$, can be a rigid, but not a globally rigid, designator.
% }}
%% {\color{red}{
%% However, an individual name that designate at a world $v$ and not at a world $w$, where $wR_{i}v$, can be a rigid, but not a strongly rigid, designator.
%% }}
%%
%
%.{\color{red} F: we have to be careful here as we assume
%    global interpretation of $\Diamond_{i}^{+}\{a\} \sqsubseteq
%    \Box_{i}^{+} \{a\}$ below. For a reduction under local reasoning
%    the reduction has to be done by carefully prefixing modalities.}
%
%  {\color{blue} Ale: This
%    $\Diamond_{i}^{+}\{a\} \sqsubseteq \Box_{i}^{+} \{a\}$ is a local
%    axiom and can be easily internalized. For S5 and the Temporal case
%    (SAT at $0$) it should work also when the axiom is interpreted
%    globally. We should introduce 2 different symbols for local and
%    global CIs.\\
%    On the other hand Abox and denotation needs local axioms in the
%    Temporal case.}
%		
%  {\color{green!75!black!75}{ M: I think the idea is indeed to
%      internalise this CI into a (``local'') concept, and keep the
%      interpretation of CIs global only. Assertions and denotation can
%      be again internalised into concepts, right? Both in the temporal
%      and in the epistemic case, we won't need local CIs anymore.  }}
%
%  {\color{blue} Ale: I consider local CIs or internalization as the
%    same kind of constraint different from having just global CIs. And
%  in this view, the case with ``just global CIs'' is not able to
%  capture either Aboxes or denotations.}
%		
%		
The following proposition shows the
%{\color{red}{global}} \nb{M: discuss -- added global} 
RDA can be enforced in interpretations
%\textcolor{red}{
by an ontology.
%}
%\nb{M: todo fix proof with local RDA}


\begin{restatable}{proposition}{rdatononrda}
\label{prop:rdatononrda}
%Let  $\Cmc$ be a class of frames. 
In $\ML^n_{\ALCOu}$ and $\MLALCOud$,
%{\color{blue}{
%\textup{(}total\textup{)}
%}}
concept $\Cmc$-satisfiability under global ontology with the RDA is poly\-time-reducible to
%{\color{blue}{
%\textup{(}total, respectively\textup{)}
%}}
concept $\Cmc$-satisfiability under global ontology,
with both constant and expanding domains.
%{\color{blue}{
%Moreover, total concept $\Cmc$-satisfiability with the RDA is polytime-reducible to total concept $\Cmc$-satisfiability, with both constant and expanding domains.
%\nb{M: check}}}
\end{restatable}


%\begin{restatable}{proposition}{rdatononrda}
%\label{prop:rdatononrda}
%%Let  $\Cmc$ be a class of frames. 
%In $\ML^n_{\ALCOu}$ and $\MLALCOud$,
%concept $\Cmc$-satisfiability \textup{(}under global ontology\textup{)} with the
%%{\color{red}{global}}
%%\nb{M: discuss -- added global}
%RDA is poly\-time-reducible to
%concept $\Cmc$-satisfiability \textup{(}under global ontology, respectively\textup{)},
%with both  constant and expanding domains.
%\end{restatable}
%
 The proof is based on the observation that
% $n$ pairs of
CIs of the form
$\{a\} \sqsubseteq \Box_i\{a\}$,
% \textcolor{red}{ and $\Diamond_i \{a\} \sqsubseteq \{a\}$},
for $i\in I$, ensure that $a$ can be made  a rigid designator in any interpretation. This provides a reduction for the case of global ontology, where a given $\Omc$ is extended with such CIs for every $a$.
%\textcolor{red}{
%\nb{added}
A similar reduction is provided in Appendix~B for concept satisfiability in total interpretations.
%}


In the sequel,
we assume implicitly that interpretations do \emph{not} satisfy the RDA, and explicitly write `with the
%{\color{red}{(global)}}
RDA' where necessary.


%%% APPENDIX REMARK
%{\color{red}{
%Observe
%\nb{M: keep only in Appendix?} 
%that, for the reduction to hold in the global ontology case, an individual name $a$ does not have to designate in every world. 
%For instance, consider an
%%expanding-domains
%interpretation $\Mmf$
%with $W = \{ w, v \}$, $wRv$, $\Delta = \{ d \}$,
%%$\Delta^{v} = \{ d, e \}$
%and such that $a$ does not designate in $w$ but $a^{\Imc_{v}} = d$.
%%Clearly, $\Mmf$ satisfies the RDA but cannot be made total by assigning an interpretation of $a$ at $w$ without breaking the RDA.
%In this example, $a$ is rigid and the CI above is vacuously satisfied 
%because $a$ does not designate at $w$.
%The same applies to an expanding domain variant of the example above, where $\Delta^{w} = \{ d \}$, $\Delta^{v} = \{ d, e \}$, $a$ does not designate in $w$, and $a^{\Imc_{v}} = e$.
%
%For the \emph{total} concept satisfiability case,
%we denote by $C'$ the concept obtained from $C$ by adding conjuncts $D_{C}$ of the form $\Box^{\pi}\forall u.(\{ a \} \Rightarrow \Box_{i} \{ a \})$, for $i\in I$, where $\Box^{\pi}$ is a suitable sequences of boxes (polynomial in the size of $C$) that captures the nesting of operators under which the nominal $a$ occurs in $C$.
%It can be seen that $C$ is $\Cmc$-satisfiable on total interpretations with the RDA iff $C'$ is $\Cmc$-satisfiable on total interpretations.
%
%However, we cannot enforce that any \emph{partial} interpretation satisfying
%$C'$
%%$C$ and the additional conjuncts of the form $D_{C}$
%at some world, can be transformed into a partial interpretation with the RDA that satisfies $C$, as witnessed by the following counterexample.
%Let $C$ be the concept
%\[
%\forall u. (\lnot \{ a \} \sqcap  \Diamond \lnot \{ a \} ) \sqcap \Diamond \exists u.\{ a \},
%\]
%%\[
%%\lnot \exists u. \{ a \} \sqcap \Diamond \exists u.\{ a \} \sqcap \lnot \exists u. \Box \{ a \},
%%\]
%and let $C'$ be the conjunction of $C$ with the concept $\forall u.(\{ a \} \Rightarrow \Box \{ a \})$.
%Consider a partial interpretation $\Mmf$ with expanding domains, such that $w R v_{i}$ and $v_{i} R u$, for $i = 1,2$, and $\Delta^{w} = \{ d \}$, $\Delta^{v_{i}} = \Delta^{u} = \{ d, e \}$. Moreover, let $a$ be non-designating in $w$, while $a^{\Imc_{v_{1}}} = d$, $a^{\Imc_{v_{2}}} = e$, and $a^{\Imc_{v_{1}}} = d$. It can be seen that $\Mmf$ is a partial interpretation satisfying $C'$ in $w$. However, we cannot turn $\Mmf$ into a partial interpretation with the RDA that satisfies $C$.
%A similar counterexample applies also to the constant domain case, by taking $\Delta = \{ d, e \}$.
%This is due to the fact that $C'$ is bounded on the levels of successors of $w$ that it can reach, whereas, under global ontology, the corresponding CI $\{ a \} \sqsubseteq \Box \{ a \}$ has to hold at all worlds of the interpretation.
%}}
%% \nb{Discuss local rigidity in expanding domains in more detail here?}
%  
%%Dropping the RDA is the most general
%%  assumption, since rigid designators can be enforced by the CI
%%  $\Diamond_{i}^{+}\{a\} \sqsubseteq \Box_{i}^{+} \{a\}$. Moreover, partial interpretations are a generalisation of the classical ones: an individual
%%  can be forced to denote at some state (i.e., not being a ghost) with the CI
%%  $\top \sqsubseteq \Diamond_{i}^{+} \exists u.\{a\}$, and to denote at all states with the formula $\Box_{i}^{+} (\top \sqsubseteq \exists u.\{a\})$.
%%  Note that a ghost individual is vacuously rigid.




%\textcolor{red}{M: mention that it does not cover $\ELOu$ and $\ELOud$? (in Section~\ref{sec:reasontfdl}?)}

 
 











%\subsection{Key Reductions}

\paragraph{From Total to Partial Satisfiability and Back}

%\textcolor{red}{
%  Partial interpretations are a generalisation of the classical ones: an individual
%  can be forced to denote at some world
%%  (i.e., not being a ghost)
%  with the concept
%  $\Diamond_{i}^{+} \exists u.\{a\}$, and to denote at all states with $\Box_{i}^{+} \exists u.\{a\}$.
%      \nb{M: to discuss: remove (covered by reduction in Lemma~\ref{lemma:redtotaltopartial})}
%}
%In the following, we illustrate a polynomial-time reduction of formula
%satisfiability on total modal or temporal interpretations without the
%RDA, to the same problem over partial ones.
Partial interpretations are a generalisation of the classical, total, interpretations, where all nominals designate at all possible worlds. It turns out that satisfiability in partial and total interpretations  are polytime-reducible to each other.
%, as illustrated by the following polynomial-time reduction of satisfiability on total interpretations  to the same problem over partial ones.
%

\begin{restatable}{proposition}{redtotaltopartial}
\label{lemma:redtotaltopartial}
%Let  $\Cmc$ be a class of frames. 
In $\ML^n_{\ALCOu}$ and $\MLALCOud$,
%\nb{M: mention that covers also $\ELOu$ and $\ELOud$? (in Section~\ref{sec:reasontfdl}?)}
total concept $\Cmc$-satisfiability \textup{(}under global ontology\textup{)} is polytime-re\-ducible to 
concept $\Cmc$-satisfiability \textup{(}under global ontology, respectively\textup{)},
 with both  constant and  expanding domains.
\end{restatable}
%

We sketch the proof for the case of global ontology. Let~$\Omc$ be an ontology. Consider the extension $\Omc'$ of $\Omc$ with CIs
$\top \sqsubseteq \exists u. \{ a \}$,
for all individual names $a$ in~$\Omc$. Clearly, these CIs  ensure that each $a$ designates in every accessible world.
%\textcolor{red}{
The case of concept satisfiability is shown in Appendix~B.
%}
%Note that the proof is independent of whether RDA is accepted or not.
%works with and but the interpretation of $a$ can vary across
%the worlds due to the lack of the RDA.
%The same proof, however, works under the RDA: it shows also that total satisfiability with the RDA is polynomial-time reducible to satisfiability with the RDA.
%\nb{move to the statement of proposition}
%\nb{M: is a reduction possible with the RDA?}


%%%OLD VERSION -- FORMULA SATISFIABILITY
%\begin{lemma}
%\label{lemma:redtotaltopartial}
%Total $\MLALCOud$ and $\TLALCOud$ formula satisfiability without the
%RDA are polynomial-time reducible to, respectively, partial
%$\MLALCOud$ and $\TLALCOud$ formula satisfiability without the RDA.
%\end{lemma}
%
%\begin{proof}
%  We adapt, to the $\MLALCOud$ and $\TLALCOud$ cases, the reduction of
%  $\ALCOud$ ontology satisfiability and entailment from total to
%  partial interpretation, given in~\cite{ArtEtAl21a}.
%%Remark~\ref{rem:redtotpart}
%%of Section~\ref{sec:observations}.
%  In particular, given an $\MLALCOud$ or $\TLALCOud$ formula $\p$, we
%  define $\p'$ as the conjunction of $\p$ with formulas of the form
%  \nb{M: todo fix - modal depth}
%\begin{equation}
%\label{eq:designate}
%\tag{$\ast$}
%\Box^{+} ( \top \sqsubseteq \exists u.\{a\}),
%\end{equation}
%%
%for every individual name $a$ occurring in $\p$.  It can be seen that
%$\p$ is satisfiable on \emph{total} modal or temporal interpretations
%without the RDA iff $\p'$ is satisfiable on \emph{partial} modal or
%temporal interpretations without the RDA, respectively.  Observe that,
%despite the fact that each individual name $a$ occurring in $\p$ is
%forced by~(\ref{eq:designate}) to denote at every world or instant of
%any model of $\p'$, its interpretation is allowed to vary across
%states, due to the lack of the RDA.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{Reduction of partial to total satisfiability}
Next, we provide the converse reduction. 
%showing that concept satisfiability (under global ontology)
%on
%partial
%interpretations
%without the RDA
%is polynomial-time reducible to the same problem over
%total
%interpretations.
%without the RDA.

\begin{restatable}{proposition}{redpartialtototal}
\label{lemma:redpartialtototal}
%Let  $\Cmc$ be a class of frames. 
In $\ML^n_{\ALCOu}$ and $\MLALCOud$,
concept $\Cmc$-satisfiability \textup{(}under global ontology\textup{)} is polytime-reducible to total
concept $\Cmc$-satisfiability \textup{(}under global ontology, respectively\textup{)},
with both constant and expanding domains.
\end{restatable}
%
We again sketch the proof for the case of global ontology. Let $\Omc$ be an ontology. Consider $\Omc'$ obtained from $\Omc$ by replacing every nominal~$\{ a \}$ in~$\Omc$ with a fresh concept name
$N_{a}$ and by extending the result with all CIs
$N_a \sqsubseteq \{ a \}$. It follows that every $a$ in $\Omc'$ can designate in all worlds, but the corresponding concept $N_a$ may still be interpreted by the empty set in some worlds, thus reflecting the fact that $a$ in $\Omc$ could have failed to designate in those worlds.
The case of concept satisfiability is dealt with in Appendix~B.
%\nb{this fails in expanding domains with RDA}
%{\color{blue}{Observe\nb{M: check + move to Appendix?} that the proof above fails if we try to obtain a reduction to total concept $\Cmc$-satisfiability \emph{with the RDA} and \emph{expanding domains}.
%}
%}


%\textcolor{red}{M: mention that it does not cover $\ELOu$ and $\ELOud$? (in Section~\ref{sec:reasontfdl}?)\\R: for the entailment problem? Satisfiability in EL is trivial (no $\bot$); also does not seem to be an issue under the global ontology}


%\paragraph{Reduction of concept satisfiability}

%\begin{remark}
%\label{rem:concsattoconcsatglobont}
%Partial (resp., total) concept satisfiability is polynomial-time reducible to partial (resp., total) concept satisfiability under global (empty) ontology.
%\nb{M: add/remove (obvious) remark on reduction of concept sat to concept sat under global (empty) ontology?}
%\end{remark}









\paragraph{Normal Form for Ontologies and Concepts}
Next,
we define normal form that will help us prove further polytime reductions, e.g., Lemma~\ref{lemma:spy-point-reduction} and Proposition~\ref{lemma:redmludtomlu}, and then complexity upper bounds.
Let $\Omc$ be an ontology  and  $C$ a subconcept in $\Omc$. Denote by $\Omc[C/A]$ the result of replacing every occurrence of~$C$ in $\Omc$ with a fresh concept name $A$, called the \emph{surrogate} of $C$. Clearly, $\Omc[C/A]\cup \{ C \equiv A\}$ is a model conservative extension of~$\Omc$. We can systematically apply this procedure to obtain an ontology in \emph{normal form} where connectives are applied only to concept names: e.g., definite descriptions occur only in the form of $\defdes B$, for a concept name~$B$.  If surrogates are introduced for innermost connectives first, then the transformation runs in polytime.

\begin{restatable}{lemma}{ontologynormalform} 
\label{lemma:ontology:normal-form}
For any $\MLALCOud$ ontology $\Omc$, we can construct in polytime an $\MLALCOud$ ontology $\Omc'$ in normal form that is a model conservative extension of $\Omc$. Moreover, $\Omc'$ uses the same set of connectives as $\Omc$.
\end{restatable}
%

If the language contains the universal role, then a similar construction transforms concepts $D$ into normal form. For a single modality ($n=1$), we can use $\Box_1^{k} \forall u.(C \Leftrightarrow A)$, for all $k \leq \md(D)$.  If $n > 1$, then we need to carefully select sequences of boxes to avoid an exponential blowup. So, for an $\MLALCOud$ concept $D$ and its subconcept $C$, we define the set of \emph{$C$-relevant paths in $D$},
denoted by $\rpath(D, C)$,
as the sequences $(i_1,\dots, i_n)$ of the $\Diamond_{i_j}$ operators under which $C$ occurs in~$D$. For example, for $D = \Diamond_1\neg A \sqcap \Diamond_2\Diamond_3 A$, we have $\rpath(D, A) =  \{(1), (2, 3) \}$ and $\rpath(D, \neg A) = \{(1)\}$.
%%
%\begin{align*}
%\rpath(A, A) & = \{\epsilon\},\\ 
%\rpath(\neg A, A) & = \{\epsilon\},\\
%\rpath(\Diamond_3 A, A) & = \{(3)\},\\
%\rpath(\Diamond_2\Diamond_3 A, \Diamond_3 A) & = \{(2)\},\\
%\rpath(\Diamond_2\Diamond_3 A, A) & = \{(2, 3)\},\\
% \rpath(\Diamond_1 \neg A, A) & = \{(1)\},\\
% \rpath(\Diamond_1 \neg A\sqcap \Diamond_2\Diamond_3 A,  A) & = \{(1), (2, 3) \},\\
% \rpath(\Diamond_1 \neg A\sqcap \Diamond_2\Diamond_3 A, \neg A) & = \{(1) \}. 
% \end{align*}
 %
Note that the maximum length of a path in $\rpath(D, C)$ is $\md(D)$.
% \textcolor{red}{and that $\bigcup_{C \in \sub{D}} \rpath(D, C)$ is closed under taking prefixes.}
We also define the `$\Box$-modality' for each path: %referring to the $C$-relevant paths in $D$: 
for a concept $E$, we recursively define
%
\begin{equation*}
	\Box^{\epsilon} E  = E  \text{ and } \Box^{i \cdot \pi} E =  \Box_{i} \Box^{\pi} E, \text{ for any path } \pi.
\end{equation*}
%
As before,  the \emph{surrogate} of $C$ is  a fresh concept name $A$, and $D[C/A]$ denotes the result of replacing~$C$ with $A$ in $D$.
%We now show the following lemma.

%Let $D$ be a concept, $C$ its subconcept and $A$ a fresh concept name. Denote by $D[C/A]$ is the result of replacing $C$ with  $A$ in $D$.
%%We show that
%the conjunction $D'$  of $D[C/A]$ and all 
%%
%\begin{equation*}
%\Box^\pi \forall u.(A \Rightarrow C) \text{ and } \Box^\pi \forall u.(C \Rightarrow A), \text{ for } \pi \in \rpath(D, C), 
%\end{equation*}
%%
%is a model conservative extension of $D$.

\begin{restatable}{lemma}{normalformconc}
\label{lem:normalformconc}
Let $D$ be an $\MLALCOud$ concept and $C$ its subconcept. 
Denote by $D'$  the conjunction of $D[C/A]$ and
%
\begin{equation}
\label{eq:normalformconj}
\Box^\pi \forall u.(C \Leftrightarrow A), \text{ for all } \pi \in \rpath(D, C).
\end{equation}
%
Then $D'$ is a model conservative extension of $D$. Moreover,
$\rpath(D', A) = \rpath(D, C)$ and $\rpath(D', E) = \rpath(D, E)$, for any subconcept $E$ of $C$.
\end{restatable}


For any concept $D$, by repeatedly replacing non-atomic subconcepts with their surrogates, one can obtain a concept $D^{\ast}$ in \emph{normal form}, which is a conjunction of a concept name and concepts of the form~\eqref{eq:normalformconj}. By Lemma~\ref{lem:normalformconc}, $D^{\ast}$ is a model conservative extension of~$D$. Moreover, if  surrogates are introduced  for innermost  non-atomic concepts first, the procedure runs in polytime in the size of $D$.



\paragraph{Spy Points: Eliminating the Universal Role}
Our next observation allows us to eliminate occurrences of the universal role from ontologies. % (it again does not depend on RDA).

\begin{restatable}{lemma}{spypointreduction}
\label{lemma:spy-point-reduction}
Let $\Omc$ be an $\MLALCOud$ ontology in normal form. Denote by $\Omc'$ the $\MLALCOd$ ontology obtained from $\Omc'$ by replacing
%
\begin{itemize}
\item each CI of the form $B \sqsubseteq \exists u.B'$ with $B \sqsubseteq \exists r.B'$, and
\item each CI of the form $\exists u.B \sqsubseteq B'$ with the following:
% \neg B' \sqsubseteq \forall u.\neg B
%
\begin{equation*}
\top  \sqsubseteq \exists r.\{e\},\ \  A \sqsubseteq \{e\}, \ \
\neg B'  \sqsubseteq \exists r.A, \ \
\exists r.A \sqsubseteq \neg B, 
\end{equation*}
%
\end{itemize}
%
where $r$, $e$ and $A$ are fresh role, nominal and concept names, respectively. % 
Then $\Omc'$ is a model conservative extension of~$\Omc$, and the size of $\Omc'$ is linear in the size of $\Omc$.
\end{restatable}
%
Intuitively, positive occurrences of $\exists u.B'$ ensure that $B'$ is non-empty, which can also be achieved with a fresh role~$r$. For negative occurrences of $\exists u.B'$, we use a spy-point $e$, which is accessible, via a fresh $r$, from every domain element and belongs to $A$ whenever $\neg B'$ is non-empty (that is, whenever $B'$ does not coincide with the domain). If this is the case, then no domain element can be in~$B$, which, by contraposition, implies $\exists u.B\sqsubseteq B'$. Note that $e$ can be rigid.






























\paragraph{From Nominals to Definite Descriptions and Back}

%\paragraph{Nominals without RDA to Definite Descriptions}

%\textcolor{red}{say that in a language without nominals, the RDA and totality are trivial}
%\nb{M: to discuss (we might introduce assertions and formulas as primitive, and then satisfy  $\Box C(a) \land \Diamond  (\lnot C(a))$
%without the RDA and
%$\lnot (A(a)) \land \lnot (\lnot A(a))$
%without totality (but with totality issue we enter a mess)}
We first observe that nominals can be easily encoded with definite descriptions. Indeed, given an ontology $\Omc$, take a fresh concept name $N_{a}$ for each individual name $a$ in~$\Omc$, and let $\Omc'$ be the result of replacing every occurrence of $\{ a \}$ in~$\Omc$
with~$\{ \defdes N_{a} \}$. Clearly, $\Omc'$ is a model conservative extension of $\Omc$,
and vice versa.
Note that $\Omc'$ is in the fragment $\MLALCud$ without nominals, which 
has no distinction 
between partial and total interpretations,
and
between the RDA and no-RDA cases.
Thus, we have the following result.
%
\begin{restatable}{proposition}{nomnonrdatodefdes}
\label{prop:nomnonrdatodefdes}
%Let  $\Cmc$ be a class of frames. 
In $\ML^n_{\ALCOu}$ and $\MLALCOud$,
concept $\Cmc$-satisfiability \textup{(}under global ontology\textup{)} is polytime-reducible to
$\MLALCud$ concept $\Cmc$-satisfiability \textup{(}under global ontology, respectively\textup{)},
with both constant and expanding domains.
%\nb{M: mention that covers also $\ELOu$ and $\ELOud$? (in Section~\ref{sec:reasontfdl}?)}
\end{restatable}
%





Conversely,
%In the converse direction,
we now show how to replace definite
descriptions $\iota C$ with nominals using the universal role.
%, hence reducing the 
%satisfiability
%problem in $\MLALCOud$ to
%satisfiability
%in $\MLALCOu$.

%\nb{M: keep this Lemma}

\begin{restatable}{proposition}{redmludtomlu}
\label{lemma:redmludtomlu}
%Let  $\Cmc$ be a class of frames. 
$\MLALCOud$ concept $\Cmc$-satisfiability \textup{(}under global ontology\textup{)} is polytime-reducible to
%\nb{removed: total \\ M: ok but in proof of Thm. 11 added ref. to Prop. 5}
$\MLALCOu$
concept $\Cmc$-satisfiability \textup{(}under global ontology, respectively\textup{)},
with both constant and expanding domains.
\end{restatable}
%
The proof reduces the total $\Cmc$-satisfiability problems in $\MLALCOud$ to total $\Cmc$-satisfiability in $\MLALCOu$, which, by Propositions~\ref{lemma:redpartialtototal} and \ref{lemma:redtotaltopartial} gives us the required result. We sketch the case of the global ontology. By Lemma~\ref{lemma:ontology:normal-form}, we can assume that the given $\Omc$ is in normal form. Let $\Omc\red$ be the result of replacing each $A_{\{ \defdes  B \}} \equiv \{\defdes B\} $ in $\Omc$ with CIs
%
\begin{equation*}
A_{\{\defdes B\}} \sqsubseteq B\sqcap \{a_B \} \text{ and } B \sqcap \forall u.(B\Rightarrow \{a_B\}) \sqsubseteq A_{\{\defdes B\}}, 
%\}.
\end{equation*}
%
where $a_B$ is a fresh individual name. Intuitively, the first CI ensures that the surrogate for $\{\defdes B\}$ belongs to $B$ and is never interpreted by more than one domain element. The second CI ensures that if $B$ is a singleton, then that element belongs to the surrogate for $\{\defdes B\}$. Formally, we show that $\Omc\red$ is a model conservative extension of $\Omc$.
The case of concept satisfiability relies on normal form of concepts (Lemma~\ref{lem:normalformconc}) and is treated in Appendix~B.


%\textcolor{red}{M: mention that it does not cover $\ELOu$ and $\ELOud$? (in Section~\ref{sec:reasontfdl}?)}







\paragraph{Expanding to Constant Domains}

It is known that, for the satisfiability problems, the interpretations with expanding domains can be simulated by constant domain interpretations, where a fresh concept name representing the domain is used to relativise concepts and CIs; see e.g.,~\cite[Proposition 3.32~(ii), (iv)]{GabEtAl03}. We restate this standard result in our setting for completeness:
%\nb{M: to discuss: enough total int. without $\defdes$?}
%
\begin{restatable}{proposition}{redexptoconst}
\label{prop:redexptoconst}
%Let  $\Cmc$ be a class of frames. 
In $\ML^n_{\ALCOu}$
%\nb{added the language with $\iota$ }
and $\MLALCOud$,
concept  $\Cmc$-satisfiability \textup{(}under global ontology\textup{)} with expanding domains is polytime-re\-ducible to concept $\Cmc$-satisfiability \textup{(}under global ontology, respectively\textup{)} with constant domain.
\end{restatable}

In the sequel,
we implicitly  adopt  the \emph{constant domain assumption}~\cite{GabEtAl03}, and explicitly write when we consider interpretations with expanding domains instead.



















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "rda"
%%% End:

==> camera-ready/4-ml-reasoning.tex <==
% !TEX root =  rda.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Non-Rigid Designators and Counting}
\label{sec:counting}

%{\bf First option.}

%Define the formulas $\varphi$ of FOML$_{n}^{\not=}$ by setting follows: 
%\begin{gather*}
%	\varphi ::= A(x) \mid \neg\varphi \mid \varphi \wedge \psi \mid \exists x \varphi \mid \exists^{\leq 1}\varphi \mid \Diamond_{i} \varphi
%\end{gather*}
%where $A$ ranges over an infinite set of monadic predicate symbols which, for simplicity, we identify 
%with the set $\NC$ of concept names. FOML$_{n}^{\not=}$
%is interpreted in modal models $\Mmf$ (in which the interpretation of role and individual names is not relevant). Given a valuation $\mathfrak{v}$ of $x$ into $\Delta_{w}$ with $w$ a root of $\Mmf$ we set
%\begin{itemize}
%	\item $\Mmf,v\models_{\mathfrak{v}} A(x)$ iff $v(x)\in P^{\Imc_{v}}$;
%	\item etc.
%\end{itemize}  


%{\bf Second Option}

%Alternative formulation with description logic operators $\exists^{\not=}u.C$ (``elsewhere''). Denote this language $\mathcal{ML}_{\text{Diff}}^{n}$
	
\newcommand{\MLDiff}{\mathcal{ML}_{\text{\textup{Diff}}}^{n}}	
	
We prove a strong link between non-rigid designators and the first-order one-variable modal logic enriched with the `elsewhere' quantifier, $\MLDiff$, introduced and investigated in~\cite{DBLP:conf/aiml/HampsonK12,HamKur15,DBLP:conf/aiml/Hampson16}. We define $\MLDiff$ using DL-style syntax: concepts in $\MLDiff$ are of the form 
%
\begin{equation*}
  C ::= A \mid \lnot
  C \mid (C \sqcap C)
\mid \exists u.C
\mid \exists^{\ne} u.C
\mid \Diamond_i C,
\end{equation*}
%
where $i\in I$. Observe that the language has no terms and no roles apart from the universal role $u$. 
All constructs are interpreted as before,
with the addition of
%and 
%
\begin{align*}
  (\exists^{\ne} u.C)^{\Imc_{w}} &= \bigl\{ d \in \Delta^w \mid 
  C^{\Imc_{w}} \setminus \{ d \} \ne \emptyset
  \bigr\}.
\end{align*}
%
Note that our language contains existential quantification, which in~\cite{HamKur15} is introduced as an abbreviation for $C \sqcup \exists^{\ne} u.C$. In fact,
$\MLDiff$ can be regarded as a basic first-order modal logic with counting because the counting quantifier $\exists^{=1}u.C$ (`there is exactly one $C$') with
\begin{align*}
	(\exists^{=1} u.C)^{\Imc_{w}} &= \bigl\{ d \in \Delta^w \mid 
	|C^{\Imc_{w}}|=1\bigr\}
\end{align*}
%
is clearly logically equivalent to the  $\MLDiff$-concept \mbox{$\exists u.(C \sqcap \neg \exists^{\ne}u.C)$}. Conversely, $\exists^{\ne}u.C$ is logically equivalent to
$\exists u.C\sqcap (C \Rightarrow \neg \exists^{=1} u.C)$.
%$(\exists^{=1}u.C \sqcap \neg C) \sqcup (\neg \exists^{=1}u.C \sqcap \exists u.C)$ 
So, one could replace $\exists^{\ne}$ by $\exists^{=1}$ in the definition $\MLDiff$ and obtain a logic with exactly the same expressive power.


%	
\begin{restatable}{theorem}{diff}
\label{th:diff}
%
%Let $\Cmc$ be a class of frames. 
%	
\textup{(1)} $\Cmc$-satisfiability of $\MLALCOu$-concepts \textup{(}under global ontology\textup{)}
	can be reduced in double exponential time to $\Cmc$-satisfiability of $\MLDiff$-concepts \textup{(}under global ontology, respectively\textup{)}, with both constant and expanding domains. 
	
\textup{(2)} Conversely, $\Cmc$-satisfiability of $\MLDiff$-concepts \textup{(}under global ontology\textup{)} is polytime-reducible to $\Cmc$-satisfiability of $\MLALCOu$-concepts \textup{(}under global ontology, respectively\textup{)},  with both constant and expanding domains. 
\end{restatable}
%    
We\nb{an alternative version} first give the main ingredients for the proof of Item~(1) with global ontology~$\Omc$. If $\Omc$ contains no roles apart from $u$, then we introduce a surrogate concept name $\{a\}^\sharp$ for each individual name $a$ in $\Omc$ and denote by $\Omc^\sharp$ the result of replacing each $\{a\}$ with $\{a\}^\sharp$ and then extending the ontology with CIs of the form $\top \sqsubseteq \exists^{=1} \{a\}^\sharp$. The resulting $\MLDiff$ ontology $\Omc^\sharp$ is clearly a model conservative extension of~$\Omc$, which completes the reduction. If, however, $\Omc$ contains role names, then we apply the quasimodel technique~\cite{GabEtAl03} to deal with binary relations (roles), whose interpretations in different worlds are independent from each other. This technique is also used in Sections~\ref{sec:reasoning} and~\ref{sec:reasontfdl}. In quasimodels, each DL interpretation is represented as a \emph{quasistate}, which is a non-empty set of \emph{types}, maximal consistent sets of subconcepts of $\Omc$ and their negations: each type~$\contp$ represents all domain elements satisfying the concepts in~$\contp$. 
In this proof, we can characterise  possible quasistates for $\Omc$  using concepts: the \emph{description} $\Xi_{\settp}$ of a quasistate $\settp$ is  
%
\begin{equation*}
\forall u.\bigsqcup_{\contp\in\settp} \contp \ \ \sqcap \ \ \bigsqcap_{\contp\in\settp}  \exists u.\contp,
\end{equation*}
% 
where $\contp$ is the conjunction ($\sqcap$) of all concepts $C\in\contp$. The set $\Smc_\Omc$ of quasistates that can possibly occur in interpretations satisfying $\Omc$ can be obtained by checking whether the \emph{modal abstraction} $\Xi_{\settp}^\ast$ of its description $\Xi_{\settp}$  is satisfiable, where $\cdot^\ast$ is the result of replacing subconcepts starting with a modal operator by fresh concept names. Since satisfiability of $\ALCOu$-concepts under $\ALCOu$ ontologies is in \textsc{ExpTime}, the set~$\Smc_\Omc$ can be computed in double exponential time. In order to ensure that quasistates fit together to form a representation of an interpretation satisfying $\Omc$, we use the \emph{DL-abstraction} $\cdot^\sharp$ described above, except that now we replace not only nominals but also existential restrictions with fresh concept names. We construct $\MLDiff$-ontology $\Omc^\sharp$ by replacing CIs $C\sqsubseteq D$ in $\Omc$ with $C^\sharp\sqsubseteq D^\sharp$ and extending the result with CIs  $\top\sqsubseteq \bigsqcup_{\settp\in \Smc_\Omc} \Xi_{\settp}^\sharp$  and  $\top \sqsubseteq \exists^{=1} \{a\}^\sharp$, for all individual names $a$. Then we show that $A$ is $\Cmc$-satisfiable under $\Omc$ iff $\contp^\sharp$ is $\Cmc$-satisfiable under $\Omc^\sharp$, for some type $\contp$ containing~$A$. 
See Appendix~C for full details and the case of concept satisfiability (without ontology).

%The proof of (1) and proofs in Sections~\ref{sec:reasoning} and~\ref{sec:reasontfdl} use \emph{types}~$\contp$, sets of (negated) subconcepts of the input concept (and ontology) such that, for any subconcept $C$, either $C\in \contp$ or $\neg C\in \contp$.\nb{comment on the closure under $\sqcap$?} A \emph{quasistate} $T$ is a set of types and stands for a world satisfying exactly the types in $T$~\cite{GabEtAl03}. Given a quasistate $T$, one can check in polytime whether its \emph{non-modal abstraction}, obtained by replacing all concepts starting with a modal operator by a concept name, is satisfiable in a DL interpretation. On the other hand, assuming that $\mathcal{C}$-satisfiability of $\MLDiff$-concepts
%is decidable, one can check whether its \emph{non-DL abstraction}, in which existential restrictions and nominals are replaced by concept names, is satisfiable in a $\MLDiff$ model in which the concept names replacing nominals are interpreted as singletons.  As observed above, to enforce interpretation of a concept name $A$ as a singleton in all worlds one can use the $\MLDiff$ CI $\top \sqsubseteq \exists^{=1}u.A$. For concept satisfiability (without ontology) one makes the same statement for all worlds reachable along relevant paths. The reduction is now implemented using both abstractions. It requires double exponential time because the number of quasistates is double exponential in the size of the input. 

Item (2) is proved by lifting to the modal description logic setting the observation of \citeauthor{DBLP:journals/jphil/GargovG93}~(\citeyear{DBLP:journals/jphil/GargovG93}) that the difference modality and nominals are mutually interpretable by each other; see the equivalences that show the same expressive power of $\exists^{\ne}$ and $\exists^{= 1}$.

Using Theorem~\ref{th:diff}, one can transfer a large number of (un)decidability results and lower complexity bounds from first-order modal logics with `elsewhere' to modal DLs with non-rigid designators; see, e.g., Theorem~\ref{thm:k:global:sat} in Section~\ref{sec:reasoning}. Conversely, the results proved below entail new results for first-order modal logics with `elsewhere' and/or counting.

%{\color{red} 
%	
%	According to \cite{DBLP:conf/aiml/Hampson16} we have upper complexity bounds for $\K$, S5, Alt with elsewhere. 
%	
%	Hampson poses the question whether these decidability can be extended to monodic fragments. In this paper we show that this is indeed the case.    
%}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reasoning in Modal Free Description Logics}
\label{sec:reasoning}
%
%
%\begin{table*}[t] % put at top of page if possible 
%\centering
%	\begin{tabular}{l|c|c|c|c}
%	        & \multicolumn{2}{c|}{concept satisfiability} &  \multicolumn{2}{c}{concept sat. under global ontology}\\
%		\mbox{}\hfil modal logic $L$ & const.\ domain & exp.\ domains & const.\ domain & exp.\ domains  \\
%		\hline
%		$\K^n$, $n \geq 1$ & NExp-c & NExp-c & undec. & ? \\[4pt]
%		$\Sfive$, $\KDfourfive$ & NExp-c & NExp-c & NExp-c & NExp-c \\
%		$\Sfive^{n}$, $\KDfourfive^{n}$, $n\geq 2$ & NExp-c & NExp-c & undec. & undec. \\[4pt]
%%		$\KDfourfive$ & NExp-c & NExp-c & NExp-c & NExp-c \\
%		$\Kfour$ & ? & ? & ? & ?\\
%		$\Kfour^{n}, n\geq 2$ & ? & ? & undec. & ?\\[4pt]
%		$\GL$, $\Grz$ & ? & decidable & ? & decidable\\
%%		$\K^{n}, n\geq 1$ & NExp-c & NExp-c & undec & undec. \\
%%		$\KDfourfive_{n}, n\geq 2$ & NExp-c & NExp-c & undec & undec\\
%		$\GL^{n}$, $\Grz^{n}$, $n\geq 2$ & ? & ? & undec. & ?
%	\end{tabular}
%	\caption{Concept satisfiability (under global ontology) for $L_{\ALCOud}$ and $L_{\ALCOu}$}\label{table:complexity}
%\end{table*}

The aim of this section is to show the results presented in Table~\ref{table:complexity} and also discuss a few related logics.
For some basic frame classes, it will be convenient to use standard modal logic notation when discussing the satisfiability problem.
So, given a propositional modal logic $L$ with $n$ operators and a DL fragment $\DL$, the problem of  
\emph{$L_{\DL}$ concept satisfiability} (\emph{under global ontology}) is the
 problem of deciding $\mathcal{C}_{L}$-satisfiability of $\mathcal{ML}^{n}_{\DL}$-concepts \textup{(}under global ontology, respectively\textup{)}, where $\mathcal{C}_{L}$ is the class of all frames validating $L$.  We focus on the modal logics $L$ characterised by the following classes $\Cmc_L$ of frames, with $n \geq 1$:
 %
\begin{description}
\item[$\K^n$\textnormal{:}] $\Cmc_L$ is the class of all frames $(W,R_1,\dots,R_n)$;
%\item for $L = \KDfourfive$, $\mathcal{C}_{L}$ is the class of all %frames $(W,R)$ such that $R$ is serial, transitive, and Euclidean;
\item[$\Sfive^n$\textnormal{:}] $\Cmc_L$ is the class of all frames $(W,R_1,\dots,R_n)$ such that the $R_i$ are equivalence relations;
%\emph{reflexive}, \emph{transitive}, and \emph{symmetric}
%(i.e., an \emph{equivalence})
%\item for $L = \Kfour$, $\mathcal{C}_{L}$ is the class of all frames %$(W,R)$ such that $R$ is a transitive relation;
%\item for $L = \GL$, $\mathcal{C}_{L}$ is the class of all frames %$(W,R)$ such that $R$ is transitive, irreflexive, and %\emph{Noetherian} (there is no infinite chain $x_{0}Rx_{1}R\cdots$ %with $x_{i}\not=x_{i+1}$);
%\item for $L = \Grz$, $\mathcal{C}_{L}$ is the class of all frames %$(W,R)$ such that $R$ is transitive, reflexive, and Noetherian.
\item[$\K^{\ast n}$\textnormal{:}] $\Cmc_L$ is the class of all frames $(W,R_{1},\ldots,R_{n},R)$ such that $R$ is the transitive closure of $R_{1}\cup\cdots \cup R_{n}$;
\item[$\Kfn$\textnormal{:}] $\Cmc_L$
is as for $\K^{\ast n}$ and, in addition, $W$ is finite and $R$ is irreflexive (in other words, there are no chains $w_{0}R_{i_{1}}w_{1}\cdots R_{i_{n}}w_{n}$ with $w_{0}=w_{n}$).
\end{description}
%For any $L$ with one modal operator and $n\geq 1$ we denote by $\mathcal{C}_{L^{n}}$ the class of frames $(W,R_{1},\ldots,R_{n})$ such that $(W,R_{i})\in \mathcal{C}_{L}$ for $1\leq i \leq n$.


%\color{blue}%
To illustrate the language $\Sfive^{2}_{\ALCOud}$, we express that Agent 2 \emph{knows that} Agent 1 does \emph{not know of} the General Chair of KR 2024 that they are the General Chair of the KR Conference held in Southeast Asia:
\begin{multline*}
\Box_{2} \exists u. (
\{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \} \sqcap
\lnot \Box_{1} \{ \defdes \exists \mathsf{isGenChair}. \\ \{ \defdes ( \mathsf{KRConf} \sqcap \exists \mathsf{hasLoc}.\mathsf{SEAsiaLoc}) \} \}  ).
\end{multline*}%
%or, to stress the scope distinctions for $\Box_{1}$ and $\Box_{2}$, as:
%\begin{multline*}
%\Box_{2} [
%\lnot \Box_{1} \{ \defdes \exists \mathsf{isGenChair}.  \{ \defdes ( \mathsf{KRConf} \sqcap \\ \exists \mathsf{hasLoc}.\mathsf{SEAsiaLoc}) \} \} (\{ \defdes \exists \mathsf{isGenChair}. \{ \mathsf{kr24} \} \} )].
%\end{multline*}
%\color{black}


The two main new results in Table~\ref{table:complexity} are the \NExpTime{} upper bound for $\K^{n}$ and $\Sfive^{n}$ and decidability of $\Kfn$. The remaining results are by (sometimes non-trivial) reductions to known results.
\begin{restatable}{theorem}{modconcdec}
	\label{thm:modconcdec}
	For $L\in \{ \K^{n},\Sfive^{n} \}$ with $n \geq 1$, $L_{\ALCOud}$
	concept
	satisfiability 
	is in $\NExpTime$ with both constant and expanding domains.
\end{restatable}
We provide a sketch of the main ideas of the proof for $\Sfive^{n}$.
First, observe  (using an unfolding argument) that any satisfiable concept $C$ is satisfied in world $w_{0}$ in a model based on a frame $\mathfrak{F}=(W,R_{1},\ldots,R_{n})$ such that the domain $W$ of $\mathfrak{F}$ is a prefix-closed set of words of the form 
%
\begin{equation*}%\label{eq:world}
	\avec{w}=w_{0}i_{0}w_{1}\cdots i_{m-1}w_{m},
\end{equation*}
%
where $1\leq i_{j}\leq n$, $i_{j}\not=i_{j+1}$, and each $R_{i}$ is 
the smallest equivalence relation containing all pairs of the form $(\avec{w},\avec{w}iw)\in W\times W$. One can assume that $m$ is smaller than the modal depth of $C$. Next, one can substitute the first-order domain by quasistates (as introduced in Section~\ref{sec:counting}) and work with \emph{quasimodels} $\Qmf = (\mathfrak{F}, \funcand, \runs)$, in which $\funcand$ associates a quasistate with any world, and a set of \emph{runs} $\runs$ represents first-order domain elements as functions mapping every world $w$ to a type in $\funcand(w)$; note that runs were implicit in the proof of Theorem~\ref{th:diff} and could be defined as the domain elements in the interpretations for $\MLDiff$. If $\contp\in \funcand(w)$ contains a nominal, there is only one $r\in \runs$ with $r(w)=\contp$; this condition\nb{added \\ M: clarify?} was expressed by the  CIs of the form~$\top\sqsubseteq \{a\}^\sharp$. Now, one can apply selective filtration and some surgery to such a quasimodel
in order\nb{M: added `in order'}
to obtain a quasimodel
%\nb{cut  `of the above form'}
with at most exponential outdegree (and so of at most exponential size), from which one can then extract
%\nb{replaced  `reconstruct'}
a model of exponential size. 
%
\begin{restatable}{theorem}{moddickson}
	\label{thm:moddickson}
$\Kfn_{\ALCOud}$ concept
	satisfiability under global ontology is decidable with expanding domains,
	 for $n\geq 1$.
\end{restatable}
The proof is again based on appropriate quasimodels, which are now based on expanding domain models using finite frames $\mathfrak{F}=(W,R_{1},\ldots,R_{n},R)$ such that the transitive closure $R$ of $R_{1}\cup \cdots \cup R_{n}$
%\nb{added second $\cup$ and $R$}
contains no cycles. Unfolding shows that we may assume
that $(W,R)$ is a forest. We show decidability by proving a recursive bound on the size of these models. Let
%\nb{added}
$\extN = \mathbb{N}\cup \{\infty\}$, where we assume  $m \leq \infty$ and $m + \infty = \infty$, for all $m\in\extN$.
We fix an ordering $\contp_{1},\ldots,\contp_{k}$ of the types and represent a quasistate as a vector $(x_{1},\ldots,x_{k})\in \extN^{k}$, where $x_{i}$ is the number of domain elements that satisfy type $\contp_{i}$ in a world (equivalently, the number of runs through $\contp_{i}$). Let $|\avec{x}|=x_{1}+\cdots + x_{k}$
for $\avec{x}=(x_{1},\ldots, x_{k})\in\extN^k$. Observe that expanding domains correspond to the condition that $wR_{i}v$ implies $|\avec{x}| \leq |\avec{y}|$,
%\nb{more detailed explanation}
where  $\funcand(w), \funcand(v)$ are represented by $\avec{x}, \avec{y}\in\extN^k$, respectively. 
To obtain a recursive bound on the size of a finite model satisfying a concept we then apply Dickson's Lemma to the quasistates. Define the product ordering $\leq$ on $\extN^{k}$ by setting $\avec{x}\leq \avec{y}$ if $x_{i}\leq y_{i}$ for all $1\leq i \leq k$, where $\avec{x}=(x_{1},\ldots,x_{k})$ and $\avec{y}=(y_{1},\ldots,y_{k})$. 
A pair $\avec{x},\avec{y}$ with $\avec{x} \leq \avec{y}$ is called an \emph{increasing pair}. Dickson's Lemma states every infinite sequence $\avec{x}_{1},\avec{x}_{2},\ldots\in \extN^{k}$ contains an
increasing pair $\avec{x}_{i_{1}},\avec{x}_{i_{2}}$ with $i_{1}<i_{2}$.
In fact, assuming $|\avec{x}_{i}|\leq |\avec{x}_{i+1}|$ for all $i\geq 0$ and
given recursive bounds on $|\avec{x}_{1}|$ and
$|\avec{x}_{i+1}|-|\avec{x}_{i}|$, one can compute a recursive
bound on the length of the longest sequence without any increasing pair~\cite{DBLP:conf/lics/FigueiraFSS11}. Now, the proof of a recursive bound
on the size of a satisfying model consists in manipulating the quasimodel so that the outdegree of the forest is recursively bounded and Dickson's Lemma becomes applicable. The expanding domain assumption is crucial for this.  
 
We comment on the remaining results in Table~\ref{table:complexity}.
The $\NExpTime$-hardness results already hold without nominals~\cite[Theorem 14.14]{GabEtAl03} (the proof goes through also with expanding domain). The lower bounds for $\Kfn$ and $\K^{\ast n}$
follow from the following lemma and the corresponding lower bounds proved in the next section for temporal DLs (Table~\ref{table:complexity:temporal}).   
%
\begin{lemma}\label{lemma:ltl-to-kfn}
Concept satisfiability for $\LTLf_{\ALCOu}$ and $\LTL_{\ALCOu}$ are polytime-reducible to concept satisfiability for $\Kfn_{\ALCOu}$ and $\K^{\ast n}_{\ALCOu}$,
respectively, with and without ontology and with both constant and expanding domains.
\end{lemma}
%
The proof of this reduction from logics of linear frames with transitive closure to logics of branching frames with transitive closure is not trivial but can be done by adapting the reduction given in the proof of Theorem 6.24 in \cite{GabEtAl03} for product modal logics. 

Finally,  undecidability of concept satisfiability under global ontology for $\K^{n}$
%\nb{para changed, theorem added}
with $n \geq 1$ follows from undecidability of  $\MLDiff$~\cite{DBLP:conf/aiml/HampsonK12} using the reduction of Theorem~\ref{th:diff}. The result for  $\Sfive^{n}$ with $n \geq 2$ can be obtained in a similar way, see, e.g.,~\cite{GabEtAl03}.
%\nb{more specific reference for two S5 = K?} 
%Finally, the undecidability of concept satisfiability for $\K^{n}$ and $\Sfive^{n}$ under ontologies with constant domain can be proved in the same way as the undecidability of $\MLDiff$\nb{cut `extended with the universal modality'} over arbitrary frames\nb{cut `shown in'}~\cite{DBLP:conf/aiml/HampsonK12} using the reduction of Theorem~\ref{th:diff}.\nb{new theorem}

\begin{theorem}\label{thm:k:global:sat}
Concept satisfiability under global ontology is undecidable with constant domains for $\Sfive^n_{\ALCOu}$, with $n \geq 2$, and  for $\K^n_{\ALCOu}$ with $n \geq 1$.
\end{theorem}


For many important modal logics the decidability status
of modal DLs with non-rigid designators remains open. Most prominently, for the modal logics of (reflexive) transitive frames ${\bf K4}$ (and ${\bf S4}$, respectively), decidability of concept satisfiability with or without ontologies and with expanding or constant domains is open. As a ``finitary'' approximation and a first step to understand ${\bf K4}$ and ${\bf S4}$, we prove, as a specialisation of the proof of Theorem~\ref{thm:moddickson}, decidability of concept satisfiability for the G\"odel-L\"ob logic $\GL_{\ALCOud}$ ($\GL$ is the logic of all transitive and Noetherian\footnote{$(W,R)$ is \emph{Noetherian} if there is no infinite chain $w_{0}Rw_{1}R\cdots$ with $w_{i}\not= w_{i+1}$.} frames~\cite{boolos1995logic}) and Grzegorczyk's logic $\Grz_{\ALCOud}$ ($\Grz$
is the logic of all reflexive and transitive Noetherian frames~\cite{grzegorczyk1967some})
in expanding domain models with and without ontologies.
Alternatively, the decidability of concept satisfiability for
$\GL_{\ALCOud}$ and $\Grz_{\ALCOud}$ can be proved by a double-exponential-time reduction (similar to Theorem~\ref{th:diff}) to satisfiability in expanding domain
products of transitive Noetherian frames, which is known to be decidable~\cite{DBLP:journals/apal/GabelaiaKWZ06}.
%
%The decidability of concept satisfiability for
%$\GL_{\ALCOu}$ and $\Grz_{\ALCOu}$ under expanding domains is now a direct consequence of Theorem~\ref{thm:noether} and the decidability results proved for concept satisfiability in $\mathcal{ML}^{n}_{lin}$ in~\cite{DBLP:journals/apal/GabelaiaKWZ06}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "rda"
%%% End:



==> camera-ready/5-time-reasoning.tex <==
% !TEX root =  rda.tex

%\section{Temporal Free Description Logics}
\section{Reasoning in Temporal Free Description Logics}
\label{sec:reasontfdl}

%\subsection{$\LTLfALCOud$ formula satisfiability}
%on finite traces

In this section, we consider the temporal setting.
For the temporal DL language, we build $\TLALCOud$
\emph{terms}, \emph{concepts}, \emph{concept inclusions} and
\emph{ontologies} similarly to the $\MLALCOud$ case, with $n = 2$: the
language has two modalities --- temporal operators `sometime in
the future', $\Diamond$, and `at the next moment',~$\Next$.
In particular, the $\TLALCOud$ \emph{concepts} are defined by the grammar
%
\begin{gather*}
C ::= A
 \mid \{ \tau \}
 \mid \lnot C
 \mid (C \sqcap C)
\mid \exists r.C
\mid \exists u.C
\mid \Diamond C
\mid \Next C,
%\mid (C \Until C),
\end{gather*}
%
where $\tau$ is a $\TLALCOud$ \emph{term}, defined as in Section~\ref{subsec:ml-nonrig}.
%Similarly, an \emph{$\TLALCOud$ formula} is constructed as follows:
%%
%\[
%\p ::=
%(\alpha)
%\mid \neg \p \mid (\p \land \p)
%\mid \Diamond \p
%\mid \Next \p
%%\mid (\p \Until \p).
%\]
%%
%All the usual syntactic abbreviations are assumed.
%In particular, for temporal concepts, we set:
%$\Diamond C = \top \Until C$ (\emph{eventually});
%$\Diamond^{+} C = C \sqcup \Diamond C$ (\emph{reflexive eventually});
%$\Box C = \lnot \Diamond \lnot C$ (\emph{reflexive always});
%$\Box^{+} C = C \sqcap \Box C$ (\emph{reflexive always});
%$\Next C = \bot \Until C$ (\emph{strong next});
%$\Wnext C = \lnot \Next \lnot C$ (\emph{weak next}).
%Similar abbreviations holds for formulas.
%%\nb{M: add full syntax}



%%% VERSION EXPANDING DOMAIN
%A \emph{flow of time} a frame $\Fmf = (T, <)$, where $T$ is a
%non-empty set of \emph{instants} and $< \ \subseteq T \times T$ is a
%strict linear order on $T$.  
A  \emph{flow of time} $\Fmf$ is a pair $(T, <)$, where $T$ is either the set  $\Nbl$ of 
non-negative integers or a subset of $\Nbl$ of the form $[0, n]$, for $n\in\Nbl$, and $<$ is the strict linear order on $T$. Elements of $T$ are called \emph{instants} (rather than worlds). A flow of time $(T, <)$ naturally gives rise to a frame $(T, <, \textit{succ})$ for  $\TLALCOud$, where $\textit{succ}$ is the successor relation: $\textit{succ} = \{ (t, t+1) \mid t, t+1\in T\}$. So, we will often say that an  interpretation $\Mmf$ is based on a flow $\Fmf$ if its frame is induced by $\Fmf$. We
%\nb{moved here to avoid duplication}
denote it (with an abuse of notation) by
$\Mmf = (\Delta, (\Imc_{t})_{t \in T})$. 
%A \emph{partial temporal interpretation with expanding domains} is a triple
%$\Mmf = ( \Fmf, \Delta, \Int)$, defined as in the modal case.
%We similarly define the notion of \emph{total model with expanding domains}.
If $\Mmf$ is based
on  $(\Nbl, <)$, then we call it an \emph{$\LTLALCOud$  interpretation}; if it is
based on $([0, n], <)$, for some $n\in\Nbl$, it is
called an \emph{$\LTLfALCOud$  interpretation}.
% and often denoted by
%$\Mmf = (\Delta, (\Imc_{t})_{t \in [0, n]})$. %\textcolor{red}{Let $\textbf{Fin}$ be the class of frames based on finite flows of time $([0,n], <)$.?}




Given
%a partial trace
$\Mmf = (\Delta, (\Int_t)_{t\in T})$, the \emph{value} of a $\TLALCOud$ term~$\tau$ at $t\in T$ and
the \emph{extension} of a $\TLALCOud$ concept~$C$ at $t\in T$, are defined
as in the modal case for $n = 2$: in particular, we have
%
\begin{equation*}
  (\Next D)^{\Imc_{t}}  \!=  \begin{cases} D^{\Imc_{t+1}},\hspace*{-0.7em} & \text{if } t + 1 \in T,\\\emptyset, & \text{otherwise},\end{cases} \text{ and }
  (\Diamond D)^{\Imc_t} \! = \hspace*{-1.7em}\bigcup_{t' \in T \text{ with }  t < t'} \hspace*{-1.9em} D^{\Imc_{t'}}.			
\end{equation*}
%
Note that $\Diamond$ is interpreted by $<$ and so
%\nb{replaced `thus'}
does not include the current instant.
%\nb{M: removed $\Diamond^{+}$}
%Note that $\Diamond$ is interpreted by $<$ and thus does not include the current instant, but we also use standard abbreviations $\Diamond^+$ and $\Box^+$, which include the current time instant. 


%%% VERSION -- EXAMPLE OF TL_ALCOu+iota CI
%\nb{M: todo add example}
%{\color{blue}{
%As an example of a $\TLALCOud$ CI, we can express as follows that whoever is a Program Chair of KR will not be Program Chair of KR again, but is always appointed as either the General Chair or a PC member of next year's KR:
%	\begin{multline*}
%\exists {\sf isProgChair}.\{ {\sf kr} \} \sqsubseteq \lnot \Diamond \exists {\sf isProgChair}.\{ {\sf kr} \} \sqcap \\
%							 ( \{ \defdes \exists {\sf isGenChair}. \Next \{ {\sf kr} \} \} \sqcup \exists {\sf isPCMember}. \Next \{ {\sf kr } \} ).
%	\end{multline*}
%}}

%by replacing the semantics of the $\Diamond$
%modal operator with the following one for the $\Until$ temporal
%operator:
%%
%\begin{gather*}
%  (C \Until D)^{\Imc_{t}} = \{ d \in \Delta \mid \text{there is} \
%%			\exists
%			u \in T, t < u \colon d \in D^{\Imc_u} 
%%			\land
%			\ \text{and, for all} \
%%			\forall
%			v \in (t,u)
%%			\colon
%			,
%			d \in C^{\Imc_v}
%		\}
%			.
%\end{gather*}
%
%Similarly, the \emph{satisfaction} of a $\TLALCOud$ formula $\p$ at
%instant $t$ of $\Mmf$ is defined as for the modal case,
%with the following additional clause for the $\Next$ operator:
%%
%\begin{gather*}
%  \Mmf, t \models \Next \psi \ \text{iff} \ t+1 \in T \ \text{and} \ \Mmf, t+1 \models \psi.
%\end{gather*}
%with the following
%semantics of $\Until$ replacing the one for the 
%$\Diamond$ operator:
%%
%\begin{gather*}
%  \Mmf, t \models \p \Until \psi \ \text{iff} \ \text{there is} \
%%	\exists
%	u \in T, t < u \colon \Mmf, u \models \psi
%	\ \text{and, for all $v \in (t,u)$,}\
%%	\forall v \in (t,u) \colon
%	\Mmf, v \models \p.
%\end{gather*}
 
%Other semantic notions are defined as above.

%\ifappendix
%As usual, we use the until operator to define the other temporal
%operators, as follows.
%
%For concepts:
%\emph{(strong) next} operator,
%$\Next C = \bot \Until C$;
%We use the following standard abbreviations:
%\emph{weak next} operator,
%$\Wnext C = \lnot \Next \lnot C$;
%\emph{diamond} operator,
%$\Diamond C = \top \Until C$;
%and \emph{box} operator,
%$\Box C = \lnot \Diamond \lnot C$; \emph{reflexive diamond} operator,
%$\Diamond^{+} C = C \sqcup \Diamond C$; \emph{reflexive box} operator,
%$\Box^{+} C = C \sqcap \Box C$. 
%Similar abbreviations are used for formulas.


%We say that a $\TLALCOud$ formula $\p$ (resp., concept $C$)
%is \emph{satisfied in}
%%\emph{a} ({partial} or {total}) \emph{trace}
%$\Mmf$, if
%$\p$ is satisfied at instant $0$ of $\Mmf$ (resp., $C$ is satisfied at instant $0$ of $\Mmf$).
%$\Mmf, 0 \models \p$ (resp., $C^{\Imc_{0}} \neq \emptyset$).
%We say that a $\TLALCOud$ formula $\p$ (respectively, a concept $C$)
%is \emph{satisfiable on partial (total) traces}, if $\p$
%(respectively, $C$) is satisfied at time $0$ in some partial (total)
%trace $\Mmf$.
%We say that a formula $\p$ (a concept $C$) is \emph{satisfiable on
%  infinite, finite,} or \emph{$k$-bounded traces}, if $\p$ ($C$) is
%satisfied at time $0$ in some infinite, finite, or $k$-bounded trace,
%respectively.
%A $\TLALCOud$ ontology $\Omc$ is \emph{satisfied in}
%%a (partial or total) trace
%\emph{$\Mmf$} if every CI in $\Omc$ is satisfied at instant $0$ of $\Mmf$,
%and it is \emph{globally satisfied} in $\Mmf$ if every CI in $\Omc$ is satisfied at every $t$ of $\Mmf$.
%Moreover, a $\TLALCOud$ formula $\p$ is \emph{entailed under a $\TLALCOud$ ontology $\Omc$} (with respect to partial or total traces, respectively), written $\Omc \models \p$, if,
%for every partial (resp., total) trace $\Mmf$ and every $t$ of $\Mmf$, we have that $\p$ is satisfied at $t$ whenever $\Omc$ is satisfied at $t$.
%%every partial (resp., total) modal interpretation $\Mmf = (\Fmf, \Delta, \Imc)$ that satisfies $\p$ at $w$ satisfies also $\psi$ at $w$, for every $w$ in $\Fmf$.
%Finally, we say that $\p$ is \emph{entailed under a global $\TLALCOud$ ontology $\Omc$} (with respect to partial or total traces, respectively), written $\Omc \models^{\ast} \p$, if, for every partial (resp., total) trace
%$\Mmf$ 
%and every $t$ of $\Mmf$, we have that $\p$ is satisfied at $t$ of $\Mmf$, whenever $\Omc$ is satisfied at every $t'$ of $\Mmf$.
%%Finally, a $\TLALCOud$ formula $\p$ \emph{partially} (\emph{totally}) \emph{entails} a $\TLALCOud$ formula $\psi$, written $\p \models \psi$, if every partial (total) trace that satisfies $\p$ satisfies also $\psi$.
%%\nb{M: added}
%% Finally, a KB $\Kmc$ is \emph{satisfiable on partial (total) traces} if, for each CI $C \sqsubseteq D \in \Kmc$, we have that $\Mmf, w \models C \sqsubseteq D$, for every $w \in W$. Equivalently, this holds if $\Mmf \models C \sqsubseteq^{\ast} D$, where we use the following abbreviation: $ C \sqsubseteq^{\ast} D = \Box^{+} (C \sqsubseteq D)$.
%
%
%\fi



We will consider restrictions of the base language $\TLALCOud$ along
both the DL and temporal dimensions. First, $\TLALCOd$, $\TLALCOu$ and
$\TLALCO$ stand for the fragments of $\TLALCOud$ without the universal
role, definite descriptions and both constructs, respectively.  In
addition to the basic free description logic $\ALCOud$, we define temporal extensions of the light-weight free DL $\ELOud$, which does not contain negation (and so disjunction). 
More precisely, the language $\mathcal{TL}_{\ELOud}$ is obtained from
$\TLALCOud$ by allowing only $\top$ (considered as a primitive
logical symbol), concept names, term nominals, conjunctions
%(both on concepts and formulas)
and existential restrictions in the construction of concepts.
%while negations and disjunctions can be applied to formulas only.
%
Then, by removing the universal role or/and
definite descriptions, we define $\TL_{\ELOd}$, $\TL_{\ELOu}$ and
$\TL_{\ELO}$  in the obvious way. %similarly to the fragments with $\ALCOud$.  

In the temporal dimension, given a DL $\DL$, the%
%fragments
%$\TL^{\Diamond}_{\DL}$
%and
%$\TL^{\textstyle\circ}_{\DL}$
%\nb{M: small changes}
\emph{$\Diamond\Box$-fragment},
$\TL^{\Diamond}_{\DL}$,
and
the
\emph{$\Next$-fragment},
$\TL^{\textstyle\circ}_{\DL}$,
are obtained from $\TL_{\DL}$
by disallowing the $\Next$ and the $\Diamond/\Box$ operators, respectively. Both
%the $\Diamond\Box$- and the $\Next$-
fragments
correspond to the unimodal language $\ML^1_{\DL}$, but with different accessibility relations.

In the following we will combine the syntactic restrictions
(fragments) with the semantic restrictions on interpretations and refer, for example, to
the satisfiability problem for $\mathcal{TL}^\Diamond_{\ALCOu}$
concepts in $\LTLf_{\ALCOud}$ interpretations simply as
$\LTLfdALCOu$ concept satisfiability.

%\color{blue}
As an example,
%the concept expressing that
%%KR 2025 is next year's edition of KR,
%Magdalena is a Program Chair of KR
%and either the General Chair or a PC Member of KR 2025, abbreviated as
%\[
%%\Next \{ {\sf kr } \}( {\sf kr25} )
%\exists {\sf isProgChair}.\{ {\sf kr} \} \sqcap ( \{ \defdes \exists {\sf isGenChair}. \Next \{ {\sf kr} \} \} \sqcup \exists {\sf isPCMember}. \Next \{ {\sf kr } \} (\{ {\sf magdalena} \})
%\]
%is
in $\LTLf_{\ALCOud}$, we express that whoever is a Program Chair of KR will not be Program Chair of KR again, but is always appointed as either the General Chair or a PC member of next year's KR, by means of the CI:
%we can consider
%$\LTLf_{\ALCOud}$ concept satisfiability under a global ontology stating that whoever is a Program Chair of KR will not be Program Chair of KR again, but is always appointed as either the General Chair or a PC member of next year's KR, by means of the CI:
	\begin{multline*}
\exists {\sf isProgChair}.\{ {\sf kr} \} \sqsubseteq \lnot \Diamond \exists {\sf isProgChair}.\{ {\sf kr} \} \ \sqcap \\
							 ( \{ \defdes \exists {\sf isGenChair}. \Next \{ {\sf kr} \} \} \sqcup \exists {\sf isPCMember}. \Next \{ {\sf kr } \} ).
	\end{multline*}%
%\color{black}


%On the other hand, we consider languages with restrictions on the application of modal or temporal operators.
%Given a DL $\DL$, the language $\DL$-$L$ is obtained from $L_{\DL}$ by disallowing $L$ operators over $\DL$ concepts.

%We\nb{R: cut down? } say a $\TLALCOud$ concept $C$ is \emph{satisfied at instant $t$} if
%$C^{\Imc_{t}} \neq \eset$, for some infinite model $\Mmf$; and that $C$ is \emph{satisfied at instant $t$ in finite models} if $C^{\Imc_{t}} \neq \eset$, for some finite model $\Mmf$.  Similarly to the modal case, a concept inclusion $C \sqsubseteq D$ is \emph{satisfied in~$\Mmf$}, written $\Mmf\models C\sqsubseteq D$, if 
%
%$C^{\Imc_{t}} \subseteq D^{\Imc_{t}}$, for every $t\in T$. An ontology $\mathcal{O}$ is \emph{satisfied in $\Mmf$}, written $\Mmf\models \mathcal{O}$, if every CI in $\mathcal{O}$ is satisfied in $\Mmf$.


%Given $L \in \{ \LTL, \LTLf \}$, the \emph{partial} (resp., \emph{total})  \emph{$L_{\DL}$ $P$ problem} \emph{without} (resp., \emph{with}) \emph{the RDA} is the {partial} (resp., {total}) $\TL_{\DL}$ $P$ problem without (resp., with) the RDA over the class:
%\begin{itemize}
%\item $\{ (\mathbb{N}, <) \}$, if $L = \LTL$;
%\item
%%$\mathbf{Fin}$,
%of \emph{finite strict linear orders},
%if $L = \LTLf$.
%\end{itemize}

\begin{table*}[t]%
\centering%
\newcommand{\Exp}{\textsc{Exp}}%
\newcommand{\refr}[1]{~\tiny[#1]}%
\tabcolsep=5.5pt%
\begin{tabular}{lcccc}\toprule
	       \multicolumn{1}{c}{\multirow{2}{*}{temporal logic}} & \multicolumn{2}{c}{concept satisfiability} &  \multicolumn{2}{c}{concept sat. under global ontology}\\
		 & const.\ domain & exp.\ domains & const.\ domain & exp.\ domains  \\
		\midrule
$\LTLd_{\ALCOu}$, $\LTL_{\ALCOu}$ & $\Sigma_1^1$-complete\refr{T~\ref{th:temp1:const}} & undecidable\refr{T~\ref{th:temp1:exp}.1} & $\Sigma_1^1$-complete\refr{T~\ref{th:temp1:const}}   & undecidable\refr{T~\ref{th:temp1:exp}.1}  \\
$\LTLfd_{\ALCOu}$, $\LTLf_{\ALCOu}$ & undecidable\refr{T~\ref{th:temp1:const}} & \tabcolsep=0pt\begin{tabular}{c}decidable,\\[-2pt]Ackermann-hard\end{tabular}\refr{T~\ref{th:temp1:exp}.2} & undecidable\refr{T~\ref{th:temp1:const}}  & \tabcolsep=0pt\begin{tabular}{c}decidable,\\[-2pt]Ackermann-hard\end{tabular}\refr{T~\ref{th:temp1:exp}.2} \\
$\LTLd_{\ALCO}$, $\LTL_{\ALCO}$ & ? & ? & $\Sigma_1^1$-complete\refr{T~\ref{th:temp1:const}}  & undecidable\refr{T~\ref{th:temp1:exp}.1} \\
$\LTLfd_{\ALCO}$, $\LTLf_{\ALCO}$ & ? & ? & undecidable\refr{T~\ref{th:temp1:const}}  & \tabcolsep=0pt\begin{tabular}{c}decidable,\\[-2pt]Ackermann-hard\end{tabular}\refr{T~\ref{th:temp1:exp}.2} \\
$\LTLo_{\ALCOu}$ / $\LTLo_{\ALCO}$ & \Exp-c. / in \Exp{}\refr{T~\ref{thm:temp3}} & \Exp-c. / in \Exp{}\refr{T~\ref{thm:temp3}} & undecidable\refr{T~\ref{thm:temp4}} & ? \\[2pt]
% & & Exp-c & undec. & ? \\
$\LTLfo_{\ALCOu}$ / $\LTLfo_{\ALCO}$ & \Exp-c. / in \Exp{}\refr{T~\ref{thm:temp3}} & \Exp-c. / in \Exp{}\refr{T~\ref{thm:temp3}} & undecidable\refr{T~\ref{thm:temp4}} & decidable \\\bottomrule
% & in Exp & Exp-c & undec. & decidable 
\end{tabular}
	\caption{Concept satisfiability (under global ontology) for temporal DLs}\label{table:complexity:temporal}
\end{table*}


%%%%%%%%%%%%%%%
%\subsection{Temporal Free DLs Based on \ALCO{}}

%{\color{red}{
%We make the following observations about the reductions
%\nb{M: added\\R: not sure -- too fussy, move to the appendix? \\ M: I agree, maybe I can shorten it here?}
%in Section~\ref{sec:reduction}. Lemma~\ref{lemma:ontology:normal-form} and Proposition~\ref{prop:nomnonrdatodefdes}, as well as Proposition~\ref{lemma:redpartialtototal} for the global ontology case, apply already to the $\Next$- or $\Box\Diamond$-fragments without the universal role or definite descriptions,
%%based on $\ELO$
%and
%Lemma~\ref{lemma:spy-point-reduction} holds for $\ALCO$-based $\Next$- or $\Box\Diamond$-fragments without the universal role or definite descriptions.
%Moreover, Proposition~\ref{prop:rdatononrda}, as well as Proposition~\ref{prop:redexptoconst} for the global ontology case, applies to $\Box\Diamond$-fragments
%%based on $\ELO$
%without the universal role or definite descriptions.
%}}


We
%now\nb{M: added `now'}
begin the study of the satisfiability problems for temporal DLs based on $\ALCO$ by showing that concept satisfiability in constant domains 
is undecidable or even $\Sigma_1^1$-complete (highly undecidable
%\nb{ok?}
in the analytical hierarchy) over the infinite flow of time $(\Nbl,<)$. This is very different from the classical case with RDA,  which was
  shown to be decidable in the absence of definite
  descriptions~\cite[Theorem 14.12]{GabEtAl03}. 

\begin{restatable}{theorem}{tempone}
\label{th:temp1:const}
With constant domains, concept satisfiability is  $\Sigma_1^1$-complete for $\LTLd_{\ALCOu}$   and $\LTL_{\ALCOu}$, and undecidable for
  $\LTLfd_{\ALCOu}$; also, concept satisfiability under global ontology is
  $\Sigma_1^1$-complete for $\LTLd_{\ALCO}$ and $\LTL_{\ALCO}$, and undecidable for
  $\LTLfd_{\ALCO}$.
\end{restatable}

The lower bounds follow,
%\nb{M: mention $\Sigma^{1}_{1}$-membership?}
using Theorem~\ref{th:diff}~(2), from the respective undecidability results for  the first-order one-variable temporal logic with counting~\cite{HamKur15}.
{\color{red}{
Observe that,
\nb{M: added, to check; $@$Roman: actually no need to apply Prop. 3 for the lower bound to hold, right?}
%\nb{M: add short summary of what applicable to $\ALCO$ - Lemma 6 + Proposition 3}
for $\LTLd_{\ALCO}$, we apply the spy-point universal role elimination of Lemma~\ref{lemma:spy-point-reduction}.
In addition, we note that
Propositions~\ref{prop:rdatononrda} and~\ref{prop:nomnonrdatodefdes},
Lemma~\ref{lemma:ontology:normal-form}, as well as Propositions~\ref{lemma:redpartialtototal} and~\ref{prop:redexptoconst} for the global ontology case, already hold for the $\Box\Diamond$-fragments without the universal role and definite descriptions.
%$\LTLd_{\ALCO}$.
%In addition, we note that Proposition~\ref{lemma:redpartialtototal} for the global ontology case, reducing  ...
}}

They could also be proven more directly by encoding the $\Sigma_1^1$-complete recurrence and undecidable reachability problems for the Minsky counter machines~\cite{Min61,DBLP:journals/jacm/AlurH94}.
Intuitively, the value of a
%\nb{replaced `each'}
counter of the Minsky machine can be represented as the cardinality of a certain concept. Then non-rigid nominals (or indeed the counting quantifier) can be used to ensure that the value of the counter is incremented/decremented (depending on
%\nb{inserted}
the command) by the transition: for instance, a
%\nb{inserted}
CI of the form
%
\begin{equation*}
Q_i \sqsubseteq \Next R_k \Leftrightarrow (R_k \sqcup \{ a_k \})
\end{equation*}
%
could be used to say that from state $Q_i$, the value of counter $k$ is increased by one. Note, however, that this CI uses the $\Next$ operator. Without it, the proof is considerably more elaborate and represents a
%\nb{replaced  `each'}
counter as a pair of concepts: $R_k$ is used to increment the counter, while $S_k$ to decrement it, so that the counter value is the cardinality of $R_k\sqcap \neg S_k$. Both concepts are made `monotone': $R_k \sqsubseteq \Box R_k$ and $S_k \sqsubseteq \Box S_k$, and for each transition of the Minsky machine, the non-rigid nominals pick an element that, for example, has never been in $R_k$ before but will remain in $R_k$ from the next instant on: $\neg R_k \sqcap \Box R_k$.  A sequence of these elements allows us to linearly order the domain and  construct a `diagonal' in the two-dimensional interpretation necessary for the encoding of the computation using only the $\Diamond$ operator.  

Reasoning in expanding domains turns out to be less complex, and we obtain the following:  
%  
\begin{restatable}{theorem}{temponeexp}
\label{th:temp1:exp}
\textup{(1)}  With expanding domains, concept satisfiability is
  undecidable for $\LTLd_{\ALCOu}$, and concept satisfiability under global ontology is
  undecidable for $\LTLd_{\ALCO}$.

\textup{(2)} With expanding domains, concept satisfiability  \textup{(}under global ontology\textup{)}
  is decidable  for
%  $\LTLfd_{\ALCO}$,
 % $\LTLfd_{\ALCOu}$,
 %   $\LTLfd_{\ALCOd}$
  $\LTLf_{\ALCOud}$.
However, both problems are Ackermann-hard for
  $\LTLfd_{\ALCOu}$\textup{;} 
  %and  $\LTLfd_{\ALCOd}$; 
    moreover, concept satisfiability under global ontology is Ackermann-hard for  $\LTLfd_{\ALCO}$.
%    and $\LTLfd_{\ALCOud}$.
\end{restatable}
%
Undecidability and Ackermann-hardness are proven similarly to Theorem~\ref{th:temp1:const}. In this case, however, the master problems are, respectively, the $\omega$-reachability and reachability problems for lossy Minsky machines~\cite{DBLP:conf/cade/KonevWZ05,DBLP:conf/mfcs/Schnoebelen10},
which in addition to normal transitions can also arbitrarily decrease the counter values. Such computations can be naturally encoded \emph{backwards} in interpretations with expanding domains: the arbitrary decreases of counter values correspond to the extension of the interpretation domain with fresh elements.   

The positive decidability results over the finite flows of time follows from Theorem~\ref{thm:moddickson} by Lemma~\ref{lemma:ltl-to-kfn} (together with the reduction in Proposition~\ref{lemma:redmludtomlu}).


%%%%%%%%%%%%%%%
\paragraph{Temporal Free DLs Based on \ELO{}.}

Next, we transfer the above results to the \ELO{} family. As $\TL_{\ELO}$ concepts do not contain negation and the empty concept ($\bot$), they are trivially satisfiable. Thus, our main reasoning problem is based on the notion of entailment (rather than satisfiability).
%
\begin{description}
%\item[Concept Entailment (over Finite Flows):] Given\nb{do we keep it? we do not claim any results for it - they would be about $\ELOu$ anyway and quite fiddly, as we would have to "internalise" the extra CIs} $\TL_{\DL}$-concepts $C_1$ and $C_2$, is it the case that $C_1^{\Imc(0)} \subseteq C_2^{\Imc(0)}$,  in every  interpretation $\Mmf$ based on the flow $(\mathbb{N}, <)$ (every finite flow, respectively)?
%
\item[CI Entailment  (over Finite Flows):] Given a $\TL_{\DL}$-CI $C_1\sqsubseteq C_2$ and a $\TL_{\DL}$-ontology $\Omc$, is it the case that $C_1^{\Imc_t} \subseteq C_2^{\Imc_t}$, for every $t\in T$ in  every  interpretation $\Mmf$ satisfying $\Omc$ and based  on  $(\Nbl, <)$ (every finite flow, respectively)?
\end{description}

It turns out that disjunction can be modelled in the temporal extension of $\ELO$ with the help of the $\Diamond$ modality~\cite{AKLWZ07}: intuitively, any CI of the form $\top \sqsubseteq B_1 \sqcup B_2$ is replaced with $\top \sqsubseteq\exists q.(\Diamond X_1 \sqcap \Diamond X_2)$, which says that $X_1$ and $X_2$ occur in some order in the future (possibly on another domain element). It then remains to check the order of $X_1$ and $X_2$ and, if, say, $X_1$ precedes $X_2$, then $B_1$ is chosen, otherwise $B_2$ is chosen. So, this reduction shows that the entailment problem for the fragments of $\TL^{\Diamond}_{\ELO}$ essentially has the same complexity as the complement of the satisfiability problem for the corresponding $\TL^{\Diamond}_{\ALCO}$ fragment:

\begin{restatable}{theorem}{temptwo}
\label{thm:temp2}
\textup{(1)} CI
%\nb{shortened}
entailment with constant domains  is $\Pi_1^1$-complete for $\LTLd_{\ELO}$ and 
 undecidable for $\LTLfd_{\ELO}$.
  
\textup{(2)} CI entailment with expanding domains is undecidable for $\LTLd_{\ELO}$. 

\textup{(3)}  CI entailment with expanding domains  is decidable but Ackermann-hard for $\LTLfd_{\ELO}$.
\end{restatable}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Next-Only Temporal Free DLs.}

As we have seen above, the $\Diamond$-only fragments normally exhibit the same bad computational behaviour as the full logics with both $\Diamond$ and $\Next$. We now provide some results for the fragments that contain only~$\Next$. We begin with some positive results for the satisfiability problem (without global ontology):

\begin{restatable}{theorem}{tempthree}
\label{thm:temp3}
With constant and with expanding domains,  concept satisfiability is \ExpTime-complete for $\LTLo_{\ALCOu}$ and $\LTLfo_{\ALCOu}$ and in \ExpTime{} for  $\LTLo_{\ALCO}$ and  $\LTLfo_{\ALCO}$. 
\end{restatable}
%

The  \ExpTime{} upper complexity bound can be shown by a type elimination procedure, similarly to the case of the product $\mathbf{Alt} \times \K_n$ of modal logics $\mathbf{Alt}$,  whose accessibility relation is a partial function, and multi-modal $\K_n$, which is a notational variant of $\ALC$; see~\cite[Theorem 6.6]{GabEtAl03}. One has to, in addition, take care of nominals and the universal role, but that can be done in exponential time. The matching lower bound is inherited from $\ALCOu$, but for the fragment without the universal role the exact complexity remains an open problem.

Our final result indicates that with the global ontology, the $\Next$-fragments behaves nearly as badly as the full language:

\begin{restatable}{theorem}{tempfour}
\label{thm:temp4}
With constant domains,  concept satisfiability under global ontology is undecidable for $\LTLo_{\ALCO}$ and $\LTLfo_{\ALCO}$.  
\end{restatable}
%

The proof is by a direct reduction of the reachability problem for Minsky machines, similarly to the simplified sketch for Theorem~\ref{th:temp1:const}; note the proof makes use of the spy-point universal role  elimination in Lemma~\ref{lemma:spy-point-reduction}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "rda-ale"
%%% End:


==> camera-ready/6-conclusion.tex <==
\section{Discussion and Future Work}
\label{sec:conc}

We have introduced and investigated novel fragments of first-order modal logic with non-rigid (and possibly non-referring) individual names and definite descriptions. Potential applications that remain to be explored include business process management, where formalisms for representing the dynamic behaviour of data and information are crucial~\cite{DelEtAl23,DeuEtAl18}, and context, knowledge or standpoint-dependent reasoning for which possible worlds semantics is needed~\cite{GhiSer17,AlvEtAl23}.

Besides the open decidability problems discussed above, future research directions include the extension of our results to more expressive monodic fragments~\cite{GabEtAl03,HodEtAl02},
%the study of systems based on alternative classes of frames~\cite{???},
%the introduction of hybrid~\cite{HybridIndrzejczak} or branching time logic operators~\cite{DecidableBranchingTime?},
automated support for the construction of definite descriptions and referring expressions~\cite{ArtEtAl21a,KurEtAl23}, the design of `practical' reasoning algorithms for the languages considered here, and the extension of our results to  modal DLs with hybrid~\cite{Bra14,IndZaw23}, branching-time~\cite{HodEtAl02,GutEtAl12}, dynamic~\cite{Har79}, or non-normal operators~\cite{DalEtAl23}.











%%% OLD VERSION


%We moved first steps in the study of modal free description logics, focussing in particular on the epistemic free DL $\SfiveALCOud$, and on the
%temporal free DLs $\LTLALCOud$ and $\LTLfALCOud$.
%Syntactically, these DLs extend the classical $\ALCOu$, with nominals and the universal role, by including definite descriptions and
%modal
%or temporal operators.
%Semantically, adapting ideas from the non-modal $\ALCOud$ case, we interpret these DLs over modal (epistemic or temporal) interpretations
%that allow for:
%(i) \emph{non-denoting} terms, that is, individual expressions that can be left uninterpreted at certain states, hence encoding ``error'' or ``empty'' values;
%and
%(ii) \emph{non-rigid} designators, making individual names and definite descriptions referential devices capable of picking different objects at different states, to represent ``dynamic'' or ``flexible'' values.
%The main technical results concern formula satisfiability: we show that, while this problem is $\NExpTime$-complete for $\SfiveALCOud$ on epistemic frames, it becomes undecidable 
%both for
%$\LTLALCOud$ and $\LTLfALCOud$
%on, respectively, infinite and finite temporal traces.
%%
%
%As future work, we intend to strengthen our results, as well as deepen the connections between free DLs with definite descriptions, on the one hand, and modal operators, on the other.
%On the epistemic side, we are interested in:
%(i) considering frames for the propositional modal logics $\mathbf{K4}$, $\mathbf{T}$, $\mathbf{S4}$, or $\mathbf{KD45}$,
%to model different doxastic or epistemic attitudes that might satisfy or not the so-called \emph{factivity} and \emph{introspection} principles~\cite{GabEtAl03};
%(ii) investigating of non-rigid descriptions and names
%in the context of \emph{non-normal} modal DLs, such as the ones obtained from the systems $\mathbf{E}$, $\mathbf{M}$, $\mathbf{C}$, and $\mathbf{N}$~\cite{DalEtAl19,DalEtAl22,DalEtAl23},
%to avoid the \emph{logical omniscience} problem (i.e., an agent knows all the logical truths and all the consequences of their background knowledge), which affects all the systems extending $\mathbf{K}$~\cite{Var86,Var89};
%(iii) addressing less expressive DL languages, such as $\ELOud$, in an epistemic setting, and connect them with the recently investigated \emph{standpoint DL} family~\cite{GomEtAl22,GomEtAl23}.
%
%
%On the temporal side, and in particular concerning our undecidability proofs, we observe the following.
%\citeauthor{DegEtAl02}~\cite{DegEtAl02} use equality
%%to enforce uniqueness of two objects at the subsequent instant of a trace is what
%to encode a one-unit addition or subtraction from a register's value at subsequent steps of a two-counter Minsky machine computation.
%In our case, the same effect is due to the interplay between non-rigid (and possibly non-denoting) nominals and the universal role.
%%Indeed, at subsequent time points, these non-rigid nominals allow for at most one object in their extension, and such object is implied to be different over time. It would not be possible to obtain an analogous behaviour if nominals were interpreted rigidly.
%%Moreover, the universal role plays a key role in forcing the extension of the concepts encoding the values of the counters to be suitably increased or decreased by one unit.
%%
%Related results appear also in~\citeauthor{HamKur15}~\cite{HamKur15},
%%Our findings are also in line with the results in
%%~\cite{HamKur15}, by Hampson and Kurucz,
%where the undecidability of \emph{one-variable first-order temporal logic with counting to two}, denoted by FOLTL$^{\neq}$, is proved.
%In their setting,  the \emph{difference} existential quantifier $\exists^{\neq}x$ extends the language of one-variable (monadic) first-order temporal logic: formulas like $\exists^{\neq}x \p$ enforce that $\p$ holds for some individual different from the one assigned to $x$.
%Their undecidability proof for satisfiability of FOLTL$^{\neq}$ on finite or infinite traces with constant domains is also based on an encoding of the computation of two-counter Minsky machines.
%%
%
%It seems thus that a form of interaction between the universal role and counting constructors (even simply up to one, as in $\LTLALCOu$, with non-rigid and possibly non-denoting nominals) plays a role in these kinds of undecidability proofs.
%However, it is not yet clear whether already $\LTLALCO$ or $\LTLALCOd$ satisfiability, on partial temporal interpretations and with non-rigid nominals, but \emph{without} the universal quantifier, is undecidable.
%To obtain a similar proof, one would have to suitably replace the universal role with dedicated roles for counters, while forcing them to stay ``global'' enough not to lose any information about the values of the counters at subsequent computation steps.
%We leave this open question for future work.
%%
%
%Finally, we remark that the preliminary negative results presented here for temporal free DLs might not entirely undermine the use of definite descriptions on a temporal dimension.
%For applications in temporal conceptual modelling and ontology-mediated query answering~\cite{LutEtAl08,ArtEtAl17}, it is worth exploring whether more encouraging
%%decidability and complexity
%results can be obtained in fragments restricting the use of temporal operators (limited, e.g., to the $\Box$ operator only), or constraining the DL dimension (such as the already mentioned $\LTLALCOd$, without the universal role, or lightweight members of the $\TDLite$ family~\cite{ArtEtAl14}).
%Any of these restrictions should, of course, be designed to preserve an interesting degree of interaction between the DL constructors and the non-rigidity of names and descriptions.
%
%Finally, we are interested in studying in this setting the complexities of other problems than formula satisfiability. Related to \emph{interpolant} and \emph{explicit definition existence}~\cite{ArtEtAl21,ArtEtAl23,KurEtAl23},
%the \emph{referring expression existence} problem~\cite{ArtEtAl21a},
%which asks whether there exists a description for an individual under an ontology and a given signature,
%is of particular interest to epistemic and temporal scenarios with definite descriptions.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "rda"
%%% End:


==> camera-ready/macros.tex <==
%%%
%%%
%%% SIDE COMMENTS ENVIRONMENT

% \marginparwidth=20mm
% \newcommand{\nb}[1]{\hbox to 1pt{\textcolor{red}{\bf !}}\marginpar{\raggedright\scriptsize\textcolor{red}{#1}}}
%\newcommand{\nb}[1]{}

\marginparwidth=12mm
\newcommand{\nb}[1]{\hbox to 0pt{\textcolor{red}{\bf!}}%
\marginpar[\parbox{20mm}{\scriptsize\textcolor{red}{\raggedleft #1}}]%
{\parbox{12mm}{\scriptsize\textcolor{red}{\raggedright #1}}}}
%\newcommand{\nb}[1]{}

%%%
%%%
%%% PARAGRAPH ENVIRONMENT

\newcommand{\mypar}[1]{\medskip\noindent\textbf{#1.}}


%%%
%%%
%%% USEFUL SHORTCUTS / NOTATION

\newcommand{\e}{\emph}
\newcommand{\avec}[1]{\boldsymbol{#1}}
\newcommand{\extN}{\mathbb{N}_\infty}


\newcommand{\p}{\varphi}
\newcommand{\q}{\psi}
\newcommand{\s}{\sigma}

\newcommand{\eset}{\emptyset}
\newcommand{\mdl}{\models}
\newcommand{\Int}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\I}{\ensuremath{\Imc}}

\newcommand{\sbs}{\subseteq}
\newcommand{\sqs}{\sqsubseteq}
\newcommand{\sqst}{\sqsubseteq^*}

\newcommand{\eqv}{\ensuremath{\doteq}\xspace}

\newcommand{\lp}{{\langle}}
\newcommand{\rp}{{\rangle}}

\newcommand{\tr}{^{\dagger}}
%\newcommand{\tr}{^{\ast}}
%\newcommand{\trx}{^{\dagger_{x}}}
%\newcommand{\try}{^{\dagger_{y}}}
\newcommand{\ttr}{^{\ddagger}}
\newcommand{\startr}{^{\star}}
\newcommand{\red}{^{\ast}}


\newcommand{\boldf}{\ensuremath{\boldsymbol{f}}\xspace}


%%%
%%%
%%% VARIA



%\newcommand{\st}[2]{\ensuremath{{\pi}_{#1}(#2)}\xspace}
\newcommand{\sttr}[2]{\ensuremath{{\pi}_{#1}(#2)}\xspace}


\newcommand{\md}{\ensuremath{\mathit{md}}}


\newcommand{\rpath}{\mathsf{rp}}
\newcommand{\rpathp}{\overline{\rpath}}
\newcommand{\rpathw}{\mathsf{rw}}
\newcommand{\rpathwp}{\overline{\rpathw}}


\newcommand{\concabbr}{\ensuremath{\bar{C}}\xspace}


\newcommand{\ass}[2]{\ensuremath{(#1 : #2)}\xspace}




\newcommand{\Isf}[1]{\ensuremath{\Imf^{#1}}\xspace}
%\newcommand{\Isf}[1]{\ensuremath{\Imf^{\mid^{#1}}}\xspace}

\newcommand{\Fsuf}[1]{\ensuremath{\Fmf^{#1}}\xspace}


%%%
%%%
%%% LOGIC


%%%
%%% SIGNATURE & SYNTACTIC NOTIONS

\newcommand{\sig}[1]{\ensuremath{\Sigma_{#1}}\xspace}

\newcommand{\size}[1]{\ensuremath{|#1|}\xspace}
\newcommand{\len}[1]{\ensuremath{{\sf len}(#1)}\xspace}

\newcommand{\sub}[1]{\ensuremath{\mathsf{sub}(#1)}\xspace}
\newcommand{\subneg}[1]{\ensuremath{\mathsf{sub}_{\lnot}(#1)}\xspace}

\newcommand{\Var}{\ensuremath{\mathsf{Var}}\xspace}

\newcommand{\ind}[1]{\ensuremath{\mathsf{ind}(#1)}\xspace}

\newcommand{\con}[1]{\ensuremath{\mathsf{con}(#1)}\xspace}
\newcommand{\conneg}[1]{\ensuremath{\mathsf{con}_{\lnot}(#1)}\xspace}
%\newcommand{\subc}[1]{\ensuremath{\mathsf{subc}(#1)}\xspace}

\newcommand{\ordcon}[1]{\ensuremath{\Cmf(#1)}\xspace}

\newcommand{\rol}[1]{\ensuremath{\mathsf{rol}(#1)}\xspace}

\newcommand{\atcon}[1]{\ensuremath{\mathsf{atcon}(#1)}\xspace}

\newcommand{\cons}[1]{\ensuremath{\mathsf{cons}(#1)}\xspace}


%%% SEMANTIC NOTIONS

\newcommand{\conseq}[1]{\ensuremath{\mathit{Cons}(#1)}\xspace}

\newcommand{\reduct}{\ensuremath{\Imf_{\mid_{\Sigma}}}\xspace}

\newcommand{\assign}{\ensuremath{\sigma}\xspace}
%\newcommand{\assign}{\ensuremath{\mathfrak{a}}\xspace}

\newcommand{\tvalue}[3]{\ensuremath{{#1}^{\Mmf, {#2}}_{#3}}\xspace}
%\newcommand{\tvalue}{\ensuremath{\bar{\assign}}\xspace}

\newcommand{\dom}{\ensuremath{{\sf dom}}\xspace}



%%% TREES

\newcommand{\tree}[1]{\ensuremath{T_{#1}}\xspace}
\newcommand{\tvertex}{\ensuremath{V}\xspace}
\newcommand{\tedge}{\ensuremath{E}\xspace}
\newcommand{\tlabel}{\ensuremath{l}\xspace}
\newcommand{\leaf}[1]{\ensuremath{L(#1)}\xspace}
\newcommand{\fleaf}[1]{\ensuremath{f(#1)}\xspace}
\newcommand{\nleaf}[1]{\ensuremath{{\sf nl}(#1)}\xspace}
\newcommand{\vleaf}{\ensuremath{V}\xspace}


%%%
%%% LOGICAL OPERATORS


%\renewcommand{\U}{\ensuremath{\mathbin{\mathcal{U}}}\xspace}
\newcommand{\U}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\Until}{\ensuremath{\mathbin{\mathcal{U}}}\xspace}
\newcommand{\Since}{\ensuremath{\mathbin{\mathcal{S}}}\xspace}
\newcommand{\Wuntil}{\ensuremath{\mathbin{\mathcal{W}}}\xspace}

%\newcommand{\Next}{\ensuremath{\ocircle}}
\newcommand{\Next}{{\ensuremath{\raisebox{0.25ex}{\text{\scriptsize{$\bigcirc$}}}}}}
\newcommand{\nxt}{{\ensuremath{\raisebox{0.2ex}{\text{\tiny{$\scriptscriptstyle{\bigcirc}$}}}}}}
\newcommand{\Of}{\ocircle_{F}}
\newcommand{\Op}{\ocircle_{P}}
\newcommand{\Wnext}{\CIRCLE}

\newcommand{\D}{\Diamond}
\newcommand{\Df}{\D_{F}}
\newcommand{\Dp}{\Diamond_{P}}
\newcommand{\Dplus}{\ensuremath{\Diamond^{+}}\xspace}
\newcommand{\Uplus}{\ensuremath{\U^{+}}\xspace}
\newcommand{\B}{\Box}
\newcommand{\Bf}{\B_{F}}
\newcommand{\Bp}{\Box_{P}}

\newcommand{\Bast}{\boxast}

\newcommand{\monodic}{\ensuremath{\mathop{\ooalign{$\Box$ \cr \kern0.57ex \raisebox{0.2ex}{\scalebox{0.55}{$1$}}}\rule{0pt}{1.5ex} \kern-0.7ex}}\xspace}
%\newcommand{\monodic}{\ensuremath{(\textsf{m})}\xspace}

\newcommand{\Boxuni}{\ensuremath{\mathop{\ooalign{$\Box$ \cr \kern0.57ex \raisebox{0.2ex}{\scalebox{0.55}{$u$}}}\rule{0pt}{1.5ex} \kern-0.7ex}}\xspace}
%\newcommand{\monodic}{\ensuremath{(\textsf{m})}\xspace}


\newcommand{\CK}{\mathsf{C}}


\DeclareRobustCommand{\zerodic}{\ensuremath{\mathop{\ooalign{$\Box$ \cr \kern0.57ex \raisebox{0.2ex}{\scalebox{0.55}{$0$}}}\rule{0pt}{1.5ex} \kern-0.7ex}}\xspace}

%%%
%%% LOGIC SYSTEMS AND LANGUAGES

\newcommand{\Lang}{\ensuremath{\mathcal{L}}}

%%% FIRST-ORDER LOGIC

\newcommand{\QL}{\ensuremath{\smash{\mathcal{QL}}}\xspace}
\newcommand{\QLd}{\ensuremath{\smash{\mathcal{QL}^{\defdes}_{\lambda}}}\xspace}

\newcommand{\fv}{\ensuremath{{\sf fv}}\xspace}


%%%
%%% DESCRIPTION LOGICS


%%%
%%% SIGNATURE & SYNTACTIC NOTIONS

\newcommand{\NC}{\ensuremath{{\sf N_C}}\xspace}
\newcommand{\NI}{\ensuremath{{\sf N_I}}\xspace}
\newcommand{\NID}{\ensuremath{{\sf N_{I_{d}}}(\I)}\xspace}
\newcommand{\NR}{\ensuremath{{\sf N_R}}\xspace}
\newcommand{\NPr}{\ensuremath{\sf{N}_{\sf{P}}\xspace}}

\newcommand{\Roles}{\ensuremath{{\sf R}}\xspace}

\newcommand{\NIr}{\ensuremath{\textsf{N}_{\textsf{IR}}\xspace}}
\newcommand{\NIf}{\ensuremath{\textsf{N}_{\textsf{IF}}\xspace}}

\newcommand{\funct}[1]{\ensuremath{(\mathsf{funct} \ #1)}\xspace}





%%% DESCRIPTION LOGICS LANGUAGES

\newcommand{\DL}{\ensuremath{\mathcal{DL}}\xspace}
%\newcommand{\DL}{\ensuremath{\text{DL}}\xspace}
\newcommand{\DLs}{\ensuremath{\text{DLs}}\xspace}
\newcommand{\DLite}{\textsl{DL-Lite}\xspace}


\newcommand{\ExprDL}{\ensuremath{\textsf{ExprDL}}\xspace}
\newcommand{\LightDL}{\ensuremath{\textsf{LightDL}}\xspace}



\newcommand{\DLitea}{\ensuremath{\DLite_{\alpha}}}
\newcommand{\DLiteb}{\ensuremath{\DLite_\textit{bool}}}
\newcommand{\DLitek}{\ensuremath{\DLite_\textit{krom}}}
\newcommand{\DLitec}{\ensuremath{\DLite_\textit{core}}}


\newcommand{\ALC}{\ensuremath{\smash{\mathcal{ALC}}}\xspace}
\newcommand{\ALCO}{\ensuremath{\smash{\mathcal{ALCO}}}\xspace}
\newcommand{\ALCQI}{\ensuremath{\mathcal{ALCQI}}}
\newcommand{\DLR}{\ensuremath{\mathcal{DLR}}}
\newcommand{\ALCIO}{\ensuremath{\mathcal{ALCIO}}}
\newcommand{\ALCQO}{\ensuremath{\mathcal{ALCQO}}}
\newcommand{\ALCIQO}{\ensuremath{\mathcal{ALCIQO}}}

\newcommand{\ALCu}{\ensuremath{\smash{\mathcal{ALC}_{\!u}}}\xspace}
\newcommand{\ALCOu}{\ensuremath{\smash{\mathcal{ALCO}_{\!u}}}\xspace}
\newcommand{\ALCIOu}{\ensuremath{\mathcal{ALCIO}_{\!u}}}
\newcommand{\ALCQOu}{\ensuremath{\mathcal{ALCQO}_{\!u}}}

\newcommand{\ALCOud}{\ensuremath{\smash{\mathcal{ALCO}_{\!u}^{\defdes}}}\xspace}
\newcommand{\ALCIOud}{\ensuremath{\smash{\mathcal{ALCIO}_{\!u}^{\defdes}}}\xspace}


\newcommand{\ALCd}{\ensuremath{\smash{\mathcal{ALC}^{\defdes}}}\xspace}
\newcommand{\ALCOd}{\ensuremath{\smash{\mathcal{ALCO}^{\defdes}}}\xspace}
\newcommand{\ALCOdF}{\ensuremath{\smash{\mathcal{ALCO}^{\defdes}_{\Fmc}}}\xspace}
\newcommand{\ALCIOd}{\ensuremath{\smash{\mathcal{ALCIO}^{\defdes}}}\xspace}
\newcommand{\ALCQOd}{\ensuremath{\smash{\mathcal{ALCQO}^{\defdes}}}\xspace}
\newcommand{\ALCFOd}{\ensuremath{\smash{\mathcal{ALCFO}^{\defdes}_{\Fmc}}}\xspace}
\newcommand{\ALCIFOd}{\ensuremath{\smash{\mathcal{ALCIFO}^{\defdes}}}\xspace}


\newcommand{\ALCOat}{\ensuremath{\smash{\mathcal{ALCO}@}}\xspace}


\newcommand{\EL}{\ensuremath{\smash{\mathcal{EL}}}\xspace}
\newcommand{\ELO}{\ensuremath{\smash{\mathcal{ELO}}}\xspace}
\newcommand{\ELOB}{\ensuremath{\smash{\mathcal{ELO}_\bot}}\xspace}
\newcommand{\ELOu}{\ensuremath{\smash{\mathcal{ELO}_{\!u}}}\xspace}
\newcommand{\ELOd}{\ensuremath{\smash{\mathcal{ELO}^{\defdes}}}\xspace}
\newcommand{\ELOud}{\ensuremath{\smash{\mathcal{ELO}_{\!u}^{\defdes}}}\xspace}
\newcommand{\ELOF}{\ensuremath{\smash{\mathcal{ELO}_{\Fmc}}}\xspace}
\newcommand{\ELOFd}{\ensuremath{\smash{\mathcal{ELOF}^{\defdes}}}\xspace}

\newcommand{\ELext}[3]{\ensuremath{\smash{\mathcal{EL{#1}}^{#2}_{\!#3}}}\xspace}



\newcommand{\NKR}{\ensuremath{\smash{\mathcal{ALCO}^{\ast}}}\xspace}
\newcommand{\NKRu}{\ensuremath{\smash{\mathcal{ALCO}_{\!u}^{\ast}}}\xspace}
\newcommand{\NKRd}{\ensuremath{\smash{\mathcal{ALCO}^{\defdes \ast}}}\xspace}
\newcommand{\NKRud}{\ensuremath{\smash{\mathcal{ALCO}_{\!u}^{\defdes \ast}}}\xspace}






%%% QUASI-MODELS & REDUCTS

\newcommand{\nnf}{\ensuremath{\mathsf{nnf}}\xspace}
\newcommand{\cl}{\ensuremath{\mathsf{cl}}\xspace}

\newcommand{\clu}{\ensuremath{\cl^{\mathsf{u}}}\xspace}
\newcommand{\clc}{\ensuremath{\cl^{\mathsf{c}}}\xspace}
\newcommand{\clf}{\ensuremath{\cl^{\mathsf{f}}}\xspace}
\newcommand{\cls}{\ensuremath{\cl^\ast}\xspace}
\newcommand{\csub}{\ensuremath{\mathsf{csub}}\xspace}
\newcommand{\fsub}{\ensuremath{\mathsf{fsub}}\xspace}
\newcommand{\const}{\ensuremath{\ell_{\varphi}}\xspace}
\newcommand{\runSegments}[1]{\ensuremath{\mathsf{rs}(#1)}\xspace}
\newcommand{\roleConstraints}[1]{\ensuremath{\mathsf{rc}(#1)}\xspace}
\newcommand{\individuals}[1]{\NI(#1)}
\newcommand{\types}[1]{\mathsf{tp}(#1)}
\newcommand{\typesc}[1]{\mathsf{tp^{c}}(#1)}
\newcommand{\typesf}[1]{\mathsf{tp^{f}}(#1)}
\newcommand{\typescF}[1]{\mathsf{tp^{c}_{\Fmf}}(#1)}
\newcommand{\typesfF}[1]{\mathsf{tp^{f}_{\Fmf}}(#1)}
\newcommand{\quasistates}[1]{\mathsf{qs}(#1)}
\newcommand{\roles}[1]{\mathsf{rol}(#1)}
\newcommand{\rs}[1]{\ensuremath{\Rmc_{#1}}\xspace}


\newcommand{\real}{\ensuremath{{\sf real}}\xspace}



\newcommand{\quasimod}{\ensuremath{\Qmf}\xspace}
\newcommand{\setqm}[1]{\ensuremath{\Qmf(#1)}\xspace}
\newcommand{\setintqm}[1]{\ensuremath{\Imf(#1)}\xspace}

\newcommand{\runs}{\ensuremath{\Rmf}\xspace}
\newcommand{\gruns}{\ensuremath{\Gmf}\xspace}

\newcommand{\stcand}{\ensuremath{\Cmf}\xspace}
%\newcommand{\seqcand}{\ensuremath{\mathbf{q}}\xspace}
\newcommand{\funcand}{\ensuremath{\boldsymbol{q}}\xspace}

\newcommand{\ptcand}{\ensuremath{\Pmf}\xspace}

\newcommand{\modcand}{\ensuremath{S}\xspace}

%\newcommand{\type}{\ensuremath{{\boldsymbol{t}}}\xspace}
\newcommand{\tp}{\ensuremath{\boldsymbol{t}}\xspace}
%\newcommand{\setcontp}{\ensuremath{\boldsymbol{T}}\xspace}
\newcommand{\settp}{\ensuremath{\boldsymbol{T}}\xspace}
\newcommand{\setindtp}{\ensuremath{T^{con}}\xspace}

\newcommand{\contp}{\ensuremath{{\boldsymbol{t}}}\xspace}
\newcommand{\fortp}{\ensuremath{{\boldsymbol{f}}}\xspace}

\newcommand{\basesetcontp}{\ensuremath{T}\xspace}
\newcommand{\copysetcontp}{\ensuremath{\tilde{T}}\xspace}
%\newcommand{\undersetcontp}{\ensuremath{T}\xspace}
\newcommand{\mult}{\ensuremath{m}\xspace}






%%%
%%% MODAL LOGICS


%%% FRAMES AND MODELS

\newcommand{\FrL}{\ensuremath{\smash{\mathsf{Fr}\mathbf{L}}}\xspace}

\newcommand{\Fr}{\ensuremath{\smash{\mathcal{F}}}\xspace}


%%% MODAL LANGUAGES

\newcommand{\ML}{\ensuremath{\smash{\mathcal{ML}}}\xspace}
\newcommand{\QML}{\ensuremath{\smash{\mathcal{QML}}}\xspace}

\newcommand{\QMLl}{\ensuremath{\smash{\mathcal{QML}_{\lambda}}}\xspace}

\newcommand{\QMLd}{\ensuremath{\smash{\mathcal{QML}^{\defdes}}}\xspace}

\newcommand{\QMLdl}{\ensuremath{\smash{\mathcal{QML}^{\defdes}_{\lambda}}}\xspace}

\newcommand{\MLALC}{\ensuremath{\smash{\ML_{\mathcal{ALC}}}}\xspace}

\newcommand{\MLnALC}[1]{\ensuremath{\smash{\ML^{#1}_{\mathcal{ALC}}}}\xspace}



%\newcommand{\MLALCd}{\ensuremath{\smash{\mathcal{M}_{n}\mathcal{L}_{\mathcal{ALC}^{\defdes}}}}\xspace}
%\newcommand{\MLALCOd}{\ensuremath{\smash{\mathcal{M}_{n}\mathcal{L}_{\mathcal{ALCO}^{\defdes}}}}\xspace}
%\newcommand{\MLALCOu}{\ensuremath{\smash{\mathcal{M}_{n}\mathcal{L}_{\ALCOu}}}\xspace}
%\newcommand{\MLALCOud}{\ensuremath{\smash{\mathcal{M}_{n}\mathcal{L}_{\ALCOud}}}\xspace}

\newcommand{\MLALCO}{\ensuremath{\smash{\ML^{n}_{\mathcal{ALCO}}}}\xspace}
\newcommand{\MLALCd}{\ensuremath{\smash{\ML^{n}_{\mathcal{ALC}^{\defdes}}}}\xspace}
\newcommand{\MLALCud}{\ensuremath{\smash{\ML^{n}_{\mathcal{ALC}_{\!u}^{\defdes}}}}\xspace}
\newcommand{\MLALCOd}{\ensuremath{\smash{\ML^{n}_{\mathcal{ALCO}^{\defdes}}}}\xspace}
\newcommand{\MLALCOu}{\ensuremath{\smash{\ML^{n}_{\ALCOu}}}\xspace}
\newcommand{\MLALCOud}{\ensuremath{\smash{\ML^{n}_{\ALCOud}}}\xspace}

%\newcommand{\MLALCd}{\ensuremath{\smash{\ML_{\mathcal{ALC}^{\defdes}}}}\xspace}
%\newcommand{\MLALCOd}{\ensuremath{\smash{\ML_{\mathcal{ALCO}^{\defdes}}}}\xspace}
%\newcommand{\MLALCOu}{\ensuremath{\smash{\ML_{\ALCOu}}}\xspace}
%\newcommand{\MLALCOud}{\ensuremath{\smash{\ML_{\ALCOud}}}\xspace}

\newcommand{\LALCOud}{\ensuremath{\smash{{L}_{\ALCOud}}}\xspace}


%%% MODAL SYSTEMS

\newcommand{\K}{\ensuremath{\mathbf{K}}}
\newcommand{\Kfour}{\ensuremath{\mathbf{K4}}}
\newcommand{\GL}{\ensuremath{\mathbf{GL}}}
\newcommand{\Grz}{\ensuremath{\mathbf{Grz}}}

\newcommand{\Kfn}{\ensuremath{\K\!\boldsymbol{f}^{\ast n}}}

\newcommand{\EALC}{\ensuremath{\smash{\mathbf{E}_{\mathcal{ALC}}}}\xspace}
\newcommand{\MALC}{\ensuremath{\smash{\mathbf{M}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KALC}{\ensuremath{\smash{\mathbf{K}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KtwoALC}{\ensuremath{\smash{\mathbf{K}^{2}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KthreeALC}{\ensuremath{\smash{\mathbf{K}^{3}_{\mathcal{ALC}}}}\xspace}

\newcommand{\KnALC}[1]{\ensuremath{\smash{\mathbf{K}^{#1}_{\mathcal{ALC}}}}\xspace}


\newcommand{\KDfourfive}{\ensuremath{\mathbf{KD45}}}

\newcommand{\Sfive}{\ensuremath{\mathbf{S5}}}
\newcommand{\Sfivee}{\ensuremath{\mathbf{S5}\times\mathbf{S5}}}

\newcommand{\SfiveALC}{\ensuremath{\mathbf{S5}_{\mathcal{ALC}}}}
\newcommand{\SfiveALCu}{\ensuremath{\mathbf{S5}_{\ALCu}}}
\newcommand{\SfiveALCQI}{\ensuremath{\mathbf{S5}_{\mathcal{ALCQI}}}}
\newcommand{\SfiveALCOu}{\ensuremath{\mathbf{S5}_{\ALCOu}}}
\newcommand{\SfiveALCOud}{\ensuremath{\mathbf{S5}_{\ALCOud}}}

\newcommand{\SfiveELOud}{\ensuremath{\mathbf{S5}_{\ELOud}}}


\newcommand{\Sfiven}{\ensuremath{\mathbf{S5}^{n}}}

\newcommand{\SfivenALC}{\ensuremath{\Sfiven_{\mathcal{ALC}}}}
\newcommand{\SfivenALCu}{\ensuremath{\Sfiven_{\ALCu}}}
\newcommand{\SfivenALCQI}{\ensuremath{\Sfiven_{\mathcal{ALCQI}}}}
\newcommand{\SfivenALCOu}{\ensuremath{\Sfiven_{\ALCOu}}}
\newcommand{\SfivenALCOud}{\ensuremath{\Sfiven_{\ALCOud}}}

\newcommand{\SfivebELOud}{\ensuremath{\Sfiven_{\ELOud}}}



%%%
%%% TEMPORAL LOGICS


%%% TEMPORAL LANGUAGES (WITH NON RIGID-DESIGNATORS)

\newcommand{\TL}{\ensuremath{\smash{\mathcal{TL}}}\xspace}
%\newcommand{\TL}{\ensuremath{\smash{\mathcal{LTL}}}\xspace}
%\newcommand{\TL}{\ensuremath{\smash{\textnormal{LTL}}}\xspace}
%\newcommand{\TL}{\ensuremath{\smash{\mathcal{LT}_{\Until}\mathcal{L}}}\xspace}
%\newcommand{\QML}{\ensuremath{\smash{\mathcal{QML}}}\xspace}
\newcommand{\BTL}{\ensuremath{\smash{\mathcal{BT}_{\Until}\mathcal{L}}}\xspace}


\newcommand{\TLALC}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALC}}}}\xspace}
\newcommand{\TLALCO}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALCO}}}}\xspace}
\newcommand{\TLnALCO}{\ensuremath{\smash{\mathcal{TL}^{\textstyle\circ}_{\mathcal{ALCO}}}}\xspace}

\newcommand{\TLALCd}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALC}^{\defdes}}}}\xspace}

\newcommand{\TLALCOd}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALCO}^{\defdes}}}}\xspace}
\newcommand{\TLALCOud}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALCO}_{\!u}^{\defdes}}}}\xspace}
\newcommand{\TLALCOu}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALCO}_{\!u}}}}\xspace}
\newcommand{\TLnALCOu}{\ensuremath{\smash{\mathcal{TL}^{\textstyle\circ}_{\mathcal{ALCO}_{\!u}}}}\xspace}

\newcommand{\TLALCIQOd}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALCIQO}^{\defdes}}}}\xspace}
\newcommand{\TLALCIQOu}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALCIQO}_{\!u}}}}\xspace}
\newcommand{\TLALCIQOud}{\ensuremath{\smash{\mathcal{TL}_{\mathcal{ALCIQO}_{\!u}^{\defdes}}}}\xspace}

%\newcommand{\TLALC}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALC}}}}\xspace}
%\newcommand{\TLALCO}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALCO}}}}\xspace}
%
%\newcommand{\TLALCOd}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALCO}^{\defdes}}}}\xspace}
%\newcommand{\TLALCOud}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALCO}_{\!u}^{\defdes}}}}\xspace}
%\newcommand{\TLALCOu}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALCO}_{\!u}}}}\xspace}
%
%\newcommand{\TLALCIQOd}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALCIQO}^{\defdes}}}}\xspace}
%\newcommand{\TLALCIQOu}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALCIQO}_{\!u}}}}\xspace}
%\newcommand{\TLALCIQOud}{\ensuremath{\smash{\mathcal{T}\mathcal{L}^{\Until}_{\mathcal{ALCIQO}_{\!u}^{\defdes}}}}\xspace}


%\newcommand{\TLALC}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALC}}}}\xspace}
%\newcommand{\TLALCO}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALCO}}}}\xspace}
%
%\newcommand{\TLALCOd}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALCO}^{\defdes}}}}\xspace}
%\newcommand{\TLALCOud}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALCO}_{\!u}^{\defdes}}}}\xspace}
%\newcommand{\TLALCOu}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALCO}_{\!u}}}}\xspace}
%
%\newcommand{\TLALCIQOd}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALCIQO}^{\defdes}}}}\xspace}
%\newcommand{\TLALCIQOu}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALCIQO}_{\!u}}}}\xspace}
%\newcommand{\TLALCIQOud}{\ensuremath{\smash{\mathcal{T}_{\Until}\mathcal{L}_{\mathcal{ALCIQO}_{\!u}^{\defdes}}}}\xspace}

%\newcommand{\TLALC}{\ensuremath{\smash{\TL_{\mathcal{ALC}}}}\xspace}
%\newcommand{\TLALCO}{\ensuremath{\smash{\TL_{\mathcal{ALCO}}}}\xspace}
%
%\newcommand{\TLALCOd}{\ensuremath{\smash{\TL_{\mathcal{ALCO}^{\defdes}}}}\xspace}
%\newcommand{\TLALCOud}{\ensuremath{\smash{\TL_{\mathcal{ALCO}_{\!u}^{\defdes}}}}\xspace}
%\newcommand{\TLALCOu}{\ensuremath{\smash{\TL_{\mathcal{ALCO}_{\!u}}}}\xspace}
%
%\newcommand{\TLALCIQOd}{\ensuremath{\smash{\TL_{\mathcal{ALCIQO}^{\defdes}}}}\xspace}
%\newcommand{\TLALCIQOu}{\ensuremath{\smash{\TL_{\mathcal{ALCIQO}_{\!u}}}}\xspace}
%\newcommand{\TLALCIQOud}{\ensuremath{\smash{\TL_{\mathcal{ALCIQO}_{\!u}^{\defdes}}}}\xspace}



\newcommand{\LTL}{\ensuremath{\mathbf{LTL}}}
\newcommand{\LTLfo}{\ensuremath{\LTLf^{\textstyle\circ}}}
\newcommand{\LTLo}{\ensuremath{\LTL^{\textstyle\circ}}}
\newcommand{\LTLd}{\ensuremath{\LTL^\Diamond}}
%\newcommand{\LTL}{\ensuremath{\textsl{LTL}}\xspace}
\newcommand{\LTLf}{\ensuremath{\LTL\!{\text{\ensuremath{\boldsymbol{f}}}}}}
\newcommand{\LTLfd}{\ensuremath{\LTLf^\Diamond}}
%\newcommand{\LTLf}{\ensuremath{\LTL_{\boldsymbol{f}}}\xspace}
%\newcommand{\LTLf}{\ensuremath{\LTL\boldsymbol{f}}\xspace}




\newcommand{\LTLALC}{\ensuremath{\smash{\LTL_{\mathcal{ALC}}}}\xspace}
\newcommand{\LTLALCO}{\ensuremath{\smash{\LTL_{\mathcal{ALCO}}}}\xspace}

\newcommand{\LTLALCOd}{\ensuremath{\smash{\LTL_{\mathcal{ALCO}^{\defdes}}}}\xspace}
\newcommand{\LTLALCOud}{\ensuremath{\smash{\LTL_{\mathcal{ALCO}_{\!u}^{\defdes}}}}\xspace}
\newcommand{\LTLALCOu}{\ensuremath{\smash{\LTL_{\mathcal{ALCO}_{\!u}}}}\xspace}

\newcommand{\LTLALCIQOd}{\ensuremath{\smash{\LTL_{\mathcal{ALCIQO}^{\defdes}}}}\xspace}
\newcommand{\LTLALCIQOu}{\ensuremath{\smash{\LTL_{\mathcal{ALCIQO}_{\!u}}}}\xspace}
\newcommand{\LTLALCIQOud}{\ensuremath{\smash{\LTL_{\mathcal{ALCIQO}_{\!u}^{\defdes}}}}\xspace}

\newcommand{\LTLBALCO}{\ensuremath{\smash{\LTL^{\Box}_{\mathcal{ALCO}}}}\xspace}
\newcommand{\LTLBNALCO}{\ensuremath{\smash{\LTL^{\Box\nxt}_{\mathcal{ALCO}}}}\xspace}
\newcommand{\LTLELO}{\ensuremath{\smash{\LTL_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLBELO}{\ensuremath{\smash{\LTL^{\Box}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLBNELO}{\ensuremath{\smash{\LTL^{\Box\nxt}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLDELO}{\ensuremath{\smash{\LTL^{\Diamond}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLDNELO}{\ensuremath{\smash{\LTL^{\Diamond\nxt}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLBDNELO}{\ensuremath{\smash{\LTL^{\Box\Diamond\nxt}_{\mathcal{ELO}_\bot}}}\xspace}

\newcommand{\LTLfELO}{\ensuremath{\smash{\LTLf_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLfBELO}{\ensuremath{\smash{\LTLf^{\Box}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLfBNELO}{\ensuremath{\smash{\LTLf^{\Box\nxt}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLfDELO}{\ensuremath{\smash{\LTLf^{\Diamond}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLfDNELO}{\ensuremath{\smash{\LTLf^{\Diamond\nxt}_{\mathcal{ELO}_\bot}}}\xspace}
\newcommand{\LTLfBDNELO}{\ensuremath{\smash{\LTLf^{\Box\Diamond\nxt}_{\mathcal{ELO}_\bot}}}\xspace}


\newcommand{\LTLfELOnb}{\ensuremath{\smash{\LTLf_{\mathcal{ELO}}}}\xspace}
\newcommand{\LTLELOnb}{\ensuremath{\smash{\LTL_{\mathcal{ELO}}}}\xspace}


\newcommand{\LTLfALC}{\ensuremath{\smash{\LTLf_{\!\mathcal{ALC}}}}\xspace}
\newcommand{\LTLfALCO}{\ensuremath{\smash{\LTLf_{\!\mathcal{ALCO}}}}\xspace}

\newcommand{\LTLfALCOd}{\ensuremath{\smash{\LTLf_{\!\mathcal{ALCO}^{\defdes}}}}\xspace}
\newcommand{\LTLfALCOu}{\ensuremath{\smash{\LTLf_{\!\mathcal{ALCO}_{\!u}}}}\xspace}
\newcommand{\LTLfALCOud}{\ensuremath{\smash{\LTLf_{\!\mathcal{ALCO}_{\!u}^{\defdes}}}}\xspace}

\newcommand{\LTLfALCIQOd}{\ensuremath{\smash{\LTLf_{\mathcal{ALCIQO}^{\defdes}}}}\xspace}
\newcommand{\LTLfALCIQOu}{\ensuremath{\smash{\LTLf_{\mathcal{ALCIQO}_{\!u}}}}\xspace}
\newcommand{\LTLfALCIQOud}{\ensuremath{\smash{\LTLf_{\mathcal{ALCIQO}_{\!u}^{\defdes}}}}\xspace}



%%% LTLf_DL with DIAMOND ONLY

\newcommand{\LTLfdALCO}{\ensuremath{\smash{\LTLf^{\Diamond}_{\!\ALCO}}}\xspace}
\newcommand{\LTLfdALCOu}{\ensuremath{\smash{\LTLf^{\Diamond}_{\!\ALCOu}}}\xspace}
\newcommand{\LTLfdALCOud}{\ensuremath{\smash{\LTLf^{\Diamond}_{\!\ALCOud}}}\xspace}

\newcommand{\LTLfdELO}{\ensuremath{\smash{\LTLf^{\Diamond}_{\!\ELO}}}\xspace}
\newcommand{\LTLfdELOu}{\ensuremath{\smash{\LTLf^{\Diamond}_{\!\ELOu}}}\xspace}
\newcommand{\LTLfdELOud}{\ensuremath{\smash{\LTLf^{\Diamond}_{\!\ELOud}}}\xspace}



\newcommand{\BTLALC}{\ensuremath{\smash{\BTL_{\mathcal{ALC}}}}\xspace}
\newcommand{\BTLALCOd}{\ensuremath{\smash{\BTL_{\mathcal{ALCO}^{\defdes}}}}\xspace}



\newcommand{\TLNKR}{\ensuremath{\smash{\TL_{\mathcal{ALCO}^{\ast}}}}\xspace}
\newcommand{\TLNKRd}{\ensuremath{\smash{\TL_{\mathcal{ALCO}^{\defdes \ast}}}}\xspace}

\newcommand{\TLNKRIQ}{\ensuremath{\smash{\TL_{\mathcal{ALCIQO}^{\ast}}}}\xspace}
\newcommand{\TLNKRIQd}{\ensuremath{\smash{\TL_{\mathcal{ALCIQO}^{\defdes \ast}}}}\xspace}




%\newcommand{\QLog}[1]{\ensuremath{\textnormal{\textsf{QLog}}_{\Until}(#1)}\xspace}
\newcommand{\QLog}{\ensuremath{\textnormal{\textsf{QLog}}^{f}_{\Until}}\xspace}

%\newcommand{\QMLd}{\ensuremath{\smash{\mathcal{QML}^{\defdes}_{\lambda}}}\xspace}

\newcommand{\RVLTL}{\ensuremath{\textsl{RV-LTL}}\xspace}

%\newcommand{\QTL}{\ensuremath{\mathcal{QT\!L}}\xspace}
\newcommand{\QTL}{\ensuremath{{\textsl{T}_{\Until}\mathcal{QL}}}\xspace}

\newcommand{\QTLfr}[3]{\ensuremath{{\mathcal{T}_{\Until}\mathcal{QL}^{#2}_{#3}}}\xspace}
%\newcommand{\QTLfr}[3]{\ensuremath{{\textsl{T}_{\Until}\mathcal{QL}^{#2}_{#3}}}\xspace}
%%\newcommand{\QTLfr}[3]{\ensuremath{{\textsl{T}_{\Until}^{\ #1}\mathcal{QL}^{#2}_{#3}}}\xspace}
%%\newcommand{\QTLfr}[3]{\ensuremath{\mathcal{\QTL}^{#1}_{#2}{#3}}\xspace}

\newcommand{\QTLn}[1]{\ensuremath{\smash{\QTL_{#1}}}\xspace}
%\newcommand{\QTLi}{{\ensuremath{\QTL^{1}}}}
%\newcommand{\QTLii}{{\ensuremath{\QTL^{2}}}}
%\newcommand{\QTLn}{{\ensuremath{\QTL^{n}}}}

\newcommand{\QTLm}{{\ensuremath{\QTL(\textsf{m})}}}
%\newcommand{\QTLiim}{{\ensuremath{\QTL^{2}(\textsf{m})}}}

\newcommand{\QTLf}{{\ensuremath{\QTL}}}
\newcommand{\QTLfn}[1]{\ensuremath{\smash{\QTL_{#1}}}\xspace}
%\newcommand{\QTLf}{{\ensuremath{\QTL^{f}}}}
%\newcommand{\QTLfn}[1]{\ensuremath{\smash{\QTL^{f}_{#1}}}\xspace}
%\newcommand{\QTLfi}{{\ensuremath{\QTL_{f}^{1}}}}
%\newcommand{\QTLfii}{{\ensuremath{\QTL_{f}^{2}}}}
%\newcommand{\QTLfn}{{\ensuremath{\QTL_{f}^{n}}}}

\newcommand{\QTLfm}{{\ensuremath{\QTLf(\textsf{m})}}}
\newcommand{\QTLfnm}{{\ensuremath{\QTLfn(\textsf{m})}}}
%\newcommand{\QTLfiim}{{\ensuremath{\QTL_{f}^{2}(\textsf{m})}}}

\newcommand{\QTLk}{{\ensuremath{\QTL^{k}}}}
\newcommand{\QTLkn}[1]{\ensuremath{\smash{\QTL^{k}_{#1}}}\xspace}



\newcommand{\TDL}{\ensuremath{\text{TDL}}\xspace}
\newcommand{\TDLs}{\ensuremath{\text{TDLs}}\xspace}
\newcommand{\TDLite}{\ensuremath{\textit{TDL-Lite}}\xspace}
\newcommand{\TDLitef}{\ensuremath{\textsl{TDL-Lite}_{\textit{f}}}\xspace}


\newcommand{\TuDLite}[2]{\ensuremath{\textsl{T}_{\Until}\DLite^{#1}_{#2}}\xspace}
\newcommand{\TfDLite}[1]{\ensuremath{\textsl{T}^{f}_{\Until}\DLite_{#1}}\xspace}
\newcommand{\TkDLite}[1]{\ensuremath{\textsl{T}^{k}_{\Until}\DLite_{#1}}\xspace}

%\newcommand{\TDLiteb}{\ensuremath{T_{\Until}\DLite_{bool}}\xspace}
%\newcommand{\TfDLiteb}{\ensuremath{T^{f}_{\Until}\DLite_{bool}}\xspace}
%\newcommand{\TkDLiteb}{\ensuremath{T^{k}_{\Until}\DLite_{bool}}\xspace}

\newcommand{\TusDLf}{\textsl{T}_{\mathcal{US}}\textit{DL}_{\textit{f}}}

\newcommand{\TALC}{\ensuremath{\smash{\mathcal{T}_{\U}\mathcal{L}_{\mathcal{ALC}}}}\xspace}
%\newcommand{\TALC}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}
\newcommand{\TALCQI}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALCQI}}}}}

\newcommand{\TALCf}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}

\newcommand{\TALCk}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}
\newcommand{\TALCfk}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}

\newcommand{\TALCfg}{\ensuremath{\smash{\textsl{T}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}
\newcommand{\TALCfkg}{\ensuremath{\smash{\textsl{T}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}
%\newcommand{\TALCf}{\ensuremath{\smash{\textsl{T}^{f}_{\U}{\mathcal{ALC}}}}\xspace}
%
%\newcommand{\TALCk}{\ensuremath{\smash{\textsl{T}^{k}_{\U}{\mathcal{ALC}}}}\xspace}
%\newcommand{\TALCfk}{\ensuremath{\smash{\textsl{T}^{k}_{\U}{\mathcal{ALC}}}}\xspace}
%
%\newcommand{\TALCfg}{\ensuremath{\smash{\textsl{T}^{f}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}
%\newcommand{\TALCfkg}{\ensuremath{\smash{\textsl{T}^{k}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}

\newcommand{\TALCfB}{\ensuremath{\smash{\textsl{T}^{f}_{\Box}{\mathcal{ALC}}}}\xspace}

\newcommand{\TuALC}[1]{\ensuremath{\smash{\textsl{T}^{#1}_{\U}{\mathcal{ALC}}}}\xspace}



%%%
%%% MONODIC AXIOMS

\newcommand{\monod}{\ensuremath{\smash{\textnormal{\textit{\textbf{T}}}_{\U}{\textnormal{\textbf{QL}}_{\monodic}}}}\xspace}


%%%
%%% FINITE VS INFINITE TRACES

\newcommand{\finit}[2]{\textnormal{\ensuremath{\smash{\textsf{F}_{#1 #2}}}\xspace}}
\newcommand{\infinit}[2]{\textnormal{\ensuremath{\smash{\textsf{I}_{#1 #2}}}\xspace}}

\newcommand{\last}{\ensuremath{\textit{last}}\xspace}

\newcommand{\Pre}{\ensuremath{\textit{Pre}}\xspace}
\newcommand{\Prel}[1]{\ensuremath{\Pre_{l \geq #1}}\xspace}

\newcommand{\Ext}{\ensuremath{\textit{Ext}}\xspace}

\newcommand{\satfin}[1]{\ensuremath{\textsc{sat}_{f}(#1)}\xspace}
\newcommand{\satinf}[1]{\ensuremath{\textsc{sat}_{i}(#1)}\xspace}

\newcommand{\equivfin}[2]{\ensuremath{#1 \equiv_{\Fmf} #2}\xspace}
\newcommand{\equivinf}[2]{\ensuremath{#1  \equiv_{\Imf} #2}\xspace}
%\newcommand{\equivfin}[2]{\ensuremath{\textsc{equ}_{f}(#1, #2)}\xspace}
%\newcommand{\equivinf}[2]{\ensuremath{\textsc{equ}_{i}(#1, #2)}\xspace}


%%%
%%% DEFINITE DESCRIPTIONS

\newcommand{\NIInt}{\ensuremath{{\sf N}_{\sf I}^{\Imc}}\xspace}

\newcommand{\Ex}{\ensuremath{\mathsf{Ex}}\xspace}

\newcommand{\De}{\ensuremath{\mathsf{De}}\xspace}
%\newcommand{\De}{\ensuremath{\mathsf{Ex}}\xspace}


\newcommand{\exrel}{\ensuremath{\downarrow\Ex}\xspace}

\newcommand{\derel}{\ensuremath{\downarrow\De}\xspace}


\newcommand{\OutDom}{\ensuremath{\Delta}\xspace}
\newcommand{\InnDom}{\ensuremath{\mathfrak{d}}\xspace}

%\newcommand{\defdes}{\ensuremath{\smash{\textit{\riota \,}}}\xspace}
\newcommand{\defdes}{\ensuremath{\smash{\iota}}\xspace}

\newcommand{\concgzero}{\ensuremath{C^{\geq 1}_{\tau}}\xspace}
\newcommand{\concleqone}{\ensuremath{C^{\leq 1}_{\tau}}\xspace}
\newcommand{\conceqone}{\ensuremath{C^{= 1}_{\tau}}\xspace}


\newcommand{\topex}{\boldsymbol{{\mathsf{T}}}}
%\newcommand{\topex}{{\rotatebox[origin=c]{-90}{$\models$}}}

\newcommand{\simul}{\ensuremath{\leq}}






%%%
%%% PARTIAL CLOSED WORLD ASSUMPTION

\newcommand{\pcwmodels}{\mathbin{\ensuremath{\smash{\models_{{\sf PCWA}(\Sigma)}}}}\xspace}

%%%
%%%
%%% COMPLEXITY

\newcommand{\ACz}{{\ensuremath{\textsc{AC}^0}}}
\newcommand{\LogSpace}{\textsc{LogSpace}}
\newcommand{\NLogSpace}{\textsc{NLogSpace}}
\newcommand{\PTime}{\textsc{PTime}}
\newcommand{\NP}{\textsc{NP}}
\newcommand{\PSpace}{\textsc{PSpace}}
\newcommand{\ExpTime}{\textsc{ExpTime}}
\newcommand{\NExpTime}{\textsc{NExpTime}}
\newcommand{\ExpSpace}{\textsc{ExpSpace}}
\newcommand{\expsp}{\textsc{ExpSpace}}


%%%
%%%
%%% SANS-SERIF LETTERS

\newcommand{\Asf}{\ensuremath{\textsf{A}}\xspace}
\newcommand{\Bsf}{\ensuremath{\textsf{B}}\xspace}
\newcommand{\Csf}{\ensuremath{\textsf{C}}\xspace}
\newcommand{\Dsf}{\ensuremath{\textsf{D}}\xspace}
\newcommand{\Esf}{\ensuremath{\textsf{E}}\xspace}
\newcommand{\Fsf}{\ensuremath{\textsf{F}}\xspace}


%%%
%%%
%%% FRAKTUR LETTERS

\newcommand{\Amf}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand{\Bmf}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\Cmf}{\ensuremath{\mathfrak{C}}\xspace}
\newcommand{\Dmf}{\ensuremath{\mathfrak{D}}\xspace}
\newcommand{\Emf}{\ensuremath{\mathfrak{E}}\xspace}
\newcommand{\Fmf}{\ensuremath{\mathfrak{F}}\xspace}
\newcommand{\Gmf}{\ensuremath{\mathfrak{G}}\xspace}
\newcommand{\Hmf}{\ensuremath{\mathfrak{H}}\xspace}
\newcommand{\Imf}{\ensuremath{\mathfrak{I}}\xspace}
\newcommand{\Jmf}{\ensuremath{\mathfrak{J}}\xspace}
\newcommand{\Kmf}{\ensuremath{\mathfrak{K}}\xspace}
\newcommand{\Lmf}{\ensuremath{\mathfrak{L}}\xspace}
\newcommand{\Mmf}{\ensuremath{\mathfrak{M}}\xspace}
\newcommand{\Nmf}{\ensuremath{\mathfrak{N}}\xspace}
\newcommand{\Omf}{\ensuremath{\mathfrak{O}}\xspace}
\newcommand{\Pmf}{\ensuremath{\mathfrak{P}}\xspace}
\newcommand{\Qmf}{\ensuremath{\mathfrak{Q}}\xspace}
\newcommand{\Rmf}{\ensuremath{\mathfrak{R}}\xspace}
\newcommand{\Smf}{\ensuremath{\mathfrak{S}}\xspace}
\newcommand{\Tmf}{\ensuremath{\mathfrak{T}}\xspace}
\newcommand{\Umf}{\ensuremath{\mathfrak{U}}\xspace}
\newcommand{\Vmf}{\ensuremath{\mathfrak{V}}\xspace}
\newcommand{\Wmf}{\ensuremath{\mathfrak{W}}\xspace}
\newcommand{\Xmf}{\ensuremath{\mathfrak{X}}\xspace}
\newcommand{\Ymf}{\ensuremath{\mathfrak{Y}}\xspace}
\newcommand{\Zmf}{\ensuremath{\mathfrak{Z}}\xspace}

\newcommand{\FEmf}{\ensuremath{\Fmf \cdot_{E} \Emf}\xspace}
\newcommand{\FEmfC}{\ensuremath{\Fmf \cdot_{E} \Emf}\xspace}
\newcommand{\FImf}{\ensuremath{\Fmf \cdot \Imf}\xspace}
\newcommand{\FEImf}{\ensuremath{\Fmf \cdot_{E} \Imf}\xspace}



%%%
%%%
%%% MATHCAL LETTERS

\newcommand{\Amc}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\Bmc}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\Cmc}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\Dmc}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\Emc}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\Fmc}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\Gmc}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\Hmc}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\Imc}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\Jmc}{\ensuremath{\mathcal{J}}\xspace}
\newcommand{\Kmc}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\Lmc}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Mmc}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\Nmc}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\Omc}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\Pmc}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Qmc}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\Rmc}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\Smc}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\Tmc}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\Umc}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\Vmc}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\Wmc}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\Xmc}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\Ymc}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\Zmc}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\FEmc}{\ensuremath{\Fmc \cdot_{E} \Emc}}
\newcommand{\FImc}{\ensuremath{\Fmc \cdot \Imc}}
\newcommand{\FEImc}{\ensuremath{\Fmc \cdot_{E} \Imc}\xspace}


%%%
%%%
%%% BLACKBOARD LETTERS 

\newcommand{\Abl}{\ensuremath{\mathbb{A}}\xspace}
\newcommand{\Bbl}{\ensuremath{\mathbb{B}}\xspace}
\newcommand{\Cbl}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Dbl}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\Ebl}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\Fbl}{\ensuremath{\mathbb{F}}\xspace}
\newcommand{\Gbl}{\ensuremath{\mathbb{G}}\xspace}
\newcommand{\Hbl}{\ensuremath{\mathbb{H}}\xspace}
\newcommand{\Ibl}{\ensuremath{\mathbb{I}}\xspace}
\newcommand{\Jbl}{\ensuremath{\mathbb{J}}\xspace}
\newcommand{\Kbl}{\ensuremath{\mathbb{K}}\xspace}
\newcommand{\Lbl}{\ensuremath{\mathbb{L}}\xspace}
\newcommand{\Mbl}{\ensuremath{\mathbb{M}}\xspace}
\newcommand{\Nbl}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Obl}{\ensuremath{\mathbb{O}}\xspace}
\newcommand{\Pbl}{\ensuremath{\mathbb{P}}\xspace}
\newcommand{\Qbl}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Rbl}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\Sbl}{\ensuremath{\mathbb{S}}\xspace}
\newcommand{\Tbl}{\ensuremath{\mathbb{T}}\xspace}
\newcommand{\Ubl}{\ensuremath{\mathbb{U}}\xspace}
\newcommand{\Vbl}{\ensuremath{\mathbb{V}}\xspace}
\newcommand{\Wbl}{\ensuremath{\mathbb{W}}\xspace}
\newcommand{\Xbl}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\Ybl}{\ensuremath{\mathbb{Y}}\xspace}
\newcommand{\Zbl}{\ensuremath{\mathbb{Z}}\xspace}


%%%
%%%
%%% BOLDFACE LETTERS

\newcommand{\Abf}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\Bbf}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\Cbf}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\Dbf}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\Ebf}{\ensuremath{\mathbf{E}}\xspace}
\newcommand{\Fbf}{\ensuremath{\mathbf{F}}\xspace}
\newcommand{\Gbf}{\ensuremath{\mathbf{G}}\xspace}
\newcommand{\Hbf}{\ensuremath{\mathbf{H}}\xspace}
\newcommand{\Ibf}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\Jbf}{\ensuremath{\mathbf{J}}\xspace}
\newcommand{\Kbf}{\ensuremath{\mathbf{K}}\xspace}
\newcommand{\Lbf}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\Mbf}{\ensuremath{\mathbf{M}}\xspace}
\newcommand{\Nbf}{\ensuremath{\mathbf{N}}\xspace}
\newcommand{\Obf}{\ensuremath{\mathbf{O}}\xspace}
\newcommand{\Pbf}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\Qbf}{\ensuremath{\mathbf{Q}}\xspace}
\newcommand{\Rbf}{\ensuremath{\mathbf{R}}\xspace}
\newcommand{\Sbf}{\ensuremath{\mathbf{S}}\xspace}
\newcommand{\Tbf}{\ensuremath{\mathbf{T}}\xspace}
\newcommand{\Ubf}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\Vbf}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\Wbf}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\Xbf}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\Ybf}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\Zbf}{\ensuremath{\mathbf{Z}}\xspace}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}} 
\newcommand{\Nbb}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Zbb}{\ensuremath{\mathbb{Z}}\xspace}





%%%
%%%
%%% USELESS

%\newcommand{\A}{\ensuremath{\mathcal{A}}}
%\newcommand{\K}{\ensuremath{\mathcal{K}}}
%\newcommand{\T}{\ensuremath{\mathcal{T}}}
%\newcommand{\LL}{\ensuremath{\mathcal{L}}}

%
%\newcommand{\QT}{Q_\T}
%\newcommand{\QA}{Q_\A}
%
%\newcommand{\TuDLbn}{\ensuremath{\smash{\textsl{T}_{\mathcal{US}}\DLbn}}}%
%\newcommand{\TuDLcn}{\ensuremath{\smash{\textsl{T}_{\mathcal{US}}\DLcn}}}%
%
%\newcommand{\TdDLan}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLan}}}%
%\newcommand{\TdDLbn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLbn}}}%
%\newcommand{\TdDLkn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLkn}}}%
%\newcommand{\TdDLcn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLcn}}}%
%
%\newcommand{\TdDLaHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLaHN}}}%
%\newcommand{\TdDLbHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLbHN}}}%
%\newcommand{\TdDLkHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLkHN}}}%
%\newcommand{\TdDLcHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLcHN}}}%
%
%\newcommand{\TdxDLan}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLan}}}
%\newcommand{\TdxDLbn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLbn}}}%
%\newcommand{\TdxDLkn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLkn}}}%
%\newcommand{\TdxDLcn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLcn}}}%
%
%\newcommand{\zSVDLan}{\ensuremath{\smash{\textsl{T}_{U}\DLan}}}%
%\newcommand{\zSVDLb}{\ensuremath{\smash{\textsl{T}_{U}\DLbn}}}%
%\newcommand{\zSVDLk}{\ensuremath{\smash{\textsl{T}_{U}\DLkn}}}%
%\newcommand{\zSVDLc}{\ensuremath{\smash{\textsl{T}_{U}\DLcn}}}%
%
%\newcommand{\TxDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{X}\DLbn}}}%
%\newcommand{\TdrDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P}\DLbn}}}%
%\newcommand{\TurDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{U}\DLbn}}}%
%
%\newcommand{\TdxrDLcn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P\!X}\DLcn}}}%
%\newcommand{\TdxrDLkn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P\!X}\DLkn}}}%


